Provable Meta-Learning of Linear Representations

Meta-learning, or learning-to-learn, seeks to design algorithms that can utilize previous experience to rapidly learn new skills or adapt to new environments. Representation learning -- a key tool for performing meta-learning -- learns a data representation that can transfer knowledge across multiple tasks, which is essential in regimes where data is scarce. Despite a recent surge of interest in the practice of meta-learning, the theoretical underpinnings of meta-learning algorithms are lacking, especially in the context of learning transferable representations. In this paper, we focus on the problem of multi-task linear regression -- in which multiple linear regression models share a common, low-dimensional linear representation. Here, we provide provably fast, sample-efficient algorithms to address the dual challenges of (1) learning a common set of features from multiple, related tasks, and (2) transferring this knowledge to new, unseen tasks. Both are central to the general problem of meta-learning. Finally, we complement these results by providing information-theoretic lower bounds on the sample complexity of learning these linear features.

==> icml/Code/.git/objects/36/3d63ae4a001bbd0d34f500ba9adb9f19be716c <==
x¥ÎM @aל'h`:ü41ƸòfZ¡
ÒûÛoàö[¼¼¸–'»T§Þˆd0Ä4zeHÁšqˆ9xEì¬KÈV±…FµK¶‰1Mà,¦‰À$šÇ!š5DaïËÚä#¿è½ÈgËÛÞB¥šåµ~­tŸKȯK\ËMjãF´Æ¡—g啇«þŠü*¹ÎârN

==> icml/Code/.git/objects/47/348079968540d09c813db246e063a7f22a1300 <==
xMÕwTTGðEPjb+V°@@0'D34(+$^ײÊXøv…X±\ŒÝØ{!ˆØEØˆ`Æb,Ă
ŠŠ9Æv̄ٓ"ýcϾ߼¹{ß7óދŒOŒtñòõí©™b;7]]F"`°D¤"ÄØèQË-ʘœ"ê•h2x$$Ç[b#L¦ˆTGsTD|"ɶjÜ1ڒšdp"®–,1Úµµ­M:êìÝ´¶:©½áôA~j¾´êF8˜ªfL{!àȨG¨ccàp¿O›f™žÏ0œ"="¹Æ³J £1¡‰Rÿ!Ǘ–mz"ðãcBS¥Ž¶ÝÌú@àF3Bs¥¡Ïªl7ÅÜpf´ ´Têì÷¡áûÕe­­	mz´uSC+§^_>+£¡½Òž-zMٙ)µ£#¡"R§W+Óú¾$ЙáJ°V BÇ.4ü¢@FWB7uî¼èÿGÇ
º3Ü	J§û¹Ä9ää	|Êð$x)ž™UèZ Ûàc`ôÔ9ü·X£ñ™½¬7Íbºðv×S_Æç"/T‰€©¹®é¾dô&ôQjo¸6®Yï{_1ÁOéZ÷Ksw4–i|Íð'(EÛã€ÒÛ}ýß(ýËý<'l,dô'PÚùȵ‡]J'ZÂ@™g°µ½®*ˎÉ4Bß¾S¿ˆó;ø"_`ƒƒ•}u¹Œz
"2†">mUq«ó¸SC:Â0¥¡¥¸+u8ca¤Ò9"cã›,UÏEWÚyj"åv2ûï"H™g"®ŽÌ3²fó#ZƒµÝîEŠ+ž	Œfü@ˆQ<¢ƒv¾*3ŽeŒ!Ä)<iüÞÉïåîŒg$ŒJ;¸SÝ¡ZVHd$ ôí»NËå¹&†™`QJ6ÕƺR"c	ã"&åÕËöK"R©"ešã­í\–s2æœÀÆDÂ$5¡ŠÞ˜'!¯o2c
!MiÂ;ûXdšSÓӕFڕϸ^rV`ƒ	éJÇuÌÜåÐRæ6"ña–Ò'§ñ&Wi6ca®RóŸ'«ÎEóó	dšuõdšæX£%F&úïÃäg=Y{ÞúhU®ÿy'‹KKU•–•«|öJ]ÆXNX¡´ÛrsÖã0©+««•6Öi˜kA…ÀÆZÂ:¥¯½õJCäf^ÏØ@ب´gxʛÛën
d0~!d*Ý~Çl¯"Ùó&Fa³Œt‹µ½1OîL›ž$°•±°]M¨oo¬œ?Y ›ñ+a‡ÒAšaދç­ØÉØEØ­4ÑÛ¿"£õ=Œ½"}J[Ým70eéýŒÂ¥÷Œ–£³ãVd"ü¦ÔasۿŨE‡¹"#2Ò£:ÇÿE*oùcz·¶ì"gã±@nÇŒ<Â愈{vß^–†òQw''O(Pé?âˆyQ±À)ÆiÂ¥cÜñô¨"{ã,ã¡Pi£¸áÛú¤ÀyÆÂE¥NçÒ׬ϸĸL(Rºm÷ú{Õ÷\a\%ËD¯YÛóòÊìÚ|Ɂ?×	7ԄòŒÀâ쌁›Œ["?•ö;>óÝa¯…·%"R¥ûæïzÙ>M࣌pWé¼-_×î6Uàã>áÒîéo´L(g<$<RÚÔϡֆ,ÇŒ
B¥LôIÍ-k¶à©UnÚhí©à6Á.¶Á~u'§ÔÖ8jÞ]Ñx¦®ùeÂsmm½\
‹)"ÖnÄ­sM!‹Ál'‡ÕòÐN›If¼Ô¶IöøîÎݏ

==> icml/Code/.git/objects/62/75b63fd6565785bbc9e6a8fb1b2c14cf1a00aa <==
xMÕyxLWðD&ˆ¥ilA"	Q[bÍHðÑˈ,CIfÞÉD­úil%ö}kiìµ…(©½Ö–*‰D"ö‰9óôéüqŸ3¿{Ïw¿ûιgÂbLa­:ûúv·›í;­¾¶]¬Ñ:"bM±°7 š6<.!֜än²½bb¬Q¡Kh'&><4&Ô¢ƒ:¯‰°&™T×W"%&ù¢†ÎNg?Ž"šZƒÞ^ª?j¾—ŸªƒÎΊÚaµ¢OeNÛ¾L@Ãp"ԉtˆ¬P‹{œ\Úö¥@]F='³Ò¦Ë{mÓþS"PŸÑ€ÐPiÝ?È(hÄøˆà¢4pËûG^=ø˜áJhl«ûzõõÔà"&Œ¦"fJ+)~C}·|æ7B£-µêÔÛËí|2\¯´b¸Z+usYï<âÝeOmm•úYÆ]í¦»'ð)£ÁVá¦Ç]Í;—[íOum¢Ë"‡•CdÝŒŽ/¥Ûs[[+¥vb|Fè¬4ºÔ;ù͛s]]	݌ŒîúZÿýX"Lð6ÀÇv»ý¢6ßY!óôeô ø©#ó^DîÏݓáOè¥ô`ãzýžö"õfB¥™æíËê>èËèGP:%ý¯ìK%÷ú3*õIÚÕãœå'À Æ`Â¥–卜Ø@j CG*ó²µ7u_Ï჋o
3††«	%N™›Íš#D©´Ø·Å˜ù‰×F1>'|¡t².÷dƒ.—F3ô"1J—xÙ1÷¬ÀXÆ8Âx¥ý#Ž6óNË00&B"¦=Žð98í´ÀDF(!Læ®w"y†U-~D`´µ»>ùvÛ¿B*&1&"m&ÞèvXfň&LQZ:zµeÖX©1ŒXBœÒ"÷UïÏ¥H51Ì(ÍoÐ|÷½T#ž`UšãWáñm¹@c*áK¥WÌ0­'šÈH"L"iN·µ×áXà<b¹2f0'	3Մ"‡Ú+}ŸIÅ˜MøJéÙ`÷µÏœøš1‡ðÒ¡C†›JgÉkç2˜0O©5Í¿"`ŠLs>#…°@éµ®O%^½(°'JøViNÒ¿,4Æ"Âb™æ½"L3>*Î)ý°™,5`™­ç2h*/ñwŒå"ªJe§"úožKMg¬$¬Rú.ÑyÓ±
©«kk•Nhø`¢©Lê:ÆzÂ¥‹ýܧKÝÈØDج´0ÐÑS{RêÆVÂ6¥Y>{Ú¹<"º±ƒ°SFú½­½ög×-3î‹ø±‹°[M˜2(ú"ß-‹ÀŒÂ¥§cï8¿Û*°—±°_©q·o·1	‡"^)qÉ>Ý&\à0ãá'¥ÜrtñœôYGÇǕ¦OwÿZgø™q'pRFzJ¯ù_¤ò•?mÀ[Ë[ríp-—O"É8K8§ŠXSÔ.­Ô,ÆyÂ/Jg·jÝÉÏ"7ËŒ‹"l¥YÍv'ð_——•ve?öPûB+Œ«"kJ}—{zw*¸Î¸AøM)MVnŸš'p"q‹p[&zÇÖÞÀôÞÍgö7ÜeÜ#ü®&xî}•'´DàÆ}Â¥sKÿ6mõÚ!ÃxHx¤Ôšä]éqï @.ã1á‰Òº†Uör=%ð'ã)!OéMÞYÑD.Ç|Æ3BÒÛæù™f³Ü`ž3
	E2Ñú:2Q«%4*.$.$&*ފbJ´º݅ ÅöA­'ú8Í®d×ÄXõ—ºˆª'¥ºU£Q("£{‡Õo
‰C¹®‹¾ºüj1šãQ¡Ó$xývÏáV

==> icml/Code/.git/objects/94/4e33f28957509402e48c2df531e7b05ac9e7dd <==
x¥ÎA …aלb. )í@bŒ'påZ'–ÄûÛx·ßâ/îÛV: ÅSo"à)"€™y ÍÙ8ž${$§ÑÆ8!¥hԋ›ÔƒÂL)ì£Õâ"õÑ¥`1äÁ!›1˜èú²7x"UÞ<[y}W©®õgý û¼qY/qßn`F§ÉOd=œµÓZz\íòWDqJ¥ÎMõU÷O®

==> icml/Code/.git/objects/bc/eaa157c51c49a09f31b03a79de982d3ebe1d5b <==
x¥ÎK!Pל¢/ éæ3@bŒ'på §Q‡1ˆ÷wô
¦voQU¼.K ­Ù.y¡vÙ$	Ʉ8Iðä&Ü"¬s(<«gêÒx&ËÎxb´Ž'—Rr¤¬‹æ¢cÊvÂh­Jïq_;\êC^w¸öú|÷Ô¤U8¶ŸÎ·%Õǁ×åäúh'°Ç€¨6Ý®ù«D¥y®í廩>0äNa

==> icml/Code/.git/objects/cd/e29bf75822d1fc1ebb29f16c3b21f599ab5db8 <==
x­ÎM
Â0@a×9E.`™4͈ˆèRWz€L2¥Á6-1]x{¥gpû-/ÌӔ*oØÕBÄ¥sÖÄ­	Ò z´°€F÷?#«HƒU½Slñ…råR˨¥§ÎÄQv½@ï|Dׇd"̯u˜¿§'Þ"´¬ÅgʉòfõG§"Úæ–Æ'rNëԜ©¼h¤Os½<\(ã:­'|€…m¾ÒŸ³,ΙØe7XZ

==> icml/Code/.git/objects/f4/32e7556dea2fcef49a52c2432c4170f72411f3 <==
xMÕ{XÍwð""*3sÍ=¤H.Y-C_ä2~J>¨ÎR§"²:õ>çÄl!·O³¡lÌ%ƈ\æ6wÊýn$s‰\¢\"¹=Øû®ïyöìüqžó{ý¾ßÏù<ïßç{NLbrL«®þºtÇÉÐyëkétº$"-z%%'ÁÁ€jÞFsjRʤNÆd‹©SRj¢-!Úb‰žäb5F'F[\à¨î»ÄÚ&¥˜\य&KÄ¢º¦Ó2Pƒàì­9ê¤öDÍÐÐÐÁïå«êMÓÙP+&¸æ´Ui·<pa¸Üâ㝃kæfV.)jT)P›ñ¡ŽÒJýÈi~2ê>Rz~cnjs¤ÖcÔ'4Pú÷òK™©î÷2+½Vâ1M·ã®€;£	¡©ÒÖS;FÙjKmÆhNha2 ¥·ºuóbžWBÉUVBk¥±A­ë]hÃhKðTú(Ìϼ­ãav/'½ÂWztézI =£ÁG­-Œ]íµö"@G†/¡"Òìû¥ÕÓÇèÌèBèª4ß½u†¯¯\ëÇèFøØÄð××üïaÅ%#À€Oì_ç}1>2{ñS@Fw§ªDüÛ^YZó==	½"ž¸ôúV_]‰@Cz+Ý^¸»sdý;}}	ÁJOy¸Ø£X £?a€Ò:º´}ð¹%0ñaÒí÷]1κ!0˜¡†È<Cìí-=þ¤¨P¦ÊJSrÚ¸†+Û-0ŒA"áJ•4	ˆ?+0'1'®ÔßíƒðVKåÚ†ž©txÝ("Æ#££	c":¯œpd'ÌÓÀøœ¥ts'¾³òÆ2¢	12O£¾†Ì3¦jøk€ÉÞnB îºË9ŒcŒ#Ä«ÆlóûÒvrâã	_(Ýd\éÔCj"#‰`V¡ißíÞ3dF
JýÖ¶,ؙ,×ZV'Mé逛£Ÿ¤2&&*µÔ¾v.CVø'1‰ð•Lók{{Ïl9ÉçÉ4Ó"	SԆWãvô?xF`*#0Mi~³Æ¹câätNgÌ ÌT<·°³›õ˜À,2"fíµN{_xTàÆ·"ÙJu[†v'¹Ía|G˜«tæ†3qVÙÃ÷Œódšóõ®2Mk'Ù/ý÷Çd™öžËã[Ô­ûFhc!áGUÅgúš ¬£Rb,",Vêz}Œû‹©?3––*Ðg"ÿ'²ÇËË	ÙJWìŸÙ8õ•<Ä++	¿(5׫,Nñ.XÅXMøUinAXÅü"kk	92ÒuööšmЯC¸ÀzF.aƒÚàwq}Ž×€tŒM"ÍJûDô,õ)ðca«ÒyL¸¶M`c;a‡Ò×	ž|³Å2ß;	»"îÎ˸üî݁݌="½J®H7bF–À>Æ~ÂéA½Ëÿ"•G>π|{Ë#‡6ôÕråØb&QEr_žzW)÷QÆ1Âq¥åËo¯ÑË_®Œ""SJµÇoo¼¹#OÚiÆÂY¥¶NË)8Ç8OøCiø϶û.0.
"Ž.òЪß.p‰QH¸,ýÓÞÞüçåæñÓW
\a\%\Sz÷ÎÙÓ`«ÀuFá†Ò)™w͸É(&ÜRz(ÈÕÍyõDÛŒ;"»J›ÅÍ"Ϥ"qp_iÅ» —¦
"2Ê"6ÓÒËãò2ËDË«Žüˆ¨Ä«
Oxê­Åj'Bæ9"´ré]#$Ý-DçnªúïŠE…[õɂgZu½³|6Kt'9ʌJͽªÍdµÉËçòÒIÞ¶˜R¬x¡¹¤vúÑ@Ûe

==> icml/Code/.git/objects/f6/de35242cdb2764dbe4225d821ee493c5cc12cf <==
xu'I›@"sæWô}4¡Ù2Ñ4fÇf3†ÜXÚÐ6`Ì2ŒýëãL®É;•>©TÒ«*/]Gg€$éÛ<ʊ#G't"x® P'e¾xˆ£QùŠÀ\–‰É—¹¹ŒÀ§-™ŒtXƼ'=?ú/6?ÐkÝå´ý^^ºŸ€"dUD¢¨pà*2úˆžÉ,:ÛKñ0^F2´·×šÎÍRüÇVõDkðüç4Ãr|Z!Ø;–"Cl|q0`´RÃXÛ`i'KÜmÙlb͓›"|£³b\َƒu¯³µ45j[Towy|Š/ȼۉO)ÏûÈ9ßs±-DFWéçkµCöµH"I2ö¦rƒÎKa-ªÇeûç÷É°2À* :{YŸÖ5\]œ¶OÚNWË:dkž(Ùl^Ï]6ýÏ­ÆÚ»'ô¦Ç~Âû'gn''vœÙj£Û®--þÖNÝ¡±Ïf"àMÍTcJ£͞%Ê^YÖ¢é0«"=f€ßoi­S_£Íìî®ÔþR?æâñ©Õ¶¡ÊÛYhлcÁ*˜qžÔ¾lFª²gÙc@šY:4Y#HéȊpAgÿôފ†»×Ý}À›Ïãô~é‹x/¶]j
CdI_g/xÉn—ÇC¿º1|ýߍ1NOgš·àï0~ìØÍ¿

==> icml/app_aux.tex <==
%!TEX root = main.tex

\section{Auxiliary Results}
Here we collect several auxiliary results. 

We begin by stating a simple matrix perturbation result.
\begin{lemma}
\label{lem:mat_pert}
	Let $\A$ be a positive-definite matrix and $\E$ another matrix which satisfies $\norm{\E \A^{-1}} \leq \frac{1}{4}$, then,
	\begin{align*}
		(\A + \E)^{-1} = \A^{-1} + \F
	\end{align*}
	where $\norm{\F} \leq \frac{4}{3} \norm{\A^{-1}} \norm{\E \A^{-1}}$.
\end{lemma}
\begin{proof}
\begin{align*}
	(\A+\E)^{-1}=\A^{-1}(\I+\E \A^{-1})^{-1}
\end{align*}
Under the condition, $\norm{\E \A^{-1}} \leq \frac{1}{4}$, $\I+\E \A^{-1}$ is invertible and has a convergent power series expansion so
\begin{align*}
	(\A+\E)^{-1} = \A^{-1}(\I-\E \A^{-1}+(\E \A^{-1})^2+\hdots) = \A^{-1} + \F
\end{align*}
where $\F = \A^{-1} \cdot (-\E \A^{-1}+(\E \A^{-1})^2+\hdots)$. Moreover, 
\begin{align*}
	\norm{\F} \leq \norm{\A^{-1}} (\norm{\E \A^{-1}}+\norm{\E \A^{-1}}^2+\hdots) \leq \frac{\norm{\A^{-1}} \norm{\E \A^{-1}}}{1-\norm{\E\A^{-1}}} \leq \frac{4}{3} \norm{\A^{-1}} \norm{\E \A^{-1}}
\end{align*}
\end{proof}

We now present several results related to the concentration of measure.

\begin{lemma}
    Let $x, y$ be mean-zero random variables that are both sub-Gaussian with parameters $\kappa_1$ and $\kappa_2$ respectively. Then $z = xy-\mE[xy] \sim \sE(8 \kappa_1 \kappa_2, 8 \kappa_1 \kappa_2)$.
    \label{lem:prod_sg}
\end{lemma}

The proof is a standard argument and omitted. Next we prove a matrix concentration result for the individually rescaled covariance matrices of i.i.d. random variables. The proof uses a standard covering argument.
\begin{lemma}
	\label{lem:scaled_sgvec}
	Let $\X \in \mR^{n \times d}$ be a random matrix with rows $a_i \x_i$, where $\x_i$ are i.i.d. random vectors satisfying the design conditions in \cref{assump:design}. Then, 
	\begin{align*} 
		\norm{\frac{1}{n} \X^\top \X - \sumton a_i^2 \mSigma} \leq \norm{\mSigma} K^2 \max(\delta, \delta^2) \quad \text{ for } \delta = C(\sqrt{d/n}+t/\sqrt{n})
	\end{align*}
	with probability at least $1-2\exp(-t^2)$. Here $C$ denotes a universal constant and $K = \max_i \abs{a_i}$.

\end{lemma}
\begin{proof}
First note that we bring all the vectors to isotropic position by rotating so that $\norm{\frac{1}{n} \X^\top \X - \sumton a_i^2 \mSigma} \leq \norm{\mSigma} \norm{\sumton a_i^2 (\mSigma^{-1/2} \x_i)(\mSigma^{-1/2} \x_i)^\top - \sumton a_i^2 \I_d}$. Now by definition for any fixed $\v \in \mathbb{R}^d : \norm{\v}=1$, each $\v^\top \mSigma^{-1/2} \x_i$ is $\sG(1)$ and hence $a_i^2 (\v^\top \mSigma^{-1/2} \x_i)(\mSigma^{-1/2} \x_i)^\top \v$ is $\sE(8a_i^2, 8a_i^2)$ by \cref{lem:prod_sg}. For the latter quantity \citet[Theorem 4.6.1, Eq. 4.22]{vershynin2018high} proves the result when $a_i=1$ using a standard covering argument along with a sub-exponential tail bound. A close inspection of the proof of \citet[Theorem 4.6.1, Eq. 4.22]{vershynin2018high} shows that the aforementioned analogous statement holds when the sequence of random vectors is scaled by $a_i$.
\end{proof}

We now include two useful results on operator norm bounds of higher-order matrices. The results only require the condition of $O(1)$-L4-L2 hypercontractivity (which is directly implied by \cref{assump:design} -- see for example the sub-Gaussian moment bounds in \citet[Theorem 2.6]{wainwright2019high}). Formally, we say a random vector $\x$ is $L$-L4-L2 hypercontractive if $\mE[\langle \v, \x \rangle^4] \leq L^2 (\mE[\langle \v, \x \rangle^2])^2$ for all unit vectors $\v$. Also note that if $\x$ is hypercontractive this immediately implies that $\pv \x$ is also hypercontractive with the same constant where $\pv$ is an orthogonal projection operator. 
\begin{lemma} \label{lem:l4l2norm}
    Let $\x$ be a mean-zero random vector from a distribution that is $L$-L$4$-L$2$ hypercontractive with covariance $\mSigma$ and let $\pv$ be an orthogonal projection operator onto a rank-$r$ subspace. Then 
    \begin{equation}
    \norm{\mE[\norm{\x}^2 \x\x^\top]} \leq L \tr(\mSigma) \norm{\mSigma}; \quad \norm{\mE[\norm{\pv \x}^2 \x\x^\top]} \leq L r \norm{\mSigma}^2 ; \quad \norm{\mE[\norm{\x}^2 \pv \x (\pv \x)^\top} \leq L \tr(\mSigma) \norm{\mSigma}
    \end{equation}
\end{lemma}
\begin{proof}[Proof of \cref{lem:l4l2norm}]
     We introduce a vector $\v$ with $\norm{\v} \leq 1$. Then,
\begin{align}
    & \mE[\langle \v, \norm{\x}^2 \x \x^\top \v \rangle] = \mE[\norm{\x}^2 \langle \v, \x \rangle^2] \leq (\mE[\norm{\x}^4])^{1/2} (\mE[\langle \v, \x \rangle^4])^{1/2},
\end{align}
by Cauchy-Schwarz inequality.
For the first term we have $(\mE[\norm{\x}^4])^{1/2} \leq \sqrt{L} \tr (\mSigma)$ by \cref{lem:l4l2vec}. For the second term once again using $L$-L$4$-L$2$ hypercontractivity we have,
$(\mE[\langle \v, \x \rangle^4])^{1/2} \leq \sqrt{L} \mE[\langle \v, \x \rangle]^2 \leq \sqrt{L} \norm{\mSigma}$. Maximizing over $\v$ gives the result.
The remaining statements follow using an identical calculation and appealing to \cref{lem:l4l2vec}.
\end{proof}

\begin{lemma} \label[lemma]{lem:l4l2vec}
	Let $\x$ be a mean-zero random vector from a distribution that is $L$-L$4$-L$2$ hypercontractive with covariance $\mSigma$ and let $\pv$ be an orthogonal projection operator onto a rank-$r$ subspace. Then 
    \begin{align*}
      \mE[\norm{\x}^4] \leq L (\tr \mSigma)^2 ; \quad \mE[\norm{\pv \x}^2] \leq r \norm{\mSigma} ; \quad \mE[\norm{\pv \x}^2 \norm{\x}^2] \leq L r \norm{\mSigma} (\tr \mSigma) ; \norm{\mE[\norm{\pv \x}^4]} \leq L \norm{\mSigma}^2 r^2 
    \end{align*}
\end{lemma}

\begin{proof}[Proof of \cref{lem:l4l2vec}]
A short computation using the Cauchy-Schwarz inequality and L4-L2 equivalence shows that, 
\begin{align*}
     \mE[\norm{\x}^4] = \mE[(\sum_{i=1}^d \langle \x, \e_i \rangle^2)^2] =& \mE[\sum_{a,b} \langle \x, \e_a \rangle^2 \langle \x, \e_b \rangle^2] 
    \leq \sum_{a,b} (\mE[\langle \x, \e_a \rangle^4] \mE[\langle \x, \e_b \rangle^4])^{1/2} 
     \leq L \sum_{a,b} \mE[\langle \x, \e_a \rangle^2] \mE[\langle \x, e_b \rangle^2] \leq \\ L (\tr (\mSigma))^2.
\end{align*}

The second statement follows since $\E[\norm{\pv \x}^2] = \E[\tr(\pv \x\x^\top] = \tr(\pv \mSigma) \leq r \norm{\mSigma}$
where the last line follows by the Von-Neumann trace inequality and the fact $\pv$ is a projection operator. The final statements follow by combining the previous calculations.
\end{proof}


Finally, we prove a truncated version of the matrix Bernstein inequality we can apply to matrices that are unbounded in spectral norm. This is our primary technical tool used to show concentration of the higher-order moments used in the algorithm to recover the feature matrix $\B$.
\begin{lemma}
	\label{lem:trunc_mb}
	Consider a truncation level $R > 0$. If $Z_i$ is a sequence of p.s.d. independent random matrices and if $Z_i' = Z_i \Ind[\norm{Z_i} \leq R]$, then
	\begin{align*}
		\Pr[\norm{ \frac{1}{n} \sum_{i=1}^{n} Z_i - \mE[Z_i] } \geq t] \leq \Pr[ \norm{\frac{1}{n} \sum_{i=1}^{n} Z'_i - \mE[Z_i']} \geq t-\Delta] + n \Pr[\norm{Z_i} \geq R]
	\end{align*}
	where $\Delta \geq \norm{\mE[Z_i]-\mE[Z_i']}$. Further, for $t \geq \Delta$, we have that, 
	\begin{align*}
		\Pr[ \norm{\frac{1}{n} \sum_{i=1}^{n} Z'_i - \mE[Z_i']} \geq t-\Delta] \leq 2d \exp \left(\frac{n^2(t-\Delta)^2}{\sigma^2 + 2Rn(t-\Delta)/3} \right)
	\end{align*}
	where $\sigma^2 = \norm{\sum_{i=1}^n \mE[(Z_i'-\mE[Z_i'])^2]} \leq \norm{\sum_{i=1}^n \mE[Z_i^2]}$.
\end{lemma}
\begin{proof}
	The first statement follows by splitting on the event $\{ \norm{ Z_i} \leq R :  \forall i \in [n] \}$, along with a union bound, and an application of the triangle inequality to the first term. The second is simply a restatement of the matrix Bernstein inequality in \citet{tropp2012user} along with the almost sure upper bound $\norm{Z_i'-\mE[Z_i']} \leq \norm{Z_i'} + \norm{\mE[Z_i']} \leq R+\mE[\norm{Z_i'}] \leq 2R$. The final bound on the matrix variance follows from the facts that for the p.s.d. matrix $\sum_{i=1}^n \mE[(Z_i'-\E[Z_i'])^2] \preceq \sum_{i=1}^{n} \mE[(Z_i')^2]$ and that $(Z_i')^2 \preceq Z_i^2$.
\end{proof}





==> icml/app_expts.tex <==
%!TEX root = main.tex
\section{Experimental Details}
\label{sec:app_expt}

In our experiments we did find that gradient descent was able to decrease the loss in \cref{eq:objective_main}, but the algorithm was slow to converge. In practice, we found using the L-BFGS algorithm required no tuning and optimized the loss in \cref{eq:objective_main} to high-precision in far fewer iterations \citep{liu1989limited}. Hence we used this first-order method throughout our experiments as our optimization routine. Our implementation is in Python, and we leveraged the \texttt{autograd} package to compute derivatives of the objective in \cref{eq:objective_main}, and the package \texttt{Ray} to parallelize our experiments \citep{maclaurin2015autograd,moritz2018ray}. Each experiment is averaged over 30 repetitions with error bars representing $\pm 1$ standard deviation over the repetitions. All the experiments herein were run on computer with 48 cores and 256 GB of RAM.

Note that after optimizing \cref{eq:objective_main} directly using a first-order method in the variable ($\U, \V$), we can extract an estimate $\Bone$ of $\B$ by computing the column space of $\V$ (for example using the SVD of $\V$ or applying the Gram-Schmidt algorithm).

==> icml/app_gd.tex <==
%!TEX root = main.tex

\section{Proofs in \cref{sec:lf_gd}}
In our landscape analysis we consider a setting with $t$ tasks and we observe a datapoint from each of the $t$ tasks uniformly at random at each iteration. Formally, 
we define the matrix we are trying to recover as $\M_{\star} = (\balpha_1, \hdots, \balpha_t)^\top \B^\top \underbrace{=}_{\text{SVD}} \X^{\star} \D^{\star} (\Y{\star})^\top \in \mR^{t \times d}$, with $\U^{\star}=\X^{\star} (\D^{\star})^{1/2}$, $(\D^{\star})^{1/2} (\Y^{\star})^\top = (\V^{\star})^\top$, from which we see the observations,
\begin{align}
	y_i = \langle \e_{t(i)} \x_i^\top, \M_{\star} \rangle + \epsilon_i
\end{align}
where we sample tasks uniformly $t(i) \sim \{1, \hdots, t\}$ and $\x_i$ is a $\cN(0, \I_d)$ Gaussian random vector. Note that $\M^{\star}$ is a rank-$r$ matrix, $\U^{\star} \in \mR^{t \times r}$, and $\V^{\star} \in \mR^{d \times r}$. In this section, we denote $\tld = \max\{t, d\}$ and let $\sigstarl, \sigstarr$ be the $1$-st and $r$-th eigenvalue of matrix $\M^\star$. We denote $\cn^\star = \sigstarl/\sigstarr$ as its condition number.

We now present the proof of our main result.


\begin{proof}[Proof of \cref{thm:main_landscape_convert}]
	Under the conditions of the theorem note that by \cref{thm:main_landscape} we have that, 	
\begin{equation*}
	\norm{\U\V^\top - \M^\star}_F\leq O(\sigma\sqrt{t\frac{\max\{t, d\} r\log n}{n}}).
\end{equation*}
for $n \ge \polylog(n,d,t) C \mu^2 r^4 \max\{t, d\}  (\cn^\star)^4$. 
 First recall by \cref{lem:diverse_to_incoh} the incoherence parameter can in fact be shown to be $\mu = O(\bkappa)$ under our assumptions which gives the precondition on the sample complexity due to the task diversity assumption and normalization.
	To finally convert this bound to a guarantee on the subspace angle we directly apply \cref{lem:frob_to_angle} once again noting the task diversity assumption.
\end{proof}


\subsection{Geometric Arguments for Landscape Analysis}
Our arguments here are generally applicable to various matrix sensing/completion problems so we define some generic notation below.
\begin{equation}\label{eq:objective}
f(\U, \V) = \frac{2}{n}\sum_{i=1}^n (\la \A_i, \U \V\trans \ra - y_i)^2 + \frac{1}{2}\fnorm{\U\trans\U - \V\trans\V}^2
\end{equation}
where $\A_i = \sqrt{t} \e_{t(i)} \x_i\trans$. We work under the following constraint set for large constant $C_0$:
\begin{equation}\label{eq:constraint}
\cW = \{~ (\U, \V) ~|~ \max_{i\in[t]} \norm{\e_i\trans \U}^2 \le \frac{C_0 \mu r \sigstarl}{t}, \quad 
\norm{\U}^2 \le C_0 \sigstarl, \quad \norm{\V}^2 \le C_0 \sigstarl ~\}
\end{equation}

We renormalize the statistical model for convenience as:
\begin{equation}\label{eq:model}
y_i = \la \A_i, \M^\star\ra + n_i
\end{equation}
$n_i \sim \sqrt{t} \sigma \cdot \epsilon_i$ where $\epsilon_i$ is a sub-Gaussian random vector with parameter 1 (note this is because we have scaled $\A_i$ up by a factor of $\sqrt{t}$). $\M^\star$ is rank $r$, and we let $\X$ be the left singular vector of $\M^\star$, and assume $\X$ is $\mu$-incoherent\footnote{Note that for our particular problem this is not an additional assumption since by \cref{lem:diverse_to_incoh} our task assumptions imply this.}, i.e. $\max_{i}\norm{\e_i\trans \X}^2 \le \mu r/t$.

We now reformulate the objective (denoting $\M = \U\V\trans$) as
\begin{equation}\label{eq:objective_reformed}
f(\U, \V) = 2 (\M - \M^\star):\H_0:(\M - \M^\star) + \frac{1}{2} \fnorm{\U\trans \U - \V\trans \V}^2 + Q(\U)
\end{equation}
where $\M:\H_0:\M = \frac{1}{n}\sum_{i=1}^n \la \A_i, \M \ra^2$ and $\E [\M:\H_0:\M] = \fnorm{\M}^2$ and $Q$ is a regularization term:
\begin{equation}\label{eq:regularization}
Q(\U, \V) = \frac{2}{n} \sum_{i=1}^n[(\la \M-\M^\star,\A_i\ra - n_{i})^2 - (\la \M-\M^\star,\A_i\ra)^2]
\end{equation}

In this section, we denote $\tld = \max\{t, d\}$ and let $\sigstarl, \sigstarr$ be the $1$-st and $r$-th eigenvalue of matrix $\M^\star$. We denote $\cn^\star = \sigstarl/\sigstarr$ as its condition number.

The high-level idea of the analysis uses ideas from \citet{ge2017no}. The overall strategy is to argue that if we are currently not located at local minimum in the landscape we can certify this by inspecting the gradient or Hessian of $f(\U, \V)$ to exhibit a direction of local improvement $\Delta$ to decrease the function value of $f$. Intuitively this direction brings us close to the true underlying $(\U^\star, \V^\star)$.

We now establish some useful definitions and notation for the following analysis

\subsubsection{Definitions and Notation}

\begin{definition}
\label{def:asymmetricquantities}
Suppose $\M^\star$ is the optimal solution with SVD is $\X^\star\D^\star \Y^\star{}\trans$. Let $\U^\star = \X^\star (\D^\star)^{\frac{1}{2}}$, $\V^\star = \Y^\star (\D^\star)^{\frac{1}{2}}$. Let $\M = \U\V^\top$ be the current point in the landscape. We reduce the problem of studying an asymmetric matrix objective to the symmetric case using the following notational transformations:
\begin{equation}
\W = \begin{pmatrix}\U \\ \V\end{pmatrix}, 
\W^\star = \begin{pmatrix}\U^\star \\ \V^\star\end{pmatrix}, 
\N = \W\W\trans, 
\N^\star = \W^\star \W^\star {}\trans\label{eq:defwn}
\end{equation}
\end{definition}

We will also transform the Hessian operators to operate on $(t+d)\times r$ matrices. In particular, define the Hessians $\H_1, \G$ such that for all $\W$ we have:
\begin{align*}
 \N:\H_1:\N &= \M:\H_0:\M \\
 \N:\G:\N  &= \norm{\U\trans \U - \V\trans \V}_F^2
\end{align*}

Now, letting $Q(\W) = Q(\U,\V)$, we can rewrite the objective function $f(\W)$ as
\begin{equation}
\frac{1}{2}\left[(\N - \N^\star):4\H_1:(\N - \N^\star) + \N:\G:\N \right]+ Q(\W) \label{eq:a}
\end{equation}

We not introduce the definition of local alignment of two matrices.

\begin{definition}\label{def:delta} Given matrices $\W, \W^\star \in \mR^{d\times r}$, define their difference $\Delta = \W - \W^\star \R^\star$, where $\R^\star\in \mR^{r\times r}$ is chosen as $\mat{R}^\star = \argmin_{\mat{Z}^\top \mat{Z} = \mat{Z}\mat{Z}^\top = \I}\|\W-\W^\star\mat{Z}\|_F^2.$
\end{definition}

Note that this definition tries to ``align'' $\U$ and $\U^\star$ before taking their difference, and therefore is invariant under rotations. In particular, this definition has the nice property that as long as $\N = \W\W^\top$ is close to $\N^\star = \W^\star(\W^\star)^\top$ in Frobenius norm, the corresponding $\Delta$ between them is also small (see Lemma \ref{lem:bound}).

\subsubsection{Proofs for Landscape Analysis}
With these definitions in hand we can now proceed to the heart of the landscape analysis. Since $\W^\star$ has rotation invariance, in the following section, we always choose $\W^\star$ so that it aligns with the corresponding $\W$ according to Definition \ref{def:delta}.

We first restate a useful result from \citet{ge2017no},
\begin{lemma}[{\citep[Lemma 16]{ge2017no}}]\label{lem:asymmetricmain}
For the objective \eqref{eq:a}, let $\Delta, \N, \N^\star$ be defined as in Definition~\ref{def:asymmetricquantities}, Definition~\ref{def:delta}. Then, for any $\W\in \R^{(t + d)\times r}$, we have
\begin{align}
\Delta : \hess f(\W) :\Delta 
\le &\Delta\Delta\trans: \H :\Delta\Delta\trans - 3(\N - \N^\star):\H:(\N - \N^\star)  \nn \\
&+ 4\la \grad f(\W), \Delta\ra + [\Delta : \hess Q(\W) : \Delta - 4 \la \grad Q(\W), \Delta \ra] \label{eq:main_asym}
\end{align}
where $\H = 4\H_1+\G$. Further, if $\H_0$ satisfies $\M:\H_0:\M \in (1\pm \delta)\|\M\|_F^2$ for some matrix $\M = \U\V^\top$, let $\W$ and $\N$ be defined as in \eqref{eq:defwn}, then $\N:\H:\N \in (1\pm 2\delta)\|\N\|_F^2$.
\end{lemma}

With this result we show a key result which shows that enough sample all stationary points in the incoherence ball $\cW$ that are not close to $\W^{\star}$ have a direction of negative curvature.

\begin{lemma} \label{lem:step2_mc_asym}
If \cref{assump:design} holds, then when the number of samples $n \ge C \polylog(d,n,t) \mu^2 r^4 \max\{t, d\}  (\cn^\star)^4$ for large-enough constant $C$, with probability at least $1-1/\poly(d)$, all stationary points $\W \in \text{int}(\cW)$ satisfy:
\begin{equation*}
\Delta\Delta\trans:\H:\Delta\Delta\trans - 3(\N - \N^\star):\H:(\N - \N^\star) \le -0.1  \fnorm{\N - \N^\star}^2.
\end{equation*}
\end{lemma}
\begin{proof}
We divide the proof into two cases according to the norm of $\Delta$ and use different concentration inequalities in each case.
In this proof, we denote $\Delta = (\Delta_\U\trans, \Delta_\V\trans)\trans$, clearly, we have $\fnorm{\Delta_\U} \le \fnorm{\Delta}$ and  $\fnorm{\Delta_\V} \le \fnorm{\Delta}$.


\noindent\textbf{Case 1:} $\fnorm{\Delta}^2 \le \sigstarr/1000$. In this case, $\fnorm{\Delta_\U}^2  \le \fnorm{\Delta}^2 \le\sigstarr/1000$ and $\fnorm{\Delta_\V}^2  \le \fnorm{\Delta}^2 \le\sigstarr/1000$. By \eqref{eq:DD_concen}, we have
\begin{align*}
\Delta\Delta\trans: \H:\Delta\Delta\trans \le \fnorm{\Delta \Delta\trans}^2 + 0.004\sigstarr \fnorm{\Delta_\V}^2 \le 0.005 \sigstarr  \fnorm{\Delta}^2
\end{align*}
On the other hand, denote $\mS = \W^\star\Delta\trans + \Delta(\W^\star)\trans$, by \eqref{eq:DWstar_concen} and Lemma \ref{lem:asymmetricmain}, we know:
\begin{equation*}
\mS : \H: \mS \ge 0.999\fnorm{\mS}^2
\end{equation*}
Since we choose $\W^\star$ to alighn with the corresponding $\W$ according to Definition \ref{def:delta}, by \cref{lem:bound}.
\begin{align*}
\fnorm{\mS}^2 = 2(\fnorm{\Delta\trans \W^\star}^2+ \fnorm{\Delta (\W^\star)\trans}^2)
\ge 2\fnorm{\Delta (\W^\star)\trans}^2 \ge 2\sigstarr \fnorm{\Delta}^2
\end{align*}
This gives:
\begin{align*}
&\Delta\Delta\trans:\H:\Delta\Delta\trans - 3(\N - \N^\star):\H:(\N - \N^\star) \\
=& \Delta\Delta\trans:\H:\Delta\Delta\trans - 3(\mS + \Delta\Delta\trans):\H:(\mS+\Delta\Delta\trans) \\
\le& -6 \mS:\H:\Delta\Delta\trans - 3\mS:\H:\mS\\
\le &- \mS:\H:\mS - 2\sqrt{\mS:\H:\mS}(\sqrt{\mS:\H:\mS} - 3\sqrt{\Delta\Delta\trans :\H:\Delta\Delta\trans})\\
\le & -0.999\fnorm{\mS}^2 - 2\sqrt{\mS:\H:\mS} \cdot \sqrt{\sigstarr} \cdot(\fnorm{\Delta} - 0.3\fnorm{\Delta})
\le -0.999\fnorm{\mS}^2
\end{align*}
Finally, we know $\N - \N^\star = \mS + \Delta \Delta\trans$, and $\fnorm{\mS}^2 \ge 2\sigstarr \fnorm{\Delta}^2 \ge 500 \fnorm{\Delta}^4 = 500 \fnorm{\Delta \Delta\trans}^2$. Therefore:
\begin{equation*}
\fnorm{\N - \N^\star} \le \fnorm{\mS} + \fnorm{\Delta \Delta\trans} \le 2\fnorm{\mS}
\end{equation*}
This gives:
\begin{equation*}
\Delta\Delta\trans:\H:\Delta\Delta\trans - 3(\N - \N^\star):\H:(\N - \N^\star) \le -0.999\fnorm{\mS}^2 \le -0.1 \fnorm{\N - \N^\star}^2
\end{equation*}
~

\noindent\textbf{Case 2:} $\fnorm{\Delta}^2 \ge \sigstarr/1000$, by \eqref{eq:M_concen}, we have:
\begin{align*}
\frac{1}{n}\sum_{i=1}^n\la \A_i, \M - \M^\star\ra^2 
\ge& \fnorm{\M-\M^\star}^2 - (\sigstarr)^2 /10^{6} \ge \fnorm{\M-\M^\star}^2  - 0.001\sigstarr \fnorm{\Delta}^2
\end{align*}
This implies:
\begin{equation*}
(\N - \N^\star):\H:(\N - \N^\star) \ge \fnorm{\N-\N^\star}^2 - 0.004\sigstarr \fnorm{\Delta}^2
\end{equation*}
Then by \eqref{eq:DD_concen}, we have:
\begin{align*}
&\Delta\Delta\trans:\H:\Delta\Delta\trans - 3(\N - \N^\star):\H:(\N - \N^\star) \\
\le& \fnorm{\Delta\Delta\trans}^2 +0.004\sigstarr\fnorm{\Delta}^2 - 3(\fnorm{\N-\N^\star}^2 -0.004\sigstarr\fnorm{\Delta}^2) \\
\le& -\fnorm{\N-\N^\star}^2 + 0.016\sigstarr\fnorm{\Delta}^2
\le -0.1\fnorm{\N-\N^\star}^2
\end{align*}
where the last step follows by applying \cref{lem:bound}. This finishes the proof.
\end{proof}
With this key structural lemma in hand, we now present the main technical result for the section which characterizes the effect of the additive noise $n_i$ on the landscape.

\begin{theorem}\label{thm:main_landscape}
If \cref{assump:design} holds, when the number of samples $n \ge C \polylog(n,d,t) \mu^2 r^4 \max\{t, d\}  (\cn^\star)^4$ for large-enough constant $C$, with probability at least $1-1/\poly(d)$, we have that any local minimum $(\U, \V) \in \text{int}(\cW)$ of the objective \eqref{eq:objective} satisfies:
\begin{equation*}
\norm{\U\V^\top - \M^\star}_F\leq O(\sigma\sqrt{\frac{t\max\{t, d\} r\log n}{n}}).
\end{equation*}
\end{theorem}

\begin{proof} By \cref{lem:step2_mc_asym}, we know
$$
\Delta\Delta\trans:\H:\Delta\Delta\trans - 3(\N - \N^\star):\H:(\N - \N^\star) \le -0.1 \|\N-\N^\star\|_F^2.
$$
In order to use \cref{lem:asymmetricmain}, we bound the contribution from the noise term $Q$. Recall \eqref{eq:regularization}:
\begin{align*}
Q(\W)=&-\frac{4}{n}\sum_{i=1}^n (\la \M-\M^\star,\A_i\ra n_{i}) +\frac{2}{n}\sum_{i=1}^n(n_i)^2\\
\la \grad Q(\W), \Delta \ra=&-\frac{4}{n}\sum_{i=1}^n(\la \U\Delta_\V\trans + \Delta_\U\V\trans,\A_i\ra n_i)\\
\Delta : \hess Q(\W) :\Delta=&-\frac{8}{n}\sum_{i=1}^n (\la \Delta_\U\Delta_\V\trans,\A_i\ra n_i)
\end{align*}

Let $\B_i$ be the $(d_1+d_2)\times (d_1+d_2)$ matrix whose diagonal blocks are 0, and off diagonal blocks are equal to $\A_i$ and $\A_i^\top$ respectively. Then we have
\begin{align*}
&[\Delta : \hess Q(\W) : \Delta - 4 \la \grad Q(\W), \Delta \ra]\\
=& -\frac{8}{n}\sum_{i=1}^n (\la \Delta_\U\Delta_\V\trans,\A_i\ra n_i) + \frac{16}{n}\sum_{i=1}^n(\la \U\Delta_\V\trans + \Delta_\U\V\trans,\A_i\ra n_i)\\
=& \frac{24}{n}\sum_{i=1}^n (\la \Delta_\U\Delta_\V\trans,\A_i\ra n_i) + \frac{16}{n}\sum_{i=1}^n(\la \U^\star \Delta_\V\trans + \Delta_\U(\V^\star)\trans,\A_i\ra n_i)
\end{align*}
Now we can use \cref{lem:mc_noise} again to bound the noise terms: 
\begin{align*}
|\frac{24}{n}\sum_{i=1}^n (\la \Delta_\U\Delta_\V\trans,\A_i\ra n_i)|& \le O(\sigma\sqrt{\frac{t\max\{t, d\} r\log n}{n}})\sqrt{\fnorm{\Delta_\U\Delta_\V\trans}^2 + 0.001\sigstarr \fnorm{\Delta_\V}^2}\\
|\frac{16}{n}\sum_{i=1}^n(\la \U^\star \Delta_\V\trans + \Delta_\U(\V^\star)\trans,\A_i\ra n_i)| & \leq O(\sigma\sqrt{\frac{t\max\{t, d\} r\log n}{n}})\norm{\U^\star\Delta_\V\trans +\Delta_\U(\V^{\star})\trans}_F
\end{align*}
On one hand, by \cref{lem:bound}, we have:
\begin{equation*}
\fnorm{\Delta_\U\Delta_\V\trans}^2 + 0.001\sigstarr \fnorm{\Delta_\V}^2
\le \fnorm{\Delta\Delta\trans}^2 + 0.001\sigstarr \fnorm{\Delta}^2 \le 3\fnorm{\N - \N^\star}^2.
\end{equation*}
On the other hand, again by \cref{lem:bound}, we have:
\begin{equation*}
\norm{\U^\star\Delta_\V\trans +\Delta_\U(\V^{\star})\trans}^2_F \le \norm{\W^\star \Delta\trans  +\Delta(\W^{\star})\trans}^2_F
= 2 [\fnorm{\W^\star \Delta\trans }^2 + \fnorm{\Delta\trans  \W^\star }^2] \le 10 \fnorm{\N - \N^\star}^2
\end{equation*}
In sum, we have:
\begin{equation*}
[\Delta : \hess Q(\W) : \Delta - 4 \la \grad Q(\W), \Delta \ra] \le O(\sigma\sqrt{\frac{t\max\{t, d\} r\log n}{n}})\fnorm{\N - \N^\star}.
\end{equation*}

Therefore, by Lemma \ref{lem:asymmetricmain}, the Hessian at $\Delta$ direction is equal to:
\begin{align*}
\Delta : \hess f(\W) :\Delta
\leq &-0.1\norm{\N - \N^\star}_F^2
+O(\sigma\sqrt{\frac{t\max\{t, d\} r\log n}{n}})\fnorm{\N - \N^\star}.
\end{align*}
When the point further satisfies the second order optimality condition we have
\begin{align*}
\norm{\N-\N^\star}_F \leq O(\sigma\sqrt{\frac{t\max\{t, d\} r\log n}{n}}).
\end{align*}
In particular, $\M-\M^\star$ is a submatrix of $\N-\N^\star$, so $\norm{\M-\M^\star}_F\le O(\sigma\sqrt{\frac{t\max\{t, d\} r\log n}{n}})$.
\end{proof}

\subsection{Linear Algebra Lemmas} \label{sec:lemmas}

We collect several useful linear algebra lemmas here used in our analysis.

\begin{lemma}\label{lem:bound}
Given matrices $\W,\W^\star \in \mR^{d\times r}$, let $\N = \W\W^\top$ and $\N^\star = \W^\star(\W^\star)^\top$, and let $\Delta, \R^\star$ be defined as in Definition~\ref{def:delta}, and let $\tilde{\W}^\star = \W^\star \R^\star$then we have the followings properties:
\begin{enumerate}
\item $\W (\tilde{\W}^\star)\trans$ is a symmetric p.s.d. matrix;
\item $\|\Delta\Delta^\top\|_F^2 \le 2\|\N - \N^\star\|_F^2$;
\item $\sigstarr\|\Delta\|_F^2 \le \fnorm{\Delta(\tilde{\W}^\star)\trans}^2 \le \frac{1}{2(\sqrt{2}-1)}\|\N-\N^\star\|_F^2$.
\item $\fnorm{\Delta\trans \tilde{\W}^\star}^2 \le \|\N-\N^\star\|_F^2$
\end{enumerate}
\end{lemma} 

\begin{proof}
Statement 1 is in the proof of \citet[Lemma 6]{ge2017no}. Statement 2 is by \citet[Lemma 6]{ge2017no}.
Statement 3 \& 4 follow by Lemma \ref{lem:aux_deltalinear}.
\end{proof}

\begin{lemma} \label{lem:aux_deltalinear}
Let $\U$ and $\Y$ be $d \times r$ matrices such that $\U\trans\Y = \Y\trans \U$ is a p.s.d. matrix. Then,
\begin{align*}
\sigma_{\min}(\U\trans\U)\fnorm{\U - \Y}^2 \le \fnorm{(\U-\Y)\U\trans}^2 \le& \frac{1}{2(\sqrt{2}-1)}\fnorm{\U\U\trans - \Y\Y\trans}^2\\
\fnorm{(\U-\Y)\trans\U}^2 \le& \fnorm{\U\U\trans - \Y\Y\trans}.
\end{align*}
\end{lemma}
\begin{proof}
For the first statement, the left inequality is immediate, so we only need to prove right inequality.
To prove this, we let $\Delta = \U - \Y$, and expand:
\begin{align*}
\norm{\U\U\trans - \Y\Y\trans}_F^2  =& \norm{\U\Delta\trans + \Delta\U\trans - \Delta\Delta\trans}_F^2 \\
=& \tr(2\U\trans\U\Delta\trans\Delta + (\Delta\trans\Delta)^2 + 2(\U\trans\Delta)^2 - 4\U\trans\Delta\Delta\trans \Delta) \\
=& \tr((4 - 2\sqrt{2})\U\trans (\U - \Delta) \Delta\trans\Delta + (\Delta\trans\Delta -\sqrt{2}\U\trans\Delta )^2 + 2(\sqrt{2} - 1)\U\trans\U\Delta\trans\Delta ) \\
\ge & \tr((4 - 2\sqrt{2})\U\trans\Y\Delta\trans\Delta + 2(\sqrt{2} - 1)\U\trans\U\Delta\trans\Delta) \ge 2(\sqrt{2} - 1)\fnorm{\U\Delta\trans}^2
\end{align*}
The last inequality follows since $\U\trans \Y$ is a p.s.d. matrix. For the second statement, again, we have:
\begin{align*}
\norm{\U\U\trans - \Y\Y\trans}_F^2  =& \norm{\U\Delta\trans + \Delta\U\trans - \Delta\Delta\trans}_F^2 \\
=& \tr(2\U\trans\U\Delta\trans\Delta + (\Delta\trans\Delta)^2 + 2(\U\trans\Delta)^2 - 4\U\trans\Delta\Delta\trans \Delta) \\
=& \tr(2\U\trans (\U - \Delta) \Delta\trans\Delta + (\Delta\trans\Delta -\U\trans\Delta )^2 + (\U\trans\Delta)^2 ) \\
\ge & \tr(2\U\trans\Y\Delta\trans\Delta + (\U\trans\Delta)^2) \ge \fnorm{\U\trans \Delta}^2
\end{align*}
where the last inequality follows since $\U\trans\Delta = \Delta\trans \U$.
\end{proof}

\subsection{Concentration Lemmas}

We need to show three concentration-style results for the landscape analysis. The first is a RIP condition for over matrices in the linear space $\cT = \{ \U_{\star} \X^\top + \Y \V_{\star}^\top | \X \in \mR^{t \times r}, \Y \in \mR^{d \times r} \}$ using matrix concentration. The second and third are coarse concentration results that exploit the rank $r$ structure of the underlying matrix $\M$ and are used in the two distinct regimes where the distance to optimality can be small or large. Also note that throughout we can assume a left-sided incoherence condition on the underlying matrix of the form $\max_{i \in [t]} \norm{\e_i^\top \U_{\star}}^2 \leq \frac{\mu r}{t}$ due to \cref{assump:task}.


We first present the RIP-style matrix concentration result which rests on an application of the matrix Bernstein inequality over a projected space. The proof has a similar flavor to results in \citet{recht2011simpler}. First we define a projection operator on the space of matrices as $\pt \Z = \pu \Z + \Z \pv - \pu \Z \pv$ where $\pu$ and $\pv$ are orthogonal projects onto the subspaces spanned by $U$ and $V$. While $\pu$ and $\pv$ are matrices, $\pt$ is a linear operator mapping matrices to matrices. Intuitively we wish to show that for all $\W \in \mR^{t \times d}$, that the observations matrices are approximately an isometry over the space of projected matrices w.h.p: $\sumton t(\langle \e_{t(i)} \x_i^\top, P_{\cT} \W \rangle^2 \approx \fnorm{P_{\cT} \W}^2 = \fnorm{\W}^2$. Explicitly, we define the action of the operator $\C_i = \A_i \A_i^\top$ where $\A_i = \sqrt{t} \x_i \e_j^\top$ as $\C_i(\M) = t \x_i \e_j^\top \langle \e_j \x_i^\top, \M \rangle$. 

Here we record a useful fact we will use in the sequel,
\begin{align*}
	& \sqrt{t} \pt(\x_i \e_j^\top) = \pu \e_i \x_j^\top + \e_i (\pv \x_j)^\top - (\pu \e_i)(\pv \x_j)^\top \implies \\
	& \fnorm{\pt (\x_i \e_j^\top}^2 = \langle \pt (\x_i \e_j^\top), \x_i \e_j \rangle = \norm{\pu \e_i}^2 \norm{\x_i}^2 + \norm{\e_i}^2 \norm{\pv \x_i}^2 - \norm{\pu \e_i}^2 \norm{\pv \x_j}^2 \leq \\
	& \norm{\pu \e_i}^2 \norm{\x_i}^2 + \norm{\pv \x_i}^2
\end{align*}
where the last inequality holds almost surely.

We now present the proof of the RIP-style concentration result.
\begin{lemma}\label{lem:rip_conc}
	Under \cref{assump:design,,assump:task} and the uniform task sampling model above,
	\begin{align*}
	\norm{\frac{1}{n}\sum_{i=1}^n P_{\cT} \A_i \A_i\trans P_{\cT} - P_{\cT}} \leq (\log(ndt)) \cdot O \left(\sqrt{\frac{\mu d r^2 + tr^2}{n}} + \frac{(\mu d r + r t) \log(tdn)}{n} \right)
	\end{align*}
	with probability at least $1-O(n^{-100})$, where $\mu = O(\bkappa)$.
\end{lemma}
\begin{proof}
Note that under the task assumption, \cref{lem:diverse_to_incoh} diversity implies incoherence of the matrix $\U^{\star}$ with incoherence parameter $\mu = O(\bkappa)$. 
First, note $\mE[\C_i(\M)] = \M$ so $\mE[\sumton P_{\cT} \A_i P_{\cT} - P_{\cT}] = 0$.
To apply the truncated version of the matrix bernstein inequality from \cref{lem:trunc_mb} we first compute a bound on the norms of each $\C_i$ to set the truncation level $R$. Note that $\norm{\pt \A_i \A_i \pt} = \fnorm{\pt(\x_i \e_j^\top}^2 \leq t \cdot O((\frac{\mu r}{t} \norm{\x_i}^2 + \norm{\pv \x_i}^2)$) using the fact the operator $\A_i$ is rank-one along with the \cref{lem:diverse_to_incoh} which shows task diversity implies incoherence with incoherence parameter $\bkappa$. Now exploiting Gaussianity of the design we have that Now $\norm{\x_i}^2 \leq O(d+\max(\sqrt{d \log(1/\delta)}, \log(1/\delta))) = O(d+\sqrt{d} \log(1/\delta))$ and $\norm{P_V \x_i}^2 \leq O(r + \sqrt{r} \log(1/\delta))$ with probability at least $1-2\delta$ using sub-exponential tail bounds and a union bound. Hence $\norm{P_{\cT} \A_i P_{\cT}}  \leq O(\mu r d +   \mu r \sqrt{d}\log(1/\delta)) + tr + t \sqrt{r} \log(1/\delta)) = O(\mu r d + tr + (\mu r \sqrt{d} +t \sqrt{r}) \log(1/\delta))$.

We can rearrange this statement to conclude that $\Pr[\norm{P_{\cT} \A_i \A_i^\top P_{\cT}}  \geq c_1 (\mu r d + tr) + x] \leq  \exp(-c_2 (\frac{x}{\mu r \sqrt{d} + t \sqrt{r}}))$ for some $c_1, c_2$. Define a truncation level $R = c_1 (\mu r d +rt) + K (\mu r \sqrt{d} + t \sqrt{r})$ for some $K$ to be chosen later. We can use the aforementioned tail bound to control $\norm{\mE[Z_i]-\mE[Z_i']} \leq \mE[Z_i \Ind[\norm{Z_i} \geq R]] \leq \int_{K (\mu r \sqrt{d} + t \sqrt{r})}^{\infty} \exp(-c_2 (\frac{x}{\mu r \sqrt{d} + t \sqrt{r}})) \leq O(\exp(-c K)  (\mu r \sqrt{d} + t \sqrt{r})) = \Delta$.

Now we consider the task of bounding the matrix variance term. The calculation is somewhat tedious but straightforward under our assumptions. We make use of the standard result that for two matrices $\X$ and $\Y$ that $\norm{\X-\Y} \leq \max(\norm{\X}, \norm{\Y})$.

It suffices to bound the operator norm $\norm{\E[\fnorm{\pt \A_i}^2 \pt \A_i (\pt \A_i)^\top}$. Using the calculation from the prequel and carefully cancelling terms we can see that, 
\begin{align*}
	& \norm{\mE[\fnorm{\pt \A_i}^2 \pt \A_i (\pt \A_i)^\top]} \leq \\ 
	& t^2 \norm{\mE[(\norm{\pu \e_i}^2 \norm{\x_i}^2 + \norm{\pv \x_i}^2 - \norm{\pu \e_i}^2 \norm{\pv \x_j}^2) \cdot(\norm{\pu \e_i}^2 \x_i \x_i^\top + \norm{\pv \x}^2 \e_i \e_i^\top - \norm{\pv \x_i}^2 \pu \e_i (\pu \e_i)^\top]} \\
	& \leq t^2 O(\norm{\mE[(\norm{\pu \e_i}^2 \norm{\x_i}^2 \norm{\pu \e_i}^2 \x_i \x_i^\top + (\norm{\pu \e_i}^2 \norm{\x_i}^2 \norm{\pv \x_i}^2 \e_i \e_i^\top}] + \norm{\pv \x_i}^4 \e_i \e_i^\top)
\end{align*}
 We show how to calculate these leading terms as the subleading terms can be shown to be lower-order by identical calculations. First note using the fact that $\mE[\norm{\pu \e_i}^2] \leq \frac{r}{t} \leq 1$, since $t \geq r$ by the task diversity assumption. Then $t^2 \cdot \norm{\mE[(\norm{\pu \e_i}^2 \norm{\x_i}^2 \norm{\pu \e_i}^2 \x_i \x_i^\top} \leq \norm{\mu r t \mE[\norm{\x_i}^2 \x_i \x_i^\top] \mE[\norm{\pu \e_i}^2]} \leq O(\mu r^2 d)$ appealing to the fact $\mE[\norm{\x}^2 \x \x^\top] \preceq O(\I_d)$ by \cref{lem:l4l2norm}. 
 
 Similarly, we have that, $t^2 \cdot \norm{\mE[\norm{\pu \e_i}^2 \norm{\x_i}^2 \norm{\pv \x_i}^2 \e_i \e_i^\top]} \leq \mu r \mE[\norm{\x_i}^2 \norm{\pv \x_i}^2] \leq \mu r^2 d$ using incoherence and by \cref{lem:l4l2norm}. Finally, we have that $t^2 \cdot O(\norm{\mE[ \norm{\pv \x_i}^4 \e_i \e_i^\top}) \leq O(t r^2)$. Hence we have that $\sigma^2 = n \cdot O(\mu r^2 d + t r^2)$.

Finally, we can assemble the previous two computations to conclude the result with appropriate choices of $R$ (parametrized through $K$) and $x$ by combining with \cref{lem:trunc_mb}. Let us choose $K = \frac{c_3}{c} (\log(n) + \log(d) + \log(t))$ for some sufficiently large $c_3$. In this case, we can choose $c_3$ such that $\Delta \leq O(\frac{ \mu r \sqrt{d} + t \sqrt{r}}{n^{10} d^{10} t^{10}}) \leq O(\frac{\mu}{n^{10} d^{8}})$. Similarly, our choice of truncation level becomes $R = O( \mu r d + tr + (\log n + \log d + \log t) (\mu r \sqrt{d} + t \sqrt{r})$. At this point we now choose $x = c_4 (\log n + \log d + \log t) \max(\sigma/\sqrt{n}, R/n)$ for sufficiently large $c_4$. For large enough $c_4$ we can guarantee that $x \geq 2 \Delta \implies x - \Delta \geq \frac{x}{2}$.

Hence combining these results together and applying \cref{lem:trunc_mb} we can provide the following upper bound on the desired quantity,
\begin{align*}
	\Pr[\norm{\sumton P_{\cT} \A_i P_{\cT} - P_{\cT}} \geq x] \leq O(d \exp(-c \cdot c_4 (\log n + \log d + \log t)) + O(n \sqrt{K} \exp(-c_3 (\log n + \log d + \log t)) \leq O((ndt)^{-100})
\end{align*}
by taking $c_3$ and $c_4$ sufficiently large, with $x = O((\log (ndt)) \left(\sqrt{\frac{\mu d r^2 + tr^2}{n}} +  \frac{(\mu r d + tr) + (\mu r \sqrt{d} + t \sqrt{r}) (\log(ndt)))}{n} \right)$.
\end{proof}

\begin{lemma}\label{lem:coarse_conc}
	Let the covariates $\x_i$ satisfy the design conditions in \cref{assump:design} in the uniform task sampling model. Then for all matrices $\M$ matrices that are of rank $2r$, we have uniformly that,
	\begin{align*}
	 \abs{ \frac{1}{n}\sum_{i=1}^n\la \A_i, \M\ra^2 - \fnorm{\M}^2} \leq O \left(\sqrt{\frac{\max(t, d)r}{n}} \cdot \sqrt{t} \max_i \norm{\e_i^\top \M} \fnorm{\M}  +\frac{\max(t, d)r}{n} \cdot t \max_i \norm{\e_i^\top \M}^2  \right) 
	 \end{align*}
	 with probability at least $1-(3000r )^{-10\max(t,d)r}$.
\end{lemma}
\begin{proof}
	Note that by rescaling it suffices to restrict attention to matrices $\M$ that are of rank $2r$ and have Frobenius norm $1$ (a set which we denote $\Gamma$). Applying \cref{lem:y_subexp}, we have that,
	 \begin{align*}
	 	\abs{\sumton t(\e_{t(i)}^\top \M \x_i)^2 - \norm{\M}_F^2} \leq O \left(\frac{1}{\sqrt{n}} \sqrt{\log(\frac{1}{\delta}}) + \frac{1}{n} \log(\frac{1}{\delta}) \right)
	 \end{align*}
	 for any fixed $\M \in \Gamma$ with probability at least $1-\delta$.
	 Now using \ref{prop:rankrcover} with $\epsilon = \frac{1}{1000}$ have that the set $\Gamma$ admits a cover $K$ of size at most $|K| = (3000r)^{(t+d+1)r}$. Now by choosing $\delta = (3000)^{-c (t+d+1)r}$ for a sufficiently large constant $c$ we can ensure that, 
	 \begin{align*}
	 	\abs{\sumton t(\e_{t(i)}^\top \M_j \x_i)^2 - \norm{\M_j}_F^2} \leq O \left(\frac{1}{\sqrt{n}} \sqrt{(\max(t, d) r} + \frac{1}{n} \max(t, d)r \right) \quad \forall \M_j \in K
	 \end{align*}
	 with probability at least $1-(3000r)^{-10\max(t,d)r}$ using a union bound. Now a straightforward Lipschitz continuity argument shows that since any $\M \in \Gamma$ can be written as $\M = \M_i + \epsilon a_i$ for $\M_i \in K$ and another $a_i \in \Gamma$, then $\sup_{\M \in \Gamma} \abs{\sumton t(\e_{t(i)}^\top \M \x_i)^2 - \norm{\M}_F^2}  \leq 2 (\sup_{\M_j \in K} \abs{\sumton t(\e_{t(i)}^\top \M_j \x_i)^2 - \norm{\M_j}_F^2})$ and hence the conclusion follows. Rescaling the result by $\fnorm
	 {\M}^2$ finishes the result.
\end{proof}

\begin{lemma}
	Let the covariates $\x_i$ satisfy the design condition in \cref{assump:design} in the uniform task sampling model. Then if $Y_i = t (\e_{t(i)}^\top \A \x_i)^2 - \fnorm{\A}^2$, $Y_i$ is a sub-exponential random variable, and
	 \begin{align*}
	 	\abs{\sumton t(\e_{t(i)}^\top \M \x_i)^2 - \norm{\M}_F^2} \leq O \left( \frac{\sqrt{t} \max_i \norm{\e_i^\top \M}_2 \fnorm{\M}}{\sqrt{n}} \sqrt{\log(\frac{1}{\delta})} + \frac{t \max_i \norm{\e_i^\top \M}^2}{n} \log(\frac{1}{\delta}) \right)
	 \end{align*}
	 for any fixed $\M$ with probability at least $1-\delta$.
	\label{lem:y_subexp}
\end{lemma}
\begin{proof}
	First note that under our assumptions $Y_i$, $\E[t(\e_{j}^\top \A \x_i)^2] = \norm{\A}_F^2$. To establish the result, we show the Bernstein condition holds with appropriate parameters. To do so, we bound for $k \geq 1$,
	\begin{align*}
		& \abs{\E[Y_i^k]} \leq t^{k} 2^{2k} \mE[(\e_j^\top \M_j \x_i)^{2k}] = t^{k} 2^{2k} \cdot \E[\norm{\e_j^\top \M_j}^{2k}] C^{2k} k! \leq (C')^{4k} k! \cdot \E[(t\norm{\e_j^\top \M}^2)^{k-1} \cdot (t \norm{\e_j^\top \M}^2)] \\
		& \leq (C'')^k k! (t \nu^2)^{k-2} (t\nu^2 \fnorm{\A}^2) = \frac{1}{2} k! (\underbrace{C'' t \nu^2}_{b})^{k-2} \cdot(\underbrace{C''^2 t\nu^2 \fnorm{\M}^2}_{\sigma^2})
	\end{align*}
	by introducing an independent copy of $Y$, using Jensen's inequality, and the inequality $(\frac{a+b}{2})^k \leq 2^{k-1} (a^k  + b^k)$ in the first inequality, and the sub-Gaussian moment bound $\E[Z^{2k}] \leq 2k \Gamma(k) C^{2k} \leq k! C^{2k}$ for universal constant $C$ which holds under our design assumptions. Hence directly applying the Bernstein inequality (see \citet[Proposition 2.9]{wainwright2019high} shows that,
	\begin{align*}
		\E[e^{\lambda \cdot Y_i}] \leq e^{\lambda^2 (\sqrt{2} \sigma)^2/2} \quad \forall \abs{\lambda} \leq \frac{1}{2b}
	\end{align*}
	Hence, using a standard sub-exponential tail bound we conclude that, 
	 \begin{align*}
	 	& \abs{\sumton t(\e_{t(i)}^\top \M \x_i)^2 - \norm{\M}_F^2} \leq O \left(\frac{\sigma}{\sqrt{n}} \sqrt{\log(\frac{1}{\delta}}) + \frac{b}{n} \log(\frac{1}{\delta}) \right) = \\
	 	& O \left( \frac{\sqrt{t} \max_i \norm{\e_i^\top \M}_2 \fnorm{\M}}{\sqrt{n}} \sqrt{\log(\frac{1}{\delta})} + \frac{t \max_i \norm{\e_i^\top \M}^2}{n} \log(\frac{1}{\delta}) \right)
	 \end{align*}
	 for any fixed $\A \in \Gamma$ with probability at least $1-\delta$.
\end{proof}

We now restate a simple covering lemma for rank-$O(r)$ matrices from \citet{candes2010tight}.
\begin{lemma}[Lemma 3.1 from \citet{candes2010tight}]
	Let $\Gamma$ be the set of matrices $\M \in \mR^{t \times d}$ that are of rank at most $r$ and have Frobenius norm equal to $1$. Then for any $\epsilon < 1$, there exists an $\epsilon$-net covering of $\Gamma$ in the Frobenius norm, $S$, which has cardinality at most $(\frac{9}{\epsilon})^{(t+d+1)r}$.
	\label{prop:rankrcover}
\end{lemma}

\begin{lemma}\label{lem:uniform_concentration}
Let \cref{assump:design,,assump:task} hold in the uniform task sampling model. 
When number of samples is greater than $n \ge C \polylog(d,n,t) \mu^2 r^4 \max\{t, d\}  (\cn^\star)^4$ with large-enough constant $C$, with at least $1-1/\poly(d)$ probability, we have following holds for all $(\U, \V) \in \cW$ simultanously:
\begin{align}
\frac{1}{n}\sum_{i=1}^n\la \U^\star \Delta_\V\trans + \Delta_\U(\V^\star)\trans,\A_i\ra^2  \in & (1\pm 0.001) \fnorm{\U^\star \Delta_\V\trans + \Delta_\U(\V^\star)\trans}^2\label{eq:DWstar_concen}\\
\frac{1}{n}\sum_{i=1}^n\la \A_i, \Delta_\U\Delta_\V\trans\ra^2 \le & \fnorm{\Delta_\U\Delta_\V \trans}^2 +  0.001 \sigstarr \fnorm{\Delta_\V}^2  \label{eq:DD_concen}\\
\frac{1}{n}\sum_{i=1}^n\la \A_i, \M - \M^\star\ra^2 \ge& \fnorm{\M-\M^\star}^2 - (\sigstarr)^2 /10^{6}\label{eq:M_concen}
\end{align}
where $\M = \U\V\trans$ and $\Delta_\U, \Delta_\V$ are defined as in Definition \ref{def:delta}. Here $\mu = O(\bkappa)$.
\end{lemma}

\begin{proof}
This result follows immediately by applying Lemma \ref{lem:rip_conc} to the first statement and Lemma \ref{lem:coarse_conc} to the following two statements using the definition of the incoherence ball $\cW$.
\end{proof}

\begin{lemma}\label{lem:mc_noise}
Suppose the set of matrices $\A_1,\A_2,...,\A_m$ satisfy the event in Lemma \ref{lem:uniform_concentration}, let $n_1,n_2,...,n_m$ be i.i.d. sub-gaussian random variables with variance parameter $t\sigma^2$, then with high probability for any $(\U, \V) \in \cW$, we have
\begin{align*}
|\frac{1}{n}\sum_{i=1}^n (\la \Delta_\U\Delta_\V\trans,\A_i\ra n_i)|& \le O(\sigma\sqrt{\frac{t\max\{t, d\} r\log n}{n}})\sqrt{\fnorm{\Delta_\U\Delta_\V\trans}^2 + 0.001\sigstarr \fnorm{\Delta_\V}^2}\\
|\frac{1}{n}\sum_{i=1}^n(\la \U^\star \Delta_\V\trans + \Delta_\U(\V^\star)\trans,\A_i\ra n_i)| & \leq O(\sigma\sqrt{\frac{t\max\{t, d\} r\log n}{n}})\norm{\U^\star\Delta_\V\trans +\Delta_\U(\V^{\star})\trans}_F
\end{align*}
\end{lemma}

\begin{proof}
Note since the left hand side of the expressions are linear in the matrices we can normalize to those of Frobenius norm 1. The proof of both statements is identical so we simply prove the second. 

Define $\delta = \fnorm{\U^\star \Delta_\V\trans + \Delta_\U(\V^\star)\trans}$ and $\M=\U^\star \Delta_\V\trans + \Delta_\U(\V^\star)\trans$ for convenience, which can be thought of as arbitrary rank-r matrices. Then let $S$ be an $\epsilon$-net for all rank-$r$ matrices with Frobenius norm 1; by \cref{prop:rankrcover} we have that $\log |S| \leq O(\max(t,d) r \log(\frac{1}{\epsilon}))$. We set $\epsilon=\frac{1}{n^3}$ so $\log(\frac{1}{\epsilon}) = O(\log n)$. Now for any matrix $\M \in S$ we have that $\frac{1}{n} \langle \A_i, \M \rangle$ is a sub-gaussian random variable with variance parameter at most $t \sigma^2 \frac{\delta^2}{n}$. Thus, using a sub-gaussian tail bound along with a union bound over the net shows that uniformly over the $\M \in S$,
\begin{align*}
	|\frac{1}{n}\sum_{i=1}^n \langle \M,\A_i\ra n_i)| & \leq O(\sigma \delta \sqrt{\frac{t\max\{t, d\} r\log n}{n}})
\end{align*}
with probability at least $1-\frac{1}{\poly(d)}$. We now show how to lift to the set of all $\M$. Note that with probability at least $1-e^{-\Omega(n^{1/4})}$ that $\norm{\n} = O(\sqrt{t} \sigma \sqrt{n})$ by a sub-gaussian tail bound. Let $\M$ be an arbitrary element, and $\M'$ its closest element in the cover; then we have that $\z_i = \langle \A_i, \M-\M' \rangle \leq \frac{\delta}{n^2}$ using the precondition on $\A_i$. 
Combining and using a union bound then shows that,
\begin{align*}
	& \abs{\sumton n_i \langle \A_i, \M \rangle } \leq  \abs{\sumton n_i \langle \A_i, \M' \rangle } + \abs{\sumton n_i \langle \A_i, \M-\M' \rangle } \leq O(\sigma \delta \sqrt{\frac{t\max\{t, d\} r\log n}{n}}) + \frac{\sqrt{t} \sigma \delta}{\sqrt{n}}\leq \\
	& O(\sigma \delta \sqrt{\frac{t \max(t, d) r \log n}{n}})
\end{align*}
Rescaling and recalling the definition of $\delta$ gives the result. 
\end{proof}

\subsection{Task Diversity for the Landscape Analysis}
Here we collect several useful results for interpreting the results of the landscape analysis. Throughout this section we use the notation $\U \in \mR^{t \times r}$ and $\V \in \mR^{d \times r}$.

The first result allow us to convert a guarantee on error in Frobenius norm to a guarantee in angular distance, assuming an appropriate diversity condition on $\U$.

\begin{lemma}
Suppose $\V$ and $\hat{\V}$ are orthonormal projection matrices, that is $\V\trans \V = \I_r$, and $\hat{\V}\trans \hat{\V} = \I_r$. Then, for any $\epsilon>0$, if $\fnorm{\hat{\U}\hat{\V}\trans - \U\V\trans}^2 \le \epsilon$ for some $\hat{\U}$ and $\U$, then:
\begin{equation*}
\mathrm{dist}^2(\V, \hat{\V}) \le \frac{\epsilon}{\nu t}
\end{equation*}
where $\nu = \sigma_r(\U\trans \U)/t$.
\label{lem:frob_to_angle}
\end{lemma}

Here distance function is sine function of the principle angle, i.e.
\begin{equation*}
\mathrm{dist}(\V, \hat{\V}) := \norm{\V\trans \hat{\V}_\perp}.
\end{equation*}
and $\nu = \sigma_r(\U\trans \U)/t$ represents an analog of the task diversity matrix.

\begin{proof}
Let function $f(\tilde{\U}) = \fnorm{\tilde{\U}\hat{\V}\trans - \U\V\trans}^2$.
The precondition of the theorem states that there exists $\hat{\U}$ so that $\fnorm{\hat{\U}\hat{\V}\trans - \U\V\trans}^2 \le \epsilon$. This clearly implies the following:
\begin{equation} \label{eq:minimal_solution}
\min_{\tilde{\U}} f(\tilde{\U}) \le \epsilon
\end{equation}
Setting the gradient $\dd f/ \dd \tilde{\U} = 0$, we have the minimizer $\tilde{\U}^\star$ satisfies:
\begin{equation*}
(\tilde{\U}^\star \hat{\V}\trans - \U \V\trans)  \hat{\V} = 0
\end{equation*}
which gives:
\begin{equation*}
\tilde{\U}^\star = \U \V\trans \hat{\V}.
\end{equation*}
Plugging this back to Eq.\eqref{eq:minimal_solution}, gives:
\begin{equation*}
\fnorm{\U\V\trans(\hat{\V}\hat{\V}\trans - \I)}^2 \le \epsilon.
\end{equation*}
Finally, we have:
\begin{align*}
\fnorm{\U\V\trans(\hat{\V}\hat{\V}\trans - \I)}^2 = &\fnorm{\U\V\trans\hat{\V}_\perp\hat{\V}_\perp\trans}^2
= \fnorm{\U\V\trans\hat{\V}_\perp}^2 = \tr(\U\trans\U\V\trans\hat{\V}_\perp\hat{\V}_\perp\trans \V)\\
\ge & \sigma_{r}(\U\trans\U) \fnorm{\V\trans\hat{\V}_\perp}^2
\ge \sigma_{r}(\U\trans\U) \norm{\V\trans\hat{\V}_\perp}^2
\end{align*}
The second last inequality follow since  for any p.s.d. matrices $\A$ and $\B$, we have $\tr(\A\B) \ge \sigma_{\min}(\A) \tr(\B)$.
This concludes the proof.
\end{proof}

For the following let $\A = (\balpha_1, \cdots, \balpha_t)\trans \in \mR^{t\times r}$ and denote the SVD of $\A = \U \mSigma \V\trans$. Next we remark that our assumptions on task diversity and normalization implicit in the matrix $\A$ are sufficient to actually imply an incoherence condition on $\U$ (which is used in the matrix sensing/completion style analysis). 

\begin{lemma}
If $\sigma_r(\A\trans \A)/t \ge 1/(\mu r)$ and $\max_{i\in[t]} \norm{\balpha_i}^2 \le C$, then we have:
\begin{equation*}
\max_{i\in[t]} \norm{\e_i\trans \U}^2 \le \frac{C\mu r}{ t}
\end{equation*}
\label{lem:diverse_to_incoh}
\end{lemma}
\begin{proof}
Since $\max_{i\in[t]} \norm{\balpha_i}^2 \le C $, we have, for any $i\in [t]$
\begin{equation*}
C \ge \norm{\balpha_i}^2 =\norm{\e_i\trans \A}^2 = \norm{\e_i\trans \U\mSigma}^2
\ge \norm{\e_i\trans \U}^2 \sigma_{\min}^2(\mSigma) = \norm{\e_i\trans \U}^2 \sigma_{r}(\A\trans \A)
\ge (t/\mu r) \norm{\e_i\trans \U}^2
\end{equation*}
which finishes the proof. Note in the context of \cref{assump:task} the incoherence parameters corresponds to the parameter $\bkappa$.
\end{proof}


==> icml/app_lb.tex <==
%!TEX root = main.tex

\section{Proofs in \cref{sec:lf_lb}}

We begin by presenting the proof of the main statistical lower bound for recovering the feature matrix $\B$ and relevant auxiliary results. Following this we provide relevant background on Grassmann manifolds and the details of the volumetric computations in the Grassmann manifold which are necessary to establish the packing bounds for our minimax lower bound.

As mentioned in the main text our main tool is to use the  Fano method (\cref{prop:fano}) along with suitable bounds on the cardinality of the packing number $M$ and the mutual information $I(Z;J)$, we can state an asymptotic (i.e. $d \to \infty$) minimax lower bound on the difficulty of estimating $\B$. 


\begin{proof}[Proof of \cref{thm:feature_lb}]
	Our goal to apply the Fano method will be to combine our upper bound on the mutual information with the lower bounds on the local packing number in $G_{r,n}(\mR)$. For our present purposes we simply take $\Phi(\cdot)$ to be the identity function in \cref{prop:fano}. Note that \cref{cor:local_packing} establishes the existence of a $2\delta_1$-separated set contained in a ball of diameter $4 \delta_2 < 1$, with cardinality at least $\log M \geq \frac{dr}{2} \log(2 \delta_2/\delta_1)$ for $d \geq d_0(\delta_1, \delta_2, r)$. Similarly, in the setting of the theorem and the aforementioned local packing, \cref{lem:mut_info} ensures $I(Z; J) \leq 16 \delta_2^2 n$. 
	
		We now fix $\delta_1=\delta_2=\delta$ and set $\delta$ to an appropriate constant, to guarantee $\frac{I(Z;J)+\log 2}{\log M} \leq \frac{1}{2}$, recalling that we must have $4 \delta < 1$. Using the aforementioned bounds we find,
		\begin{align*}
			\frac{I(Z;J)+\log 2}{\log M} \leq \frac{16 \delta^2 n + \log 2}{\frac{dr}{2} \log 2} \leq \frac{1}{2}
		\end{align*}
		where the last inequality follows by taking $d$ sufficiently large to ensure that $\frac{2}{dr} \leq \frac{1}{100}$ and choosing $\delta^2$ such that $\frac{32 \delta^2 n}{dr} = 32 \delta^2 k = \frac{98}{100}$ -- which requires $ \delta = \frac{7}{40 \sqrt{k}}$. Finally, the constraint $ 4\delta <1$ requires $k > 100/49$.
		\end{proof}



To implement the Fano method requires an upper bound on the mutual information. 
\begin{lemma}
		\label{lem:mut_info}
	Suppose $n$ data samples $(\x_i, y_i)$ are generated from the model in \eqref{eq:model_main} with i.i.d. covariates $\x_i \sim \cN(0, \I_d)$ and independent i.i.d. noise $\epsilon_i \sim \cN(0,1)$. Further, assume the task parameters satisfy \cref{assump:task} with each task normalized to $\norm{\balpha_i}=1$ and $\nu \geq \Omega(1)$. Let $\{ \B^{1}, \hdots, \B^{M} \}$ be a $2\delta$-separated set contained within a ball of diameter $4 \delta < 1$, with distance measured in the subspace angle distance on $\Gr$. Then the mutual information $I(Z;J)$ from the setting of \cref{prop:fano} satisfies,
	\begin{align*}
		I(Z; J) \leq 16 \delta^2 n. 
	\end{align*}
\end{lemma}
\begin{proof}
	We begin by using a standard relaxation of the mutual information which exploits joint convexity of the KL-divergence to conclude,
	\begin{align*}
		I(Z;J) \leq \frac{1}{M^2} \sum_{i,j}\KL(\Pr_{\B^{i}}, \Pr_{\B^{j}}).
	\end{align*}
We now proceed to uniformly bound each KL-term. Now the joint distribution over the observations for each measure $\Pr_{\B_{1}^{i}}$ can be written as $\Pr_{\B^{i}} \equiv \Pi_{t=1}^{T} p(\X_t) p(\y|\X_t, \B^{i}, \balpha_t)$ where $p(\X_t)$ corresponds to the density of the Gaussian design matrix, and $p(\y|\X_t, \B^{i}, \balpha_t)$ the Gaussian conditionals of the observations $\y$.
	So using standard properties of the KL-divergence we find that,
	\begin{align*}
		& \KL(\Pr_{\B^{i}}, \Pr_{\B^{j}}) = \sum_{t=1}^{T} \frac{1}{2} \mE_{\X_t} \left ( \norm{\X_t \B^{i} \balpha_t - \X_t \B^{j} \balpha_t}^2 \right) = \sum_{t=1}^{T} \frac{n_t}{2} \norm{\B^{i} \balpha_t - \B^{j}\balpha_t}^2 = \sum_{t=1}^T n_t \cdot  (\norm{\balpha_t}^2 - \balpha_t^\top (\B^{i})^\top \B^{j} \balpha_t) \leq \\
		& \sum_{t=1}^{T} n_t \balpha_t^\top (\I_r - (\B^{i})^\top \B^{j}) \balpha_t \leq \sum_{t=1}^T n_t \norm{\balpha_t}^2 \sigma_{\max}(\I_r-(\B^{i})^\top \B^{j}) = \sum_{t=1}^T n_t \norm{\balpha_t}^2 (1-\sigma_{k}( (\B^{i})^\top \B^{j}))
	\end{align*}
	Recognizing $\sigma_{k}( (\B^{i})^\top \B^{j}) = \cos \theta(\B^{i}, \B^{j})$ and $\norm{(\B_{\perp}^{i})^\top \B^{j}} = \sin \theta$, where $\theta$ is $k$th principal angle between the subspaces, we have that $1-\sigma_{k}( (\B^{i})^\top \B^{j}) = 1-\sqrt{1-\norm{(\B_{\perp}^{i})^\top \B^{j}}^2} \leq 1-\sqrt{1-16\delta^2}$, using the uniform upper bound on the diameter of the set in which the $\B^{i}$ are contained. Finally using the elementary inequality $1-\sqrt{1-16\delta^2} \leq 16 \delta^2$ for $0 \leq \delta \leq \frac{1}{4}$ concludes the proof, where we have defined $n = \sum_{t=1}^{T} n_t$.
\end{proof}

\subsection{Packing bounds in $\Gr$}

Before beginning we establish several pieces of notation relevant to discussion. We denote the Grassmann manifold, which consist of the the set of $r$-dimensional subspaces within the underlying $d$-dimensional space, as $\Gr$. Another way to define it is as the homogeneous space of the orthogonal group $O(d)$ in the sense that,
	\begin{align*}
		\Gr \cong O(d)/(O(r) \times O(d-r))	
	\end{align*}
	which defines its geometric structure. The underlying measure on the manifold $G_{r, n}(\mR)$ is the associated, normalized invariant (or Haar) measure.

 Note that each orthonormal feature matrix $\B$, is contained in an equivalence class (under orthogonal rotation) of an element in $\Gr$. To define distance in $\Gr$ we define the notion of a principal angle between two subspaces $p$ and $q$. If $\C$ is an orthonormal matrix whose columns form orthonormal basis of $p$ and $\D$ is an orthonormal matrix whose columns form an orthonormal basis of $q$, then singular value of decomposition of $\C^\top \D = \U \D \V^\top$ defines the principal angles as,
\begin{align*}
	\D = \diag(\cos \theta_1, \cos \theta_2, \hdots, \cos \theta_k)
\end{align*}
where $0 \leq \theta_k \leq \hdots \leq \theta_1 \leq \frac{\pi}{2}$. As shorthand we let $\btheta = (\theta_1, \theta_2, \hdots, \theta_k)$, and let $\sin$ and $\cos$ act element-wise on its components. Two distances of interest for us will be the induced $\ell_2$ and $\ell_{\infty}$ norms on the vector $\theta$. That is the \textit{chordal} distance $d_{c}(p, q) = \norm{\sin \btheta}_2$ and the \textit{subspace angle} distance $d_{m}(p, q) = \norm{\sin \btheta}_{\infty}$.  We refer the reader to \citet{barg2002bounds} for geometric background on coding and packing/covering bounds in the context of Grassmann manifolds relevant to our discussion here.

The key result to apply the (local) Fano method is an asymptotic estimate of the volume of radius $\delta$ ball (in the \textit{max-sin} distance). With such a result standard Hamming and Gilbert-Varshamov bounds can be used to show the existence of codes as well as sufficiently large local packings in $\Gr$. 
In order show this lemma we adapt techniques from  \citet{barg2002bounds} which establish bounds on the packing of spheres in $\Gr$ in the \textit{chordal} distance on the manifold. Note that our interest is in packings with respect to the \textit{subspace angle} distance. The proof strategy is to write down the volume of a ball in $\Gr$ in angular coordinates and asymptotically evaluate the integral.

\begin{lemma}
	Let $\delta < 1$ and let $B(\delta)$ be the ball of radius $\delta$ (with respect to the subspace angle distance) in $\Gr$. For fixed $\delta, r$, as $d \to \infty$,
	\begin{align*}
			\vol(B(\delta)) =  (\delta)^{d r + o_{\delta, r}(d)}.
	\end{align*}
	\label{thm:ball_vol}
\end{lemma}
\begin{proof}
	We begin by writing down the expression for the volume of set $\Theta$ in the angular coordinates $\theta_1 \leq \theta_2 \leq \hdots \theta_r$ (the expression for the volume form can be found in \citet[Eq. 11]{barg2002bounds}). We have that, $\vol(B(\delta)) = \frac{J_r}{K(r, d)}$ with $K(r, d) = \Pi_{i=1}^{r} \frac{A(r-i+1)^2 A(d-r-i+1)}{2 A(d-i+1)}$ where $A(r) = \frac{2\pi^{r/2}}{\Gamma(r/2)}$. The expression for $J_r$ is given by the angular integral,
	\begin{align*}
			& J_r = \int_{S} \Pi_{i=1}^{r} (\sin \theta_i)^{d-2r} \cdot \Pi_{1 \leq i < j \leq r} (\sin^2 \theta_i - \sin^2 \theta_j) \theta_1 \wedge \hdots \wedge d \theta_r
			=
			\\
			& \int_{0 \leq x_1 < \hdots < x_r < 1 \cap S} \frac{(x_1 x_2 \hdots x_r)^{d-2r} \Pi_{i < j} (x_i^2-x_j^2)}{\sqrt{(1-x_1^2)(1-x_2^2) \hdots (1-x_r^2)}} dx_1 \wedge \hdots \wedge dx_r,
	\end{align*}
	where $x_i = \sin \theta_i$.
	Note that since $K(r,d)$ grows polynomially in $d$ for fixed $r$, and we are interested in the logarithmic asymptotics of the expression its exact form will not affect the result. 

Our present concern will be to compute this integral over the set $S = \{ \x : \norm{\x}_\infty \leq \delta \}$, whereas the result of \citet[Theorem 1]{barg2002bounds} estimates the volume over the set $\{ \x : \norm{\x}_2 \leq \delta \}$. For convenience we let $\Omega = S \cap \{ \x : 0 < x_1 < \hdots < x_r < 1 \}$.
	To asymptotically evaluate this expression we use a rigorous, multidimensional formulation of the Laplace method from \citet[Theorem 5, p. 131]{fedoryuk1987asymptotics} which is restated and used in \citet[Theorem 3]{barg2002bounds}. We refer the reader to \cref{thm:laplace} for the formal statement.
	
	To use this result we have that the expansion parameter is $\lambda=d$, with $S(\x) = \sum_{i=1}^r \ln(x_i)$ and
	\begin{align*}
		f(\x) = \left( \Pi_{i=1}^r x_i^{-2r} (1-x_i^2)^{-1/2} \right) \Pi_{i < j} (x_i^2-x_j^2)
	\end{align*}
	with the integration domain $\Omega$ defined above. The maximum of $S(\x)$ over $\Omega$ is attained at $\xstar = (\delta, \hdots, \delta)$ as we can verify by the KKT conditions since the optimization in the variable $\x$ is of a convex function over a convex set. 
	To satisfy the technical conditions in the theorem, the integration domain needs to be slightly adjusted. The modifications are similar to those in \citet{barg2002bounds}. First note that $S(x)$ has discontinuities at the hyperplanes $x_i=0$ and $f(x)$ has discontinuities at the hyperplanes $x_i=1$ -- so we shift the domain from these regions in a manner that doesn't affect the conclusion. Similarly, at the point $\xstar$ the boundary $\partial \Omega$ is not differentiable so we extend the domain of integration to include a small spherical cap encapsulating the boundary point $\xstar$. Formally, we let $\Omega_{\epsilon} = \Omega \cup \{ \x : \norm{\x}_2 \leq \delta \sqrt{k}, \langle \frac{\x}{\norm{\x}}, \frac{(1, \hdots, 1)}{\sqrt{k}} \rangle \leq \epsilon \} \cap \{ \x : \epsilon \leq x_i \leq 1-\epsilon \}$. In the limit of small $\epsilon$, the volume difference computed in the coordinates $\theta_1, \hdots, \theta_k$, is $\vol(\Theta \slash \Theta_{\epsilon}) + \vol(\Theta_{\epsilon} \slash \Theta) = O(\epsilon)$, since the integrand in the $\btheta$ coordinates is bounded by 1. This implies the integral of $J_r$ differs from the corresponding integral over $\Omega_{\epsilon}$ by $O(\epsilon)$ uniformly in $n$.
		
		We can now verify the conditions needed to apply the theorem.
	\begin{itemize}
		\item For the first condition, the interior normal to the spherical cap on the boundary $\partial \Omega_{\epsilon}$ has the form $n \propto -(1, \hdots, 1)$. Moreover the level surfaces of $S(\x)$ are given by $\Pi_{i=1}^r x_i = constant$, which are convex hypersurfaces and homothetic to each other with respect to the origin. Hence, we can conclude $S(\x)$ strictly increases along the diagonal $x_1=x_2=\hdots=x_k$.
		\item In the basis $(x_1, \hdots, x_r)$ the Hessian $H(\x) = \frac{\partial^2 S(\x)}{\partial x_i \partial x_j}$ has the form $-\diag(x_1^{-2}, \hdots x_r^{-2})$, and so $H(\xstar) = -\delta^2 \I_k$ which is a negative-definite quadratic form. Evidently, $H$ remains negative-definite under restriction to the tangent space $(\xi_1, \hdots, \xi_{r-1})$.
		\item Smoothness in the neighborhood of $\xstar$ follows immediately from the definitions of the functions.
	\end{itemize}
		Noting that $f(\xstar) = 0$ and applying the theorem to $J_r$ we obtain that,
		\begin{align*}
			J_r = d^{-(r+1)/2} (\delta)^{rd} \cdot O(d^{-1}) \implies \log J_r = rd \cdot \ln(\delta) + o(d) = (rd+o(d)) \ln(\delta) 
		\end{align*}
		since $\ln(\delta)$ is constant in the limit $d \to \infty$; note the error estimate may depend implicitly on $\delta$ and $r$ (which are treated as constant). Finally, to finish the volume computation we analyze the logarithmic asymptotics of the normalizer,
	\begin{align*}
			\ln K(r, d) = \sum_{i=1}^{r} 2 \ln A(r-i+1) + \ln A(d-r+i+1) - \ln A(d-i+1) - \ln 2
	\end{align*}
	However, now $\log A(x) = \frac{x}{2} \log \pi + \log 2 - \log \Gamma(x/2)$, and $\ln \Gamma(z) = z \ln z - z + \frac{1}{2} \ln z + \frac{1}{2} \ln (2 \pi) + o(1)$ as $z \to \infty$. Since in the argument $r$ is thought of as constant as $d \to \infty$ we have that, 
	\begin{align*}
		& \ln K(r,d) = \sum_{i=1}^r O(1) + (d-r+i+1) \ln(d-r+i+1) - (d-r+i+1) + \frac{1}{2} \\
		& - (d-i+1) \ln (d-i+1) + d-i+1 +\frac{1}{2} \ln(d-i+1) = \sum_{i=1}^r o(d) = o(d).
	\end{align*}
	since for the dominant terms $d \ln(d-r+i+1)-d -d \ln(d-i+1)+d= o(1)$, and other terms are of logarithmic order in $d$. Combining this estimate with the expression for $\log J_r$ gives the result.

\end{proof}
With the aforementioned result in hand, we can easily establish a lower bound on the size of a local packing in $G_{r,n}(\mR)$.

\begin{corollary}
	\label{cor:local_packing}
	Fix $r \geq 2$, $2\delta_1 < 4\delta_2 < 1$, and assume distance is measured with respect to the subspace angle distance in the underlying space $\Gr$. Then for sufficiently large $d$, there exists a $2\delta_1$-separated set $\{ \B^{1}, \hdots, \B^{M} \}$ such that each of element of the set is strictly contained in a ball of radius $4\delta_2$, $B(\delta_2) \subset \Gr$ such that,
	\begin{align*}
	\log M \geq \frac{dr}{2} \log(\frac{2\delta_2}{\delta_1})
	\end{align*}	
\end{corollary}
\begin{proof}
		First note that by the duality between packing and covering numbers we have that $\log M \geq \log N$ where $N$ denotes the covering number of the ball of radius $4\delta_2$ with balls of size $2 \delta_1$ (see for example \citet[Lemma 5.5]{wainwright2019high}). Now we adapt a standard volume covering argument to obtain the result. Note that if $\{ \B^{1}, \hdots, \B^{M} \}$ is a $2\delta_1$-covering of $B(4\delta_2)$, then it must be that $\vol(B(4\delta_2)) \leq N \vol(B(2 \delta_1))$. Now we use our approximate estimates of the volume of balls in $\Gr$ from \cref{thm:ball_vol}, to show that $\vol(B(4\delta_2)) \geq (4\delta_2)^{dr+o(d)}$ and $\vol(B(2 \delta_1)) \leq (2 \delta_1)^{dr+o(d)}$. Hence $\log N \geq dr \log(\frac{2\delta_2}{\delta_1}) + o(d) \cdot \log(\frac{2\delta_2}{\delta_1})$. Note that for sufficiently large $d > d_0(\delta_1, \delta_2, r)$, $dr \log(\frac{2\delta_2}{\delta_1}) + o(d) \cdot \log(\frac{2\delta_2}{\delta_1}) \geq \frac{dr}{2} \log(\frac{2\delta_2}{\delta_1})$, since we can ensure $o(d) \geq -\frac{d}{100}$. This concludes the proof.
\end{proof}

Finally for convenience, we restate the rigorous version of the Laplace method we use which is also restated in \citet[Theorem 3]{barg2002bounds}
\begin{theorem}\citet[p.131]{fedoryuk1987asymptotics}
Let $\Omega$ be a connected open domain in $\mR^r$, $\partial \Omega$ be its boundary, and $[\Omega] = \Omega \cup \partial \Omega$, and let $f \in C([\Omega])$ be real functions. Further, suppose that the maximum $\max_{x \in [\Omega]} S(x)$ is attained only at the  point $\xstar \in \partial \Omega$, and at this point
	\begin{itemize}
		\item $\frac{\partial S(\xstar)}{\partial \vec{n}} \neq 0$, where $\partial/\partial \vec{n}$ is differentiation along the interior normal to $\partial \Omega$ at $\xstar$.
		\item The Hessian matrix,
		\begin{align*}
			H = \left( \frac{\partial^2 S(\xstar)}{\partial \xi_i \partial \xi_j} \right)_{i,j=1}^{r-1}	
		\end{align*}
		is negative-definite, where $(\xi_1, \hdots, \xi_{r-1})$ is an orthonormal basis in the tangent space $T_{\xstar} \partial \Omega$ to $\partial \Omega$ at $\xstar$.
		\item $f, S \in C^{\infty}$ in the neighborhood of $\xstar$.
	\end{itemize}
	Then,
	\begin{align*}
		\int_{\Omega} f(x) e^{\lambda S(x)} = \lambda^{-(r+1)/2} e^{\lambda S(\xstar)} \sum_{m=0}^{\infty} a_m \lambda^{-m} \quad (\lambda \to \infty)	
	\end{align*}
	for some constants $a_m$. Moreover, $a_0$ is proportional to $f(\xstar)$.
\label{thm:laplace}
\end{theorem}



==> icml/app_train_mom.tex <==
%!TEX root = main.tex
\textbf{Notation and Set-up}
We first establish several useful pieces of notation used throughout the Appendices. We will say that a mean-zero random variable $x$ is sub-gaussian, $x \sim \sG(\kappa)$, if $\E[\exp(\lambda x))] \leq \exp(\frac{\kappa^2 \lambda^2}{2})$ for all $\lambda$. We will say that a mean-zero random variable $x$ is sub-exponential, $x \sim \sE(\nu, \alpha)$, if $\E[\exp(\lambda x)] \leq \exp(\frac{\nu^2 \lambda^2}{2})$ for all $\abs{\lambda} \leq \frac{1}{\alpha}$. We will say that a mean-zero random vector is sub-gaussian, $\x \sim \sG(\kappa)$, if $\forall \v \in \mathbb{R}^p$, $\E[\exp(\v^\top \x)] \leq \exp(\frac{\kappa^2 \Vert \v \Vert_2^2}{2})$. Moreover a standard Chernoff argument shows if $x \sim \sE(\nu, \alpha)$ then $\Pr[\abs{x} \geq t] \leq 2 \exp(-\frac{1}{2} \min(\frac{t^2}{\nu^2}, \frac{t}{\alpha}))$. Throughout we will use $c,C$ to refer to universal constants that may change from line to line. 
\\
\section{Proofs in \cref{sec:prelim}}
\label{app:prelim}
Here we provide a formal statement of \cref{thm:main_informal}. 

\begin{theorem}[Formal statement of \cref{thm:main_informal}]
	Suppose we are given $n_1$ total samples from \cref{eq:model_main} which satisfy \cref{assump:design}, with an equal number of samples from each task, which collectively satisfy \cref{assump:task}, and $n_2$ samples also from \cref{eq:model_main}, satisfying \cref{assump:design}, but from a $t+1$st task which satisfies $\norm{\balpha_{t+1}}^2 \leq O(1)$. Then, if the $n_1$ samples are used in \cref{algo:LF_learn} to learn a feature representation $\Bone$, which is used in \cref{algo:LF_newtask} along with the $n_2$ samples to learn $\halpha$, and $n_1 \gtrsim \polylog(d, n_1) \frac{\bkappa dr}{\nu}$, and $n_2 \gtrsim r \log n_2$ the excess prediction error on a new datapoint drawn from the covariate distribution (i.e., $\xstar \sim \cN(0, 1)$), is,
	\begin{align*}
		\mE_{\xstar}[\langle \xstar, \Bone \halpha - \B \balpha_{t+1} \rangle^2] \leq \tlO \left(\frac{\bkappa dr}{\nu n_1}+\frac{r}{n_2} \right)
		 \label{eq:main}
	\end{align*}
	with probability at least $1-O(n_1^{-100}+n_2^{-100})$.
	\label{thm:main_formal}
\end{theorem}
\begin{proof}
	Note that $\mE_{\xstar}[\langle \xstar, \Bone \halpha - \B \balpha_{t+1} \rangle^2] = \norm{\Bone \halpha - \B \balpha_{t+1}}^2$. Combining \cref{thm:lr_transfer} and \cref{thm:B_recovery} and applying a union bound then gives the result.
\end{proof}


\section{Proofs in \cref{sec:lf_mom}}
\label{app:mom}

Analyzing the performance of the method-of-moments estimator requires two steps. First, we show that the estimator $(1/n)\cdot \sum_{i=1}^n y_i^2 \x_i\x_i\trans$ converges to its mean in spectral norm, up to error fluctuations $\tlO(\sqrt{\frac{dr}{n}})$. Showing this requires adapting tools from the theory of matrix concentration.
Second, a standard application of the Davis-Kahan $\sin \theta$ theorem shows that top-r PCA applied to this noisy matrix, $(1/n)\cdot \sum_{i=1}^n y_i^2 \x_i\x_i\trans$, can extract a subspace $\hB$ close to the true column space of $\B$ up to a small error. Throughout this section we let $\barGamma = \sumton \barGamma_i$ with $\barGamma_i = \B \balpha_{t(i)} \balpha_{t(i)}^\top \B^\top$. We also let $\barLambda = \sumton \balpha_{t(i)} \balpha_{t(i)}^\top$ be the empirically observed task matrix. Note that under \cref{assump:task}, we have that $\barGamma$ and $\barLambda$ behave identically since $\B$ has orthonormal columns we have that $\tr(\barGamma) = \tr(\barLambda)$ and $\sigma_{r}(\barGamma) = \sigma_{r}(\barLambda)$. Furthermore throughout this section we use $\tkappa$ and $\tnu$ to refer to the average condition number and $r$-th singular value of the empirically observed task matrix $\barLambda$ -- since all our results hold in generality for this matrix. Note that under the uniform task observation model the task parameters of $\barLambda$ and the population task matrix $\frac{\A^\top \A}{t}$ are equal.

We first present our main theorem which shows our method-of-moments estimator can recover the true subspace $\B$ up to small error. 

\begin{proof}[Proof of \cref{thm:B_recovery}]
The proof follows by combining the Davis-Kahan sin $\theta$ theorem with our main concentration result for the matrix $\sumton y_i^2 \x_i^\top \x_i-\mE[\sumton y_i^2 \x_i^\top \x_i]$. First note that $\mE[\sumton y_i^2 \x_i^\top \x_i] = (2\barGamma + (1+\tr(\barGamma)) \I_d$ by \cref{lem:estimator_mean} and define $\sumton y_i^2 \x_i^\top \x_i-\mE[\sumton y_i^2 \x_i^\top \x_i] = \E$. Note that under the conditions of the result for $n \geq c d$ we have that $\norm{\E} \leq \tlO(\sqrt{\frac{d \tkappa r \tnu}{n}})$ by \cref{thm:estimator_conc} for large-enough $c$ due to the SNR normalization; so again by taking sufficiently large $c$ such that $n \geq c \cdot \polylog(d, n) \tkappa r d/\tnu$ we can ensure that $\norm{\E} \leq \delta \leq 2 \tnu$ for as small $\delta$ as we choose with the requisite probability.
	 Since $\norm{\bE} \leq \delta$ we have that $\sigma_{r+1}(y_i^2 \x_i\x_i\trans) - \sigma_{r+1}((2\barGamma + (1+\tr(\barGamma)) \I_d) \leq \delta$ and since $\barGamma$ is rank $r$,  $\sigma_{r}((2\barGamma + (1+\tr(\barGamma)) \I_d)-\sigma_{r+1}((2\barGamma + (1+\tr(\barGamma)) \I_d) = 2\sigma_{r}(\barGamma)$. Hence, applying the Davis-Kahan $\sin \theta$ theorem shows that, 
	\begin{align*}
		\norm{\Btwo^\top \B} \leq \frac{\norm{\Btwo^\top \E \B}}{2 \sigma_{r}(\barLambda) - \delta} \leq \frac{\norm{\E}}{2 \sigma_{r}(\barLambda) - \delta} \leq \frac{\norm{\E}}{\nu} \leq \tlO \left(\sqrt{\frac{1}{\tnu} \frac{d \tkappa r}{n}} \right)
	\end{align*}
	where the final inequalities follows by taking $c$ large enough to ensure $\delta \leq \mu$ and \cref{thm:estimator_conc}.

\end{proof}

We now present our main result which proves the concentration of the estimator,
\begin{theorem}
	Suppose the $n$ data samples $(\x_i, y_i)$ are generated from the model in \eqref{eq:model} and that \cref{assump:design,,assump:task} hold with $\x_i \sim \cN(0, 1)$ i.i.d. Then if $n \gtrsim c$ for sufficiently large $c$, 
	\begin{align*}
		& \norm{\sumton y_i^2 \x_i \x_i^\top - (2\barGamma + (1+\tr(\barGamma)) \I_d))} \leq \\
		& \log^3 n \cdot \log^3 d \cdot O \left(\sqrt{\frac{d \tkappa r \tnu}{n}} + \frac{d}{n} \right),
	\end{align*}
	with probability at least $1-O(n^{-100})$.
	\label{thm:estimator_conc}
\end{theorem}
\begin{proof}
	Note that the mean of $\sumton y_i^2 \x_i \x_i^\top$ is $2\barGamma + (1+\tr(\barGamma)) \I_d)$ by \cref{lem:estimator_mean}. Then using the fact that $y_i = \x_i^\top \B \balpha_{t(i)}+\epsilon_i$, we can write down the error decomposition for the estimator into signal and noise terms,
\begin{align*}
	 & \sumton y_i^2 \x_i\x_i\trans - (2\barGamma + (1+\tr(\barGamma)) \I_d = \sumton (\x_i \B \balpha_{t(i)})^2 \x_i \x_i^\top - (2\barGamma + \tr(\barGamma)) \I_d + \\
	 & \sumton 2 \epsilon_i \x_i \B \balpha_{t(i)} \x_i \x_i^\top + \sumton \epsilon_i^2 \x_i\x_i\trans - \I_d.
\end{align*}
We proceed to control the fluctuations of each term in spectral norm individually using tools from matrix concentration.
Applying \cref{lem:first_noise}, \cref{lem:second_noise}, \cref{lem:third_noise}, the triangle inequality and a union bound shows the desired quantity is upper bounded as,
\begin{align*}
& \log^3n  \cdot \log^3d \cdot O \left(\sqrt{\frac{d \max(1, \tr(\barGamma), \tr(\barGamma) \max_i \norm{\bbeta_i}^2)}{n}} + \frac{d \max(1, \max_i \norm{\bbeta_i}, \max_i \norm{\bbeta_i}^2)}{n} \right) 
& 
\end{align*}
Finally using \cref{assump:task} and the fact that $\tr{\barGamma} = \tr{\barLambda}$ and the fact $\norm{\bbeta_i}=\norm{\balpha_i}$ simplifies the result to the theorem statement. Note that since $\norm{\balpha_i} = \Theta(1)$ for all $i$ we have that, $\tr(\barGamma) = \Theta(1)$ so the SNR normalization guarantees the leading noise term satisfies $1 \leq O( \tr(\barGamma))$.
\end{proof}


We begin by computing the mean of the estimator.
\begin{lemma}
	\label{lem:estimator_mean}
	Suppose the $n$ data samples $(\x_i, y_i)$ are generated from the model in \eqref{eq:model_main} and that \cref{assump:design,,assump:task} hold. Then,
	\begin{align*}
		\mE[\sumton y_i^2 \x_i \x_i^\top] = 2\barGamma + (1+\tr(\barGamma)) \I_d
	\end{align*}
	where $\barGamma= \sumton \barGamma_i$ with $\mGamma_i = \B \balpha_{t(i)} \balpha_{t(i)}^\top \B^\top$.
\end{lemma}
\begin{proof}
	Since $\epsilon_i$ is mean-zero, using the definition of $y_i$ we immediately obtain,
	\begin{align*}
		\mE[\sumton y_i^2 \x_i \x_i^\top] = 2\barGamma + (1+\tr(\barGamma)) \I_d] = \I_d + \mE[\sumton \x_i^\top \mGamma_i \x_i \x_i \x_i^\top] = \I_d + \mE[\x^\top \barGamma \x \x \x^\top]
	\end{align*}
	for $\x \sim \cN(0, \I_d)$. Using the eigendecomposition of $\barGamma$ we have that $\mE[\x^\top \barLambda \x \x \x^\top] = \sumtor \sigma_i \mE[(\x^\top \v_i)^2 \x\x^\top]$. Due to the isotropy of the Gaussian distribution, it suffices to compute $\mE[(\x^\top \e_1)^2 \x\x^\top]$ and rotate the result back to $\v_i$. In particular we have that, 
	\begin{align*}
		& (\mE[(\x^\top \e_1)^2 \x\x^\top])_{ij} = \begin{cases}
			0 \quad i \neq j \\
			1 \quad i=j \neq 1 \\
			3  \quad i=j=1 \\
		\end{cases} \implies 
		\mE[(\x^\top \e_1)^2 \x\x^\top] = 2 \e_1 \e_1 + \I_d \implies \\
		& \implies \mE[(\x^\top \v_i)^2 \x\x^\top] = 2 \v_i \v_i + \I_d \implies \E[\x^\top \barGamma \x \x \x^\top] = 2 \barGamma + \tr(\barGamma) \I_d
	\end{align*}
	from which the conclusion follows.
\end{proof}

We start by controlling the fluctuations of the final noise term (which has identity mean). 
\begin{lemma}
	\label{lem:first_noise}
Suppose the $n$ data samples $(\x_i, y_i)$ are generated from the model in \eqref{eq:model_main} and that \cref{assump:design,,assump:task} hold. Then for $n \geq c$ for sufficiently large $c$,
	\begin{align*}
		\norm{\sumton \epsilon_i^2 \x_i \x_i^\top-\I_d} \leq O \left(\log^2 n \left(\sqrt{\frac{d}{n}} + \frac{d}{n} \right) \right).
	\end{align*}
	with probability at least $1-O(n^{-100})$.
\end{lemma}
\begin{proof}
	We first decompose the expression as,
	\begin{align*}
		\norm{\sumton \epsilon_i^2 \x_i \x_i^\top-\I_d} \leq \norm{\sumton \epsilon_i^2 \x_i \x_i^\top - \sumton \epsilon_i^2 \I_d} + \norm{\sumton \epsilon_i^2 \I_d - \I_d}
	\end{align*}
	
	We first control the second term. By a sub-exponential tail bound we have that $\Pr[\abs{\sumton \epsilon_i^2-1}\geq t] \leq 2 \exp(-C n\min(t^2/8^2, t/8))$ since $\epsilon_i^2$ is $\sE(8,8)$ by \cref{lem:prod_sg}. Letting $t=c \sqrt{\log(\frac{1}{\delta})/n}$ for sufficiently large $c$, and assuming $n \gtrsim \log(\frac{1}{\delta})$, implies $\abs{\sumton \epsilon_i^2-1} \leq  O(\sqrt{\frac{\log(1/\delta)}{n}})$ with probability at least $1-2\delta$. Hence   $\norm{\sumton \epsilon_i^2 \I_d - \I_d} \leq O(\sqrt{\frac{\log(1/\delta)}{n}})$ on this event. 
	
	Now we apply \cref{lem:scaled_sgvec} with $a_i = \epsilon_i$ to control the first term.
	Using the properties of sub-Gaussian maxima we can conclude that $\Pr[\max_i \abs{\epsilon}_i \geq t] \leq 2n \exp(-t^2/2)$; taking $t=4 \sqrt{\log n}+c\sqrt{\log(1/\delta)}$ for sufficiently large $c$ implies that $\max_{i} \abs{\epsilon_i} \leq O(\sqrt{\log n})+O(\sqrt{\log(1/\delta)})$ with probability at least $1-\delta$. In the setting of \cref{lem:scaled_sgvec}, conditionally on $\epsilon_i$, $K = \max_{i} |\epsilon_i|$ and $\mSigma=\I_d$ so taking $t = c\sqrt{\log(1/\delta)}$ for sufficiently large $c$ implies that $\norm{\sumton \epsilon_i^2 \x_i \x_i^\top - \sumton \epsilon_i^2 \I_d} \leq K \cdot O(\sqrt{d/n}+\sqrt{\log(1/\delta)/n} + \frac{d}{n} + \frac{\log(1/\delta)}{n})$ with probability at least $1-2 \delta$ conditionally on $\epsilon_i$. Conditioning on the event that $\max_{i} \abs{\epsilon_i} \leq O(\sqrt{\log n})+O(\sqrt{\log(1/\delta)})$ to conclude the argument finally shows that, 
	\begin{align*}
		& \norm{\sumton \epsilon_i^2 \x_i \x_i^\top-\I_d} \leq O(\log n+\log(1/\delta)) \cdot O(\sqrt{\frac{d}{n}}+\sqrt{\frac{\log(1/\delta)}{n}} + \frac{d}{n} + \frac{\log(1/\delta)}{n}) + O(\sqrt{\frac{\log(1/\delta)}{n}})  \\ 
	\end{align*}
	with probability at least $1-5 \delta$.
	Selecting $\delta = n^{-100}$ implies that $\norm{\sumton \epsilon_i^2 \x_i \x_i^\top-\I_d} \leq O \left(\log^2 n \left(\sqrt{\frac{d}{n}} + \frac{d}{n} \right) \right)$,
	with probability at least $1-O(n^{-100})$.
\end{proof}

We now proceed to controlling the fluctuations of the second noise term (which is mean-zero). Our main technical tool is \cref{lem:trunc_mb}.

\begin{lemma}
	\label{lem:second_noise}
	Suppose the $n$ data samples $(\x_i, y_i)$ are generated from the model in \eqref{eq:model_main} and that \cref{assump:design,,assump:task} hold. Then,
	\begin{align*}
		\norm{\sumton 2 \epsilon_i \x_i^\top \B \balpha_{t(i)} \x_i \x_i^\top} \leq O((\log n + \log d) \left(\sqrt{\frac{d \tr(\barGamma)}{n}} +  \frac{d \max_i \norm{\bbeta_i} (\log^2(n) + \log^2(d))}{n} \right).
	\end{align*}
	with probability at least $1-O((nd)^{-100})$.
\end{lemma}
\begin{proof}
	To apply the truncated version of the matrix Bernstein inequality (in the form of \cref{lem:trunc_mb}) we need to set an appropriate truncation level $R$, for which need control on the norms of $Z_i = \norm{2 \epsilon_i \x_i^\top \B \balpha_{t(i)} \x_i \x_i^\top} = 2 \abs{\epsilon_i} \norm{\x_i}^2 \abs{\x_i^\top \B \balpha_{t(i)}}$. Using sub-gaussian, and sub-exponential tail bounds we have that $\abs{\epsilon_i} \leq O(1+ \sqrt{\log(1/\delta)})$, $\norm{\x_i}^2 \leq O(d+\max(\sqrt{d \log(1/\delta)}, \log(1/\delta))) = O(d+\sqrt{d} \log(1/\delta))$, and $\abs{\x_i^\top \B \balpha_{t(i)}} \leq O(\norm{\bbeta_i}(1+\sqrt{\log(1/\delta)})$ each with probability at least $1-\delta$. Accordingly with probability at least $1-3\delta$ we have that $\norm{Z_i} \leq O(\norm{\bbeta_i} d(1+\log^2(1/\delta)))$. We can rearrange this statement to conclude that $\Pr[\norm{Z_i} \geq c_1 \norm{\bbeta_i} d + t] \leq 3 \exp(-c_2 (\frac{t}{\norm{\bbeta_i} d})^{1/2})$ for some $c_1, c_2$. Define a truncation level $R = c_1 \max_i \norm{\bbeta_i} d + K \max_i \norm{\bbeta_i} d$ for some $K$ to be chosen later. We can also use the aforementioned tail bound to control $\norm{\mE[Z_i]-\mE[Z_i']} \leq \mE[Z_i \Ind[\norm{Z_i} \geq \alpha]] \leq \int_{K \norm{\bbeta_i} d}^{\infty} 3 \exp(-c_2 (\frac{t}{\norm{\bbeta_i} d})^{1/2}) \leq O((1+\sqrt{K}) \exp(-c \sqrt{K}) \max_i \norm{\bbeta_i} d) = \Delta$.

	Next we must compute an upper bound the matrix variance term $\norm{\sum_{i=1}^n \mE[\epsilon_i^2 (\balpha_i^\top \B^\top \x_i)^2 \norm{\x_i}^2 \x_i \x_i^\top]} = \norm{\sum_{i=1}^n \mE[(\balpha_i^\top \B^\top \x)^2 \norm{\x}^2 \x \x^\top]} = n \norm{\mE[\x^\top \barGamma \x \norm{\x}^2 \x \x^\top]} = n \norm{\sumtor \sigma_i \mE[(\v_i^\top \x)^2 \norm{\x}^2 \x \x^\top]}$ taking the expectation over $\epsilon_i$ in the first equality, and diagonalizing $\barGamma$.
	As before due to isotropy of the Gaussian it suffices to compute the expectation with $\v_i = \e_1$ and rotate the result back to $\v_i$. Before computing the term we note that for a standard normal gaussian random variable $g \sim \cN(0,1)$ we have that $\mE[g^6]=15$, $\mE[g^4]=3$, $\mE[g^2]=1$. Then by simple combinatorics we find that,
	\begin{align*}
		& (\mE[x_1^2 (\sum_{a=1}^n x_a^2) \x \x^\top])_{ij} = \begin{cases}
			0 \quad i \neq j \neq 1 \\
			0 \quad i = 1 \neq j \\
			2 \cdot 3 \cdot 1 + (d-2) \cdot 1 \quad i=j \neq 1 \\
		    15 + 3(d-1) \quad i=j=1 \\
		\end{cases} \implies \mE[(\x^\top \e_1)^2 \norm{\x}^2 \x \x^\top] = (2d+8) \e_1 \e_1^\top + (d+4) \I_d \\
		& \implies \norm{\sum_{i=1}^n \mE[\epsilon_i^2 (\balpha_i^\top \B^\top \x_i)^2 \norm{\x_i}^2 \x_i \x_i^\top]} \leq n(d+4) \norm{\barGamma + \tr(\barGamma) \I_d} \leq 10 nd (\tr(\barGamma)) = \sigma^2.
	\end{align*}

Finally, we can assemble the previous two computations to conclude the result with appropriate choices of $R$ (parametrized through $K$) and $t$ by combining with \cref{lem:trunc_mb}. Before beginning recall by definition we have that $\tr(\barGamma) = \frac{1}{n}  \max_i \norm{\bbeta_i}^2$. Let us choose $\sqrt{K} = \frac{c_3}{c} (\log(n) + \log(d))$ for some sufficiently large $c_3$. In this case, we can choose $c_3$ such that $\Delta \leq O((\log n + \log d) \frac{\max_i \norm{\bbeta_i} d}{n^{10} d^{10}}) \leq O(\frac{\sqrt{\tr(\barGamma)}}{n^8 d^8})$, since $\sqrt{\tr(\barGamma)} \geq \frac{1}{\sqrt{n}} \max_i \norm{\bbeta_i}$. Similarly, our choice of truncation level becomes $R = O( (\log^2(n) + \log^2(d)) \max_i \norm{\bbeta_i} d)$. At this point we now choose $t = c_4(\log n + \log d) \max(\sigma/\sqrt{n}, R/n)$ for sufficiently large $c_4$. For large enough $c_4$ we can guarantee that $t \geq 2 \Delta \implies t - \Delta \geq \frac{t}{2}$.

Hence combining these results together and applying \cref{lem:trunc_mb} we can provide the following upper bound on the desired quantity,
\begin{align*}
	\Pr[\norm{\sumton 2 \epsilon_i \x_i^\top \B \balpha_{t(i)} \x_i \x_i^\top} \geq t] \leq O(d \exp(-c \cdot c_4 (\log n + \log d)) + O(n \sqrt{K} \exp(-c_3 (\log n + \log d)) \leq O((nd)^{-100})
\end{align*}
by taking $c_3$ and $c_4$ sufficiently large, with $t = O((\log n + \log d) \left(\sqrt{\frac{d \tr(\barGamma)}{n}} +  \frac{d \max_i \norm{\bbeta_i} (\log^2(n) + \log^2(d))}{n} \right)$.
\end{proof}

Finally we turn to controlling the fluctuations of the primary signal term around its mean using a similar argument to the previous term.

\begin{lemma}
	\label{lem:third_noise}
	Suppose the $n$ data samples $(\x_i, y_i)$ are generated from the model in \eqref{eq:model_main} and that \cref{assump:design,,assump:task} hold. Then
	\begin{align*}
		\norm{\sumton (\x_i \B \balpha_{t(i)})^2 \x_i \x_i^\top-(2\barGamma + \tr(\barGamma) \I_d)} \leq O((\log n + \log d) \left(\sqrt{\frac{d \tr(\barGamma) \max_i \norm{\bbeta_i}^2}{n}} +  \frac{d \max_i \norm{\bbeta_i}^2 (\log^2(n) + \log^2(d))}{n} \right)
	\end{align*}
	with probability at least $1-O((nd)^{-100})$.
\end{lemma}
\begin{proof}
	The proof is similar to the proof of \cref{lem:second_noise} and uses \cref{lem:trunc_mb}. We begin by controlling the norms of $Z_i = (\x_i^\top \B \balpha_{t(i)})^2 \x_i \x_i^\top$. $\norm{Z_i} = \norm{\x_i}^2 (\x_i^\top \B \balpha_{t(i)})^2$. Using Gaussian and sub-exponential tail bounds we have that, $\norm{\x_i}^2 \leq O(d+\sqrt{d} \log(1/\delta))$ and $(\x_i^\top \B \balpha_{t(i)})^2 \leq O(\norm{\bbeta_i}^2(1+\log(1/\delta)))$ each with probability at least $1-\delta$. Hence with probability at least $1-2\delta$ we find that $\norm{Z_i} \leq O(d \norm{\bbeta_i}^2 (1+ \log^2(1/\delta))$.

	We can rearrange this statement to conclude that $\Pr[\norm{Z_i} \geq c_1 \norm{\bbeta_i}^2 d + t] \leq 2 \exp(-c_2 (\frac{t}{\norm{\bbeta_i}^2 d})^{1/2})$ for some $c_1, c_2$. Define a truncation level $R = c_1 \max_i \norm{\bbeta_i}^2 d + K \max_i \norm{\bbeta_i}^2 d$ for some $K$ to be chosen later. We can use the aforementioned tail bound to control $\norm{\mE[Z_i]-\mE[Z_i']} \leq \mE[Z_i \Ind[\norm{Z_i} \geq \alpha]] \leq \int_{K \norm{\bbeta_i}^2 d}^{\infty} 2 \exp(-c_2 (\frac{t}{\norm{\bbeta_i}^2 d})^{1/2}) \leq O((1+\sqrt{K}) \exp(-c \sqrt{K}) \max_i \norm{\bbeta_i}^2 d) = \Delta$.

	Next we must compute an upper bound the matrix variance term $\norm{\sum_{i=1}^n \mE[(\balpha_i^\top \B^\top \x_i)^4 \norm{\x_i}^2 \x_i \x_i^\top]} = \norm{\sum_{i=1}^n \mE[(\bbeta_i^\top \x)^4 \norm{\x}^2 \x \x^\top]}$.
	As before due to isotropy of the Gaussian it suffices to compute each expectation assuming $\bbeta_i \propto \e_1$ and rotate the result back to $\bbeta_i$. Before computing the term we note that for a standard normal gaussian random variable $g \sim \cN(0,1)$ we have that $\mE[g^8]=105$, $\mE[g^6]=15$, $\mE[g^4]=3$, $\mE[g^2]=1$. Then by simple combinatorics we find that,
	\begin{align*}
		& (\mE[(\x^\top \e_1)^4 (\sum_{a=1}^n x_a^2) \x \x^\top])_{ij} = \begin{cases}
			0 \quad i \neq j \neq 1 \\
			0 \quad i = 1 \neq j \\
			15+3 \cdot 3 + (d-2) \cdot 3 \quad i=j \neq 1 \\
		    105 + 15(d-1) \quad i=j=1 \\
		\end{cases} \implies \mE[(\x^\top \bbeta_i)^4 \norm{\x}^2 \x \x^\top] = (2d+75) \e_1 \e_1^\top + \\
		& (3d+15) \I_d \\
		& \implies \norm{\sum_{i=1}^n \mE[(\balpha_i^\top \B^\top \x_i)^4 \norm{\x_i}^2 \x_i \x_i^\top]} \leq O(d) \norm{\sum_{i}^n \norm{\bbeta_i}^4(\bbeta_i \bbeta_i^\top + \I_d)} \leq O(d \sum_{i=1}^n \norm{\bbeta_i}_2^4) \leq O(dn \max_i \norm{\bbeta_i}^2 \tr(\barGamma)) \\
		& = \sigma^2.
	\end{align*}
Finally, we can assemble the previous two computations to conclude the result with appropriate choices of $R$ (parametrized through $K$) and $t$ by combining with \cref{lem:trunc_mb}. Before beginning recall by definition we have that $\tr{\barGamma} \geq \frac{1}{n}  \max_i \norm{\bbeta_i}^2$. Let us choose $\sqrt{K} = \frac{c_3}{c} (\log(n) + \log(d))$ for some sufficiently large $c_3$. In this case, we can choose $c_3$ such that $\Delta \leq O((\log n + \log d) \frac{\max_i \norm{\bbeta_i}^2 d}{n^{10} d^{10}}) \leq O(\frac{\sqrt{\tr(\barGamma)} \max_i \norm{\bbeta_i}}{n^7 d^7})$, since $\sqrt{\tr(\barGamma)} \geq \frac{1}{\sqrt{n}} \max_i \norm{\bbeta_i}$. Similarly, our choice of truncation level becomes $R = O( (\log^2(n) + \log^2(d)) \max_i \norm{\bbeta_i}^2 d)$. At this point we now choose $t = c_4(\log n + \log d) \max(\sigma/\sqrt{n}, R/n)$ for sufficiently large $c_4$. For large enough $c_4$ we can guarantee that $t \geq 2 \Delta \implies t - \Delta \geq \frac{t}{2}$.

Hence combining these results together and applying \cref{lem:trunc_mb} we can provide the following upper bound on the desired quantity,
\begin{align*}
	& \Pr[\norm{\sumton 2 \epsilon_i \x_i^\top \B \balpha_{t(i)} \x_i \x_i^\top} \geq t] \leq O(d \exp(-c \cdot c_4 (\log n + \log d)) + O(n \sqrt{K} \exp(-c_3 (\log n + \log d)) \leq \\
	 & O((nd)^{-100})
\end{align*}
by taking $c_3$ and $c_4$ sufficiently large, with $t = O((\log n + \log d) \left(\sqrt{\frac{d \tr(\barGamma) \max_i \norm{\bbeta_i}^2}{n}} +  \frac{d \max_i \norm{\bbeta_i}^2 (\log^2(n) + \log^2(d))}{n} \right)$.
\end{proof}

\section{Proofs in \cref{sec:new_task}}
Assuming we have obtained estimate of the column space or feature set $\Bone$ for the initial set of tasks such that $\norm{\Bone^\top \B} \leq \delta$ we now analyze the performance of the plug-in estimator (which explicitly uses the estimate $\Bone$ in lieu of the unknown $\B$) on a new task. Recall we define the estimator for the new tasks underlying parameter vector by a projected linear regression estimator: $\halpha =\argmin_{\balpha} \norm{\y-\X \Bone \balpha}^2 \implies \halpha = (\Bone^\top \X^\top \X \Bone)^{-1} \Bone^\top \X^\top \y$.

Analyzing the performance of this estimator requires first showing the low-dimensional empirical covariance and empirical correlation concentrate in $\tlO(r)$ samples and performing an error decomposition to compute the bias resulting from using $\Bone$ in lieu of $\B$ as the feature representation. We measure the performance the estimator with respect to its estimation error on the underlying parameter $\B \balpha_0$ -- which can be written as $\norm{\Bone \halpha-\B \balpha_0}^2$. Note that here our analysis can accommodate covariates $\x_i$ generated from \textit{non-Gaussian} distributions. In fact the only condition we require on the design is that the covariates are sub-Gaussian random vectors in the following sense.
	\begin{assumption}
	Each covariate vector $\x_i$ is sub-gaussian, in the sense that, $
     \mE[\exp(\v^\top \x_i)] \leq \exp \left( \frac{\Vert \mSigma^{1/2} \v \Vert^2}{2} \right)$. Moreover, the additive noise $\epsilon_i$ is i.i.d. sub-Gaussian with variance parameter $1$ and independent of $\x_i$.
	\label{assump:sg_design}
	\end{assumption}
	Note that \cref{assump:design} immediately implies \cref{assump:sg_design}.


	Throughout this section we will let $\Bone$ and $\Btwo$ be orthonormal projection matrices spanning orthogonal subspaces, which are rank $r$ and rank $d-r$ respectively -- so that $\ran(\Bone) \oplus \ran(\Btwo) = \mR^d$.

\begin{proof}[Proof of \cref{thm:lr_transfer}]
	To begin we use the definition of $\halpha = (\Bone^\top \X^\top \X \Bone)^{-1} \Bone \X^\top \y = (\Bone^\top \X^\top \X \Bone)^{-1} \Bone \X^\top \X \B \balpha_0 + (\Bone^\top \X^\top \X \Bone)^{-1} \Bone \X^\top \bepsilon$ to decompose the error as,
	\begin{align*}
		& (\Bone\halpha-\B \balpha_0) = \Bone (\Bone^\top \X^\top \X \Bone)^{-1} \Bone \X^\top \X \B \balpha_0 - \B \balpha_0 + \Bone(\Bone^\top \X^\top \X \Bone)^{-1} \Bone^\top \X^\top \bepsilon
	\end{align*}
	Now squaring both sides of the equation gives,
	So \begin{align*}
	& \norm{\Bone\halpha-\B \balpha_0}^2 \leq 2(\norm{\Bone (\Bone^\top \X^\top \X \Bone)^{-1} \Bone \X^\top \X \B \balpha_0 - \B \balpha_0}^2+\norm{\Bone(\Bone^\top \X^\top \X \Bone)^{-1} \Bone^\top \X^\top \bepsilon}^2)
	\end{align*}
	The first bias term can be bounded by \cref{lem:test_bias}, while the the variance term can be bounded by \cref{lem:test_var} . Combining the results and using a union bound gives the result.
\end{proof}

We now present the lemmas which allow us to bound the variance terms in the aforementioned error decomposition. For the following two results we also track the conditioning dependence with respect $\Cmin$ and $\Cmax$. We first control the term arising from the projection of the additive noise onto the empirical covariance matrix.
\begin{lemma}
	Let the sequence of $n$ i.i.d. covariates $\x_i$ and $n$ i.i.d. additive noise variables $\epsilon_i$ satisfy \cref{assump:sg_design}. Then if $n \gtrsim \cond^2 r \log n$,
	\begin{align*}
		\norm{\Bone(\Bone^\top \X^\top \X \Bone)^{-1} \Bone^\top \X^\top \bepsilon}^2 \leq O \left( \frac{r \log n}{\Cmin n} \right)
	\end{align*}
	with probability at least $1-O(n^{-100})$.
	\label{lem:test_bias}
\end{lemma}
\begin{proof}
Since $\norm{\Bone(\Bone^\top \X^\top \X \Bone)^{-1} \Bone^\top \X^\top \bepsilon}^2 \leq \norm{(\Bone^\top \X^\top \X \Bone)^{-1} \Bone^\top \X^\top \bepsilon}^2$, it suffices to bound the latter term. Consider $\bepsilon^\top \underbrace{\frac{1}{n} \frac{\X \Bone}{\sqrt{n}} (\Bone^\top \frac{\X^\top \X}{n} \Bone)^{-2} \frac{\Bone^\top \X^\top}{\sqrt{n}}}_{\A} \bepsilon$. So applying the Hanson-Wright inequality \citep[Theorem 6.2.1]{vershynin2018high} (conditionally on $\X$) to conclude that $\Pr[\abs{\bepsilon^\top \A \bepsilon - \E[\bepsilon^\top \A \bepsilon]} \geq t] \leq 2 \exp(-c \min(\frac{t^2}{\norm{\A}_F^2}, \frac{t}{\norm{\A}}))$. Hence $\bepsilon^\top \A \bepsilon \leq \E[\bepsilon^\top \A \bepsilon] + O(\norm{\A}_F \sqrt{\log(2/\delta_1)})+ O(\norm{\A} \log(2/\delta_1))$ with probability at least $1-\delta_1$.

	 Now using cyclicity of the trace we have that $\mE[\bepsilon^\top \A \bepsilon] = \frac{1}{n} \tr[(\Bone^\top \frac{\X^\top \X}{n} \Bone)^{-1}]$. Similarly $\norm{\A} = \frac{1}{n}\norm{(\Bone^\top \frac{\X^\top \X}{n} \Bone)^{-1}} = \frac{1}{n}\norm{(\E + \Bone^\top \mSigma \Bone)^{-1}}$. Applying \cref{lem:two_subspace_conc} to the matrix $\E$ with $\delta=n^{-200}$ and assuming $n \gtrsim \cond^2 r \log(1/\delta) \gtrsim \cond^2 r \log n$ shows that $\norm{(\Bone^\top \mSigma \Bone)^{-1} \E} \leq \frac{1}{4}$. Also note that on this event and this regime of sufficiently large $n$, this concentration result shows that $\sigma_{\min}(\Bone^\top \frac{\X^\top \X}{n} \Bone) > \Cmin/2$,  so the matrix is invertible. Hence an application of \cref{lem:mat_pert} shows that $\norm{\A} \leq \frac{1}{n} (\frac{1}{\Cmin} \cdot(1+\cond  \sqrt{\frac{r \log n}{n}} )) \leq O(\frac{1}{\Cmin n})$. Similarly since $\frac{\X \Bone}{\sqrt{n}}$ is rank $r$ and invertible on this event, it follows $\fnorm{\A} \leq \sqrt{r} \norm{\A}\leq O(\frac{\sqrt{r}}{\Cmin n})$ and that $\frac{1}{n} \tr[(\Bone^\top \frac{\X^\top \X}{n} \Bone)^{-1}] \leq \frac{r}{\Cmin n}$.

	Hence taking $\delta_1 = n^{-200}$, and using the union bound, we conclude that $\bepsilon^\top \A \bepsilon \leq \frac{1}{\Cmin} \cdot O(\frac{r}{n}) + O(\frac{\sqrt{r \log n}}{n}) + O(\frac{\log n}{n}) \leq O(\frac{r \log n}{\Cmin n})$ with probability at least $1-O(n^{-100})$.
\end{proof}

We now control the error term which arises both from the variance in the random design matrix $\X$ and the bias due to mismatch between $\Bone$ and $\B$.

\begin{lemma}
	Let the sequence of $n$ i.i.d. covariates $\x_i$ satisfy the design assumptions in \cref{assump:sg_design}, and assume $\sin(\Bone, \B) \leq \delta \leq 1$. Then if $n \gtrsim \cond^2 r \log n$,
	\begin{align*}
		\norm{\Bone (\Bone^\top \X^\top \X \Bone)^{-1} \Bone \X^\top \X \B \balpha_0 - \B \balpha_0}^2 \leq O( \norm{\balpha_0}^2 \cond^2 \delta^2 ),
	\end{align*}
	with probability at least $1-O(n^{-100})$.
	\label{lem:test_var}
\end{lemma}
\begin{proof}
To control this term we first insert a copy of the identity $\I_d = \Bone \Bone^\top+\Btwo \Btwo^\top$ to allow the variance term in the design cancel appropriately in the span of $\Bone$; formally, 
	\begin{align*}
		& \Bone (\Bone^\top \X^\top \X \Bone)^{-1} \Bone \X^\top \X \B \balpha_0 -\B \balpha_0 = \Bone (\Bone^\top \X^\top \X \Bone)^{-1} \Bone \X^\top \X (\Bone \Bone^\top + \Btwo \Btwo^\top) \B \balpha_0 - \B \balpha_0 = \\
		& (\Bone \Bone^\top - \I) \B \balpha_0 + \Bone (\Bone^\top \X^\top \X \Bone)^{-1} \Bone \X^\top \X \Btwo \Btwo^\top \B \balpha_0 = \B_2 \B_2^\top \B \balpha_0 + \Bone (\Bone^\top \X^\top \X \Bone)^{-1} \Bone \X^\top \X \Btwo \Btwo^\top \B \balpha_0 \implies \\
		& \norm{\Bone (\Bone^\top \X^\top \X \Bone)^{-1} \Bone \X^\top \X \B \balpha_0 -\B \balpha_0}^2 \leq 2(\norm{\balpha_0}^2 \delta^2 + \norm{(\Bone^\top \X^\top \X \Bone)^{-1} \Bone \X^\top \X \Btwo}^2 \delta^2 \norm{\balpha_0}^2) 
	\end{align*}
	We now turn to bounding the second error term, $\norm{(\Bone^\top \X^\top \X \Bone)^{-1} \Bone^\top \X^\top \X \B}^2$. Now let $\E_1 = \Bone^\top \frac{\X^\top \X}{n} \Bone-\Bone^\top \mSigma \Bone$ and $\E_2 = \Bone^\top \frac{\X^\top \X}{n} \B - \Bone \mSigma \B$.  Applying \cref{lem:two_subspace_conc} to the matrix $\E_1$ with $\delta = n^{-200}$ and assuming $n \gtrsim \cond^2 r \log(1/\delta) \gtrsim \cond^2 r \log n$ shows that $\norm{(\Bone^\top \mSigma \Bone)^{-1} \E_1} \leq \frac{1}{4}$ and $\norm{\E_1} \leq O(\Cmax \sqrt{\frac{r \log n}{n}})$ with probability at least $1-O(n^{-100})$. A further application of \cref{lem:mat_pert} shows that $(\Bone^\top \frac{\X^\top \X}{n} \Bone)^{-1} = (\E_1 + \Bone^\top \mSigma \Bone)^{-1} = (\Bone^\top \mSigma \Bone)^{-1} + \F $, where $\norm{\F} \leq \frac{4}{3} \norm{(\Bone^\top \mSigma \Bone)^{-1}} \norm{\E_1 (\Bone^\top \mSigma \Bone)^{-1}}$ on this event. Similarly, defining $\Bone^\top \frac{\X^\top \X}{n} \B = \E_2 + \Bone^\top \mSigma \B$	and applying \cref{lem:two_subspace_conc} again but to the matrix $\E_2$ with $\delta = n^{-200}$ and assuming $n \gtrsim \cond^2 r \log(1/\delta) \gtrsim \cond^2 r \log n$,	guarantees that $\norm{\E_2} \leq O(\Cmax (\sqrt{\frac{r \log n}{n}})$ with probability at least $1-O(n^{-100})$. 
		
		Hence on the intersection of these two events, 
		\begin{align*}& \norm{(\Bone^\top \frac{\X^\top \X}{n} \Bone)^{-1} \Bone^\top \frac{\X^\top \X}{n} \B} = \norm{((\Bone^\top \mSigma \Bone)^{-1}+\F)(\Bone^\top \mSigma \B + \E_2)} \leq \\
		& \norm{(\Bone^\top \mSigma \Bone)^{-1} \Bone^\top \mSigma \B} + \norm{(\Bone^\top \mSigma \Bone)^{-1} \E_2} + \norm{\F \Bone^\top \mSigma \B} + \norm{\E_2 \F} \leq \\
		& \cond + O(\cond \sqrt{\frac{r \log n}{n}}) + O(\cond^2 \sqrt{\frac{r \log n}{n}}) + O(\cond^2 \frac{r \log n}{n}) \leq \\
		& \cond + O(\cond^2 \sqrt{\frac{r \log n}{n}}) = O(\cond),
		\end{align*}
		under the condition $n \gtrsim \cond^2 \frac{r \log n}{n}$.
		Taking a union bound over the aforementioned events and combining terms gives the result.
\end{proof}

Finally we present a concentration result for random matrices showing concentration when the matrices are projected alongs two (potentially different) subspaces.

\begin{lemma}
	Suppose a sequence of i.i.d. covariates $\x_i$ satisfy the design assumptions in \cref{assump:sg_design}. Then, if $\A$ and $\B$ are both rank $r$ orthonormal projection matrices,	
	\begin{align*}
		\norm{(\A^\top \frac{\X^\top \X}{n} \B) - \A^\top \mSigma \B)}\leq O(\Cmax (\sqrt{\frac{r}{n}}+\frac{r}{n} + \sqrt{\frac{\log(1/\delta)}{n}} + \frac{\log(1/\delta)}{n}))
	\end{align*}
	with probability at least $1-\delta$. 
	\label{lem:two_subspace_conc}
\end{lemma}
\begin{proof}
The result follows by a standard sub-exponential tail bound and covering argument. First note that for any fixed $\u, \v \in \mathbb{S}^{r-1}$, we have that $\u^\top \A^\top \x_i$ and $\v^\top \B^\top \x_i$ are both $\sG(\sqrt{\Cmax})$. Hence for any fixed $\u, \v \in \mathbb{S}^{r-1}$, $\u^\top \A^\top \x_i \x_i^\top \B \v - \u^\top \A^\top \mSigma \B \v$ is $\sE(8 \Cmax, 8 \Cmax)$.

Now, let $S$ denote a $\epsilon$-cover of $\mathbb{S}^{r-1}$ which has cardinality at most $(\frac{3}{\epsilon})^r$ by a volume-covering argument. Hence for $\epsilon=\frac{1}{5}$,
\begin{align*}
	\Pr[\sup_{\u \in S^{r-1}, \v \in S^{r-1}}  \u^\top \A^\top \x_i \x_i^\top \B \v - \u^\top \A^\top \mSigma \B \v \geq t ] \leq 225^r \exp(- c n \min(t^2/\Cmax^2, t/\Cmax)))
\end{align*}
using a union bound over the covers and a sub-exponential tail bound. Taking $t = C \cdot \Cmax (\sqrt{\frac{r}{n}}+\frac{r}{n} + \sqrt{\frac{\log(1/\delta)}{n}} + \frac{\log(1/\delta)}{n})$ for sufficiently large $C$, shows that $225^r \exp(- c n \min(t^2/\Cmax^2, t/\Cmax)))
 \leq \delta$. Finally a standard Lipschitz continuity argument proves that,
\begin{align*}
\sup_{\u \in \mathbb{S}^{r-1}, \v \in \mathbb{S}^{r-1}} \u^\top \frac{1}{n} \sum_{i=1}^{n} \u^\top \A^\top \x_i \x_i^\top \B \v - \u^\top \A^\top \mSigma \B \v \leq \frac{1}{1-3 \epsilon} \sup_{\u \in S^{r-1}, \v \in S^{r-1}} \u^\top \A^\top \x_i \x_i^\top \B \v - \u^\top \A^\top \mSigma \B \v
\end{align*}
which gives the result.
\end{proof}


==> icml/conclusions.tex <==
%!TEX root = main.tex
\section{Conclusion}
In this paper we show how a shared linear representation may be learned and transferred between multiple linear regression tasks. We provide both upper and lower bounds on the sample complexity of learning this representation and for the problem of learning-to-learn. We believe are bounds capture important qualitative phenomena observed in real meta-learning applications absent from previous theoretical treatments. A promising direction for future work is to extend the analyses here to nonlinear models. 

==> icml/notations.tex <==
%!TEX root = main.tex

\newcommand{\pmat}[1]{\begin{pmatrix} #1 \end{pmatrix}}
\newcommand{\tld}{\tilde{d}}

% Useful
\newcommand{\sumton}{\frac{1}{n}\sum_{i=1}^{n}}
\newcommand{\sumtor}{\sum_{i=1}^{r}}
\newcommand{\barLambda}{\bar{\mLambda}}
\newcommand{\mR}{\mathbb{R}}
\newcommand{\n}{\mathbf{n}}

\newcommand{\pv}{P_{\V}}
\newcommand{\pu}{P_{\U}}
\newcommand{\pt}{P_{\cT}}


\newcommand{\barGamma}{\bar{\mGamma}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bepsilon}{\bm{\epsilon}}
\newcommand{\bkappa}{\bar{\kappa}}

\newcommand{\tkappa}{\tilde{\kappa}}
\newcommand{\tnu}{\tilde{\nu}}


\newcommand{\bE}{\mathbf{E}}
\newcommand{\C}{\mathbf{C}}
\newcommand{\hB}{\hat{\B}}
\newcommand{\hU}{\hat{\U}}
\newcommand{\hV}{\hat{\V}}
\newcommand{\halpha}{\hat{\balpha}}
\newcommand{\hSigma}{\hat{\mSigma}}
\newcommand{\DelU}{\Delta_{\U}}
\newcommand{\DelV}{\Delta_{\V}}
\newcommand{\ran}[1]{\text{range}{#1}}
\newcommand{\Cmax}{C_{\max}}
\newcommand{\Cmin}{C_{\min}}
\newcommand{\cond}{C_{\text{cond}}}
\newcommand{\vol}{\mathbf{\text{vol}}}
\newcommand{\KL}{\text{KL}}
\newcommand{\btheta}{\bm{\theta}}
\newcommand{\xstar}{\mathbf{x}_{\star}}
\newcommand{\balpha}{\bm{\alpha}}
\newcommand{\bbeta}{\bm{\beta}}
\newcommand{\ntrain}{n_{\text{train}}}
\newcommand{\ntest}{n_{\text{test}}}
\newcommand{\Gr}{\text{Gr}_{r,n}(\mR)}

% Concentration
\newcommand{\sG}{\text{sG}}
\newcommand{\sE}{\text{sE}}

% Theorems
\usepackage[colorlinks,citecolor=blue,urlcolor=black,linkcolor=blue,pdfborder={0 0 0}]{hyperref}

\usepackage[capitalize]{cleveref}  
\crefname{nlem}{Lemma}{Lemmas}
\crefname{nprop}{Proposition}{Propositions}
\crefname{ncor}{Corollary}{Corollaries}
\crefname{nthm}{Theorem}{Theorems}
\crefname{exa}{Example}{Examples}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{equation}{}{}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{claim}{Claim}
\newtheorem{corollary}{Corollary}
\newtheorem{assumption}{Assumption}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{fact}{Fact}
\theoremstyle{definition}
\newtheorem{condition}{Condition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
%\theoremstyle{remark}
\newtheorem{remark}{Remark}


% Operator

\newcommand{\vect}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\diag}{\text{diag}}
\newcommand{\mat}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\grad}{\nabla}
\newcommand{\hess}{\nabla^2}
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\fracpar}[2]{\frac{\partial #1}{\partial  #2}}
\newcommand{\Ind}[1]{\mathbbm{1}{#1}}

\newcommand{\sigmin}{\sigma_{\min}}
\newcommand{\tr}{\mathrm{tr}}
\renewcommand{\det}{\mathrm{det}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\logdet}{\mathrm{logdet}}
\newcommand{\trans}{^{\top}}
\newcommand{\poly}{\mathrm{poly}}
\newcommand{\polylog}{\mathrm{polylog}}
\newcommand{\st}{\mathrm{s.t.~}}
\newcommand{\proj}{\mathcal{P}}
\newcommand{\projII}{\mathcal{P}_{\parallel}}
\newcommand{\projT}{\mathcal{P}_{\perp}}

\newcommand{\abs}[1]{|{#1}|}
\newcommand{\norm}[1]{\|{#1} \|}
\newcommand{\fnorm}[1]{\|{#1} \|_{\text{F}}}
\newcommand{\spnorm}[2]{\| {#1} \|_{\text{S}({#2})}}
% \newcommand{\abs}[1]{\left|{#1}\right|}
% \newcommand{\norm}[1]{\left\|{#1}\right\|}
% \newcommand{\fnorm}[1]{\left\|{#1}\right\|_{\text{F}}}
% \newcommand{\spnorm}[2]{\left\| {#1} \right\|_{\text{S}({#2})}}

\newcommand{\mE}{\mathbb{E}}
\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\Var}{\text{Var}}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}



% Big O
\newcommand{\cO}{\mathcal{O}}
\newcommand{\tlO}{\tilde{O}}
\newcommand{\tlOmega}{\tilde{\Omega}}
\newcommand{\tlTheta}{\tilde{\Theta}}



% Set

%\newcommand{\mR}{\mathbb{R}}
%\newcommand{\mZ}{\mat{Z}}
%\newcommand{\mS}{\mat{S}}

%\newcommand{\Z}{\mathbb{Z}}
%\newcommand{\N}{\mathbb{N}}
%\newcommand{\R}{\mathbb{R}}
%\renewcommand{\S}{\mathbb{S}}

\renewcommand{\H}{\mathcal{H}}
\newcommand{\G}{\mathcal{G}}

\newcommand{\sigstarl}{\sigma^\star_1}
\newcommand{\sigstarr}{\sigma^\star_r}



% Matrix and Vector

\newcommand{\A}{\mat{A}}
\newcommand{\B}{\mat{B}}
\newcommand{\Bone}{\hat{\mat{B}}}
\newcommand{\Btwo}{\hat{\mat{B}}_{\perp}}
\newcommand{\Q}{\mat{Q}}
\newcommand{\mS}{\mat{S}}

\newcommand{\I}{\mat{I}}
\newcommand{\D}{\mat{D}}
\newcommand{\U}{\mat{U}}
\newcommand{\V}{\mat{V}}
\newcommand{\M}{\mat{M}}
\newcommand{\N}{\mat{N}}
\newcommand{\W}{\mat{W}}
\newcommand{\X}{\mat{X}}
\newcommand{\Y}{\mat{Y}}
\newcommand{\R}{\mat{R}}
\newcommand{\Z}{\mat{Z}}

%\newcommand{\S}{\mat{S}}

%\newcommand{\Y}{\mat{Y}}

\newcommand{\E}{\mat{E}}
\newcommand{\F}{\mat{F}}
\newcommand{\mSigma}{\mat{\Sigma}}
\newcommand{\mLambda}{\mat{\Lambda}}
\newcommand{\mGamma}{\mat{\Gamma}}
\newcommand{\e}{\vect{e}}
\renewcommand{\u}{\vect{u}}
\renewcommand{\v}{\vect{v}}
\newcommand{\w}{\vect{w}}
\newcommand{\x}{\vect{x}}
\newcommand{\y}{\vect{y}}
\newcommand{\z}{\vect{z}}
\newcommand{\g}{\vect{g}}
\newcommand{\zero}{\vect{0}}
\newcommand{\fI}{\mathfrak{I}}
\newcommand{\fS}{\mathfrak{S}}
\newcommand{\fE}{\mathfrak{E}}
\newcommand{\fF}{\mathfrak{F}}



% Special Character

\newcommand{\cF}{\mathcal{F}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cW}{\mathcal{W}}

\newcommand{\cn}{\kappa}
\newcommand{\nn}{\nonumber}

==> icml/prelim.tex <==
%!TEX root = main.tex

\section{Preliminaries}
\label{sec:prelim}

The ability of a learner to adapt to new tasks is crucial for sample-efficient inference and prediction. One of the most well-known successes of transfer learning has been in initializing neural network weights in early layers using ImageNet pre-training/features, and subsequently re-training the final layers on a new task \citep{donahue2014decaf}. However, even beyond few-shot image classification \citep{vinyals2016matching}, learning efficient data representations that can generalize to multiple, unseen tasks has also become vital in applications ranging from deep reinforcemcent learning \citep{baevski2019cloze}, to natural language processing \citep{ando2005framework, liu2019multi}.

There has been a recent resurgence of interest in developing (and understanding) generic algorithms for transfer (or ``meta") learning applicable in diverse domains \citet{finn2017model}. Surprisingly, despite a long line work on transfer learning, there are  few efficient algorithms for feature learning that \textit{provably} generalize to new, unseen tasks. Sharp guarantees are even lacking in the \textit{linear} setting. Indeed, formally characterizing the goal of learning a transferrable representation remains nontrivial. 

In this paper, we attack the problem of ``meta"-learning features in a linear model in which multiple tasks share a common set of low-dimensional features.
Our aim is twofold. First, given a set of diverse samples from $t$ different tasks we ask how we can efficiently (and optimally) learn a common feature representation? Second, having learned a common feature representation, how can we use this representation to improve sample efficiency in a new ($t+1$st) task where data may be scarce\footnote{This problem is sometimes referred to as learning-to-learn (LTL).}? 

Formally given an (unobserved) linear feature matrix $\B = ( \bb_1, \ldots, \bb_r )\in \mR^{d\times r}$ with orthonormal columns, our statistical model for data pairs $(\x_i, y_i)$ is:
\begin{equation}\label{eq:model_main}
y_i = \x_i\trans \underbrace{\B\balpha_{t(i)}}_{\bbeta_{t(i)}}  + \epsilon_i
\end{equation}
where there are $t$ (unobserved) underlying task parameters $\balpha_i$ for $i \in \{1, \hdots, t \}$. Here $\balpha_{t(i)} \in \mR^r$ is the task associated with the $i$th datapoint, $\x_i \in \mR^d$ is a random covariate, and $\epsilon_i$ additive noise. We assume the sequence $\{\balpha_{t(i)}\}_{i=1}^\infty$ is independent of all other randomness in the problem. In this framework, the aforementioned questions reduce too recovering $\B$ from data from the first $\{1, \hdots, t\}$ tasks, and using this feature representation to recover a better estimate of a new task parameter $\bbeta_{t+1} = \B \balpha_{t+1}$ (where $\balpha_{t+1}$ is also unobserved).
 
 Our main result which targets the problem of learning-to-learn (LTL), shows how a feature representation $\Bone$ learned from $t$ diverse tasks can improve learning on a unseen $t+1$st task which shares the same underlying linear representation. We informally state this result  below\footnote{This follows immediately from combining \cref{thm:B_recovery,,thm:lr_transfer}; see \cref{thm:main_formal} for a formal statement.},
\begin{theorem}[Informal]
	Suppose we are given $n_1$ total samples from $t$ diverse tasks which are used in \cref{algo:LF_learn} to learn a feature representation $\Bone$, and $n_2$ samples from a new $t+1$st task which are used along with $\Bone$ and \cref{algo:LF_newtask} to learn parameters $\halpha$ of new $t+1$st task. Then the parameter $\Bone \halpha$ has excess prediction error on a new test point $\xstar$ drawn from the training data covariate distribution of,
	\begin{align}
		\mE_{\xstar}[\langle \xstar, \Bone \halpha - \B \balpha_{t+1} \rangle^2] \leq \tlO \left(\frac{dr}{n_1} + \frac{r}{n_2} \right)	 \label{eq:main_informal}
	\end{align}
	with high probability over the training data.
	\label{thm:main_informal}
\end{theorem}
The naive complexity of linear regression which ignores the information from the previous $t$ tasks has complexity $O(\frac{d}{n_2})$. \cref{thm:main_informal} suggests that ``positive" transfer from the first $\{1, \hdots, t \}$ tasks to the final $t+1$st task can dramatically reduce the sample complexity of learning when $r \ll d$ and $\frac{n_1}{n_2} \gg r$ -- that is when 1. the complexity of the shared representation is much smaller then the dimension of the underlying space and 2. when the ratio of the number of samples used for feature learning to the number of samples present for a new unseen task exceeds the complexity of the shared representation. We believe the LTL bound in \cref{thm:main_informal} is the first bound, even in the \textit{linear} setting, to sharply exhibit this phenomena (see \cref{sec:comparisons} for a comparison to existing results). Our primary contributions in this paper are to:
\begin{itemize}[leftmargin=.5cm]
	\item Provide a method-of-moments estimator which can efficiently aggregate information across multiple differing task to estimate $\B$ -- even when it may be information-theoretically impossible to learn the parameters of any given task (see \cref{sec:lf_mom}).
	\item Understand the bias-variance trade-offs of the linear regression estimator loaded with a biased, feature estimate to demonstrate the benefits and pitfalls of transferring learned representations to new, unseen tasks (see \cref{sec:new_task}).
	\item Present a local landscape analysis of the empirical risk induced by \cref{eq:model_main} which suggests first-order methods can learn feature representations which also generalize well (see \cref{sec:lf_gd}).
	\item Show an (asymptotic) minimax lower bound for the problem of feature learning, showing the aforementioned estimator optimally estimates $\B$ up to logarithmic factors. To our knowledge, this is the first information-theoretic lower bound for feature learning (see \cref{sec:lf_lb}).
\end{itemize}

\textbf{Notation and Assumptions.}
Throughout, we will use bold lower-case letters (e.g., $\x$) to refer to vectors and bold upper-case letters to refer to matrices (e.g., $\X$). We exclusively use $\B \in \mR^{d \times r}$ to refer a matrix with orthonormal columns spanning an $r$-dimensional feature space, and $\B_{\perp}$ to refer a matrix with orthonormal columns spanning the orthogonal subspace of this feature space. The norm $\Vert \cdot \Vert$ appearing on vector or matrix refers to its $\ell_2$ norm or spectral norm respectively. $\fnorm{\cdot}$ on a matrix is its Frobenius norm. $\langle \x, \y \rangle$ is the Euclidean inner product, while $\langle \M, \N \rangle = \tr(\M \N^\top)$ is the inner product between matrices. Generically, we will use ``hatted" vectors and matrices (e.g, $\halpha$ and $\Bone$) to refer to (random) estimators of their underlying population quantities. We will use $\gtrsim$, $\lesssim$, and $\asymp$ to denote greater than, less than, and equal to up to a universal constant and use $\tlO$ to denote an expression that hides polylogarithmic factors in all problem parameters.

Formally, an orthonormal feature matrix $\B$ is an element of an equivalence class (under right rotation) of a representative lying in $\Gr$ -- the Grassmann manifold \citep{edelman1998geometry}. The Grassmann manifold, consists of the the set of $r$-dimensional subspaces within the underlying $d$-dimensional space,  we denote as $\Gr$. To define distance in $\Gr$ we define the notion of a principal angle between two subspaces $p$ and $q$. If $\C$ is an orthonormal matrix whose columns form orthonormal basis of $p$ and $\D$ is an orthonormal matrix whose columns form an orthonormal basis of $q$, then singular value of decomposition of $\C_{\perp}^\top \D = \U \D \V^\top$ defines the principal angles as,
\begin{align*}
	\D = \diag(\sin \theta_1, \sin \theta_2, \hdots, \sin \theta_k)
\end{align*}
where $0 \leq \theta_k \leq \hdots \leq \theta_1 \leq \frac{\pi}{2}$. The distance of interest for us will be the subspace angle distance $\sin \theta_1$, and for convenience we will use the shorthand $\sin \theta(\C, \D)$ to refer to it. With some abuse of notation we will use $\B$ to refer an explicit orthonormal feature matrix and the subspace in $\Gr$ it represents.

We now detail several assumptions we use in our analysis.
\begin{assumption}[Gaussian Design and Noise]
The zero-mean i.i.d. covariate vectors $\x_i \sim \cN(0, 1)$. Moreover, the additive noise $\epsilon_i$ is i.i.d. sub-gaussian with variance parameter $1$ and independent of $\x_i$.
  \label{assump:design}
\end{assumption}

Throughout we work in the setting of random design linear regression, and in this context \cref{assump:design} is standard. With the exception of \cref{thm:B_recovery}, our results do not rely critically rely the Gaussian design assumption although its use simplifies several technical arguments. 
In the following we define the population task diversity matrix as $\A = (\balpha_1, \hdots, \balpha_t)^\top \in \mR^{t \times r}$, $\nu= \sigma_r(\frac{\A^\top \A}{t})$, and the average condition number as $\bkappa = \frac{\tr(\frac{\A^\top \A}{t})}{r \nu}$.
\begin{assumption}[Task Diversity and Normalization]
\label{assump:task}
The $t$ underlying task parameters $\balpha_j$ satisfy $\norm{\balpha_j} = \Theta(1)$ for all $j \in \{1, \hdots, t\}$. Moreover, we assume $\nu > 0$.
\end{assumption}

Recovering the feature matrix $\B$ is impossible without structural conditions on $\A$. Consider the extreme case in which $\balpha_{1}, \hdots, \balpha_{t}$ are restricted to span only the first $r-1$ columns of the column space of the feature matrix $\B$. None of the data points $(\x_i, y_i)$ contain any information about the $r$th column-feature which can be any arbitrary vector in the complementary $d-r-1$ subspace. In this case recovering $\B$ accurately is information-theoretically impossible. The parameters $\nu$ and $\bkappa$ capture how ``spread-out" in the column space of $\B$ the tasks $\balpha_j$ are. The condition $\norm{\balpha_j}=\Theta(1)$ is also standard in the statistical literature and is equivalent normalizing the signal-to-noise ratio to be $\Theta(1)$.

\subsection{Related Work}
\label{sec:related_work}
While their is a vast literature on papers proposing multi-task and transfer learning methods, the number of theoretical investigations is much fewer. Understanding the statistical sample complexity of the questions\footnote{often referred to as learning-to-learning, continual learning, meta-learning, and multi-task learning.} we address here dates back to \citet{baxter2000model}, who studied a model where tasks with shared representations are sampled from the same underlying ``environment". \citet{ando2005framework} phrase multi-task learning as a semi-supervised learning problem with ``fake" tasks; however their bounds do not imply generalization to new, unseen tasks. \citet{pontil2013excess, maurer2016benefit} develop a generic framework to prove generalization bounds in the multi-task and learning-to-learn setting most closely related to ours, using tools from empirical process theory. Note all of the aforementioned works do not address the algorithmic component of meta-learning as their generalization guarantees rely on an empirical risk minimization (ERM) oracle to solve a generically \textit{non-convex} optimization problem.  
Recently, \citet{bullins2019generalize} developed an efficient online learning approach to learn linear embeddings within a \textit{discriminative} model, which can indirectly generalize across a distribution of tasks. The setting is distinct from ours and not directly comparable. However, one principal difference between our results is that \citet[Theorem 2]{bullins2019generalize} guarantees the excess-per-task loss evaluated on a feature representation learned from $t$ tasks with $n_t$ samples per task, decays as $\tlO(\frac{1}{\sqrt{t}})$ -- which does not improve as $n_t$ increases.

There has also been line of recent work providing guarantees for gradient-based meta-learning (MAML) \citep{finn2017model}. \citet{finn2019online, khodak2019provable,  denevi2019learning} work in the framework of online convex optimization (OCO)  and use a notion of task similarity assuming closeness of all tasks to a single fixed point in parameter space to provide guarantees. \citet{khodak2019adaptive} strengthens earlier meta-learning guarantees in the OCO framework and provides bounds with more general notions of data-dependent task similarity. In contrast to these works, we focus on the setting of  learning a \textit{representation} common to all tasks in a generative model. The task model parameters need not be close together in our setting.
\subsubsection{Comparisons to Related Work}
\label{sec:comparisons}

The closest guarantees to ours in \cref{thm:main_informal} we are aware of are from \citet{maurer2016benefit}. \citet[Theorem 5]{maurer2016benefit} instantiated in our setting (where $n_1=n_2=n$) provide a LTL guarantee showing the excess risk of the loss function with learned representation on a new datapoint is bounded by $\tlO(\frac{r \sqrt{d}}{\sqrt{t}} + \sqrt{\frac{r}{n}})$ w.h.p. The most striking difference between \cref{eq:main_informal} and this aforementioned guarantee is that the leading term capturing the complexity of learning the feature representation decays \textit{only in} $t$ \textit{not in} $n$ (which can be much larger then $t$). We believe for many applications (including the linear model herein) their analysis is too pessimistic to reflect the efficacy of meta-learning techniques. In practice, transfer learning is often successful even when we are presented with only a few training tasks but each with a significant number of samples per task (e.g., $n_1 \gg t$)\footnote{See \cref{fig:easy_task_n_train_change} for a numerical simulation relevant to this setting.}.
	The power of the framework of \citet{maurer2016benefit} is its generality, which extends beyond the linear setting. However, we believe their guarantee is weaker then that in \cref{thm:main_informal} because 1. they rely on uniform convergence arguments which do not leverage structure between the underlying covariates $\x$ or the potential diversity of tasks and 2. they work in a general model where tasks are sampled from an environment to provide guarantees only on the excess risk of the task-averaged loss -- which sidesteps the questions of whether an accurate estimate of the underlying feature representation (measured in the distance in the feature space) can be recovered. 
\vspace{-0.3cm}

==> icml/simulations.tex <==
%!TEX root = main.tex
\section{Simulations}
We complement our theoretical analysis with a series of numerical experiments highlighting the benefits (and limits) of meta-learning.
For the purposes of feature learning we compare the performance of the method-of-moments estimator in \cref{algo:LF_learn} vs. directly optimizing the objective in \cref{eq:objective_main}. Additional details on our set-up are provided in \cref{sec:app_expt}.  
We construct problem instances by generating Gaussian covariates and noise as $\x_i \sim \cN(0, \I_d)$, $\epsilon_i \sim \cN(0, 1)$, and the tasks and features used for the first-stage feature estimation as $\balpha_i \sim \frac{1}{\sqrt{r}} \cdot \cN(0, \I_r)$, with $\B$ generated as a (uniform) random $r$-dimensional subspace of $\mR^d$. In all our experiments we generate an equal number of samples $n_t$ for each of the $t$ tasks, so $n_1 = t \cdot n_t$. In the second-stage we generate a new, $t+1$st task instance using the same feature estimate $\B$ used in the first-stage and otherwise generate $n_2$ samples, with the covariates, noise and $\balpha_{t+1}$ constructed as before. Throughout this section we refer to features learned via the first-order method as LF-FO and the corresponding meta-learned regression parameter on a new task as obtained by meta-LR-FO. We use LF-MoM and meta-LR-MoM to refer to the same quantities save with the feature estimate learned via the method-of-moments estimator. We also use LR to refer to the baseline linear regression estimator on a new task which only uses data generated from that task.  

We begin by considering a challenging setting for feature learning where $d=100$, $r=5$, but $n_t=5$ for varying numbers of tasks $t$. 
\begin{figure}[!ht]
\centering
\begin{minipage}[c]{.45\linewidth}
\includegraphics[width=\linewidth]{Plots/angle,d=100,r=5,train_n=5,test_n=2500.pdf}
\end{minipage}
\begin{minipage}[c]{.45\linewidth}
\includegraphics[width=\linewidth]{Plots/synthetic,d=100,r=5,train_n=5,test_n=2500.pdf}
\end{minipage}
\caption{Left: LF-FO vs. LF-MoM estimator with error measured in the subspace angle distance $\sin \theta(\Bone, \B)$. Right: meta-LR-FO and meta-LR-MoM vs. LR on new task with error measured on new task parameter. Here $d=100$, $r=5$, and $n_t = 25$ while $n_2=25$ as the number of tasks is varied.
}
\label{fig:hard_task_change}
\vspace{-.5cm}
\end{figure}

As \cref{fig:hard_task_change} demonstrates, the method-of-moments estimator is able to aggregate information across the tasks as $t$ increases to slowly improve its feature estimate even though $n_t \ll  d$. The loss-based approach struggles to improve its estimate of the feature matrix $\B$ in this regime. In this setting, we also generated a $t+1$st test task with $d \ll n_2 = 2500$, to test the effect of meta-learning the linear representation on generalization in a new, unseen task against a baseline which simply performs on regression on this new task in isolation. \cref{fig:hard_task_change} also shows that meta-learned regressions perform significantly worse then simply ignoring first $t$ tasks. \cref{thm:lr_transfer} indicates the bias from the inability to learn an accurate feature estimate of $\B$ overwhelms the benefits of transfer learning. 
In this regime $n_2 \gg d$ so the new task can be efficiently learned in isolation.  
We believe this simulation represents a simple instance of the empirically observed phenomena of ``negative" transfer \citep{wang2019characterizing}.

We now turn to the more interesting use cases where meta-learning is a powerful tool. We consider a setting for feature learning $d=100$, $r=5$, and $n_t=25$ for varying numbers of tasks $t$. However, now we consider a new, unseen task where data is scarce $n_2=25 < d$.
\begin{figure}[!ht]
\vspace{-0.25cm}
\centering
\begin{minipage}[c]{.45\linewidth}
\includegraphics[width=\linewidth]{Plots/angle,d=100,r=5,train_n=25,test_n=25.pdf}
\end{minipage}
\begin{minipage}[c]{.45\linewidth}
\includegraphics[width=\linewidth]{Plots/synthetic,d=100,r=5,train_n=25,test_n=25.pdf}
\end{minipage}
\caption{Left: LF-FO vs. LF-MoM estimator with error measured in the subspace angle distance $\sin \theta(\Bone, \B)$. Right: meta-LR-FO and meta-LR-MoM vs. LR on new task with error measured on new task parameter. Here $d=100$, $r=5$, $n_t = 25$ while $n_2=25$ while the number of tasks is varied.
}
\label{fig:easy_task_t_change}
\vspace{-0.25cm}
\end{figure}
As \cref{fig:easy_task_t_change} shows in this regime both the method-of-moments estimator and loss-based approach can learn a non-trivial estimate of the feature representation. The benefits transferring this representation are also evident in the improved generalization performance seen by the meta-regression procedures on the new task. Interestingly, the loss-based approach learns an accurate feature representation $\Bone$ with significantly fewer samples then in the previous task.

Similarly if we consider an instance where $d=100$, $r=5$, $t=20$, and $n_2=50$ with varying numbers of training points $n_t$ per task, we similarly see that meta-learning representations provides significant value in a new task in \cref{fig:easy_task_n_train_change}. Note that these numerical experiments show that as the number of tasks is fixed, but $n_t$ increases the generalization of ability of the meta-learned regressions significantly improves as reflected in the bound \cref{eq:main_informal}. As in the previous experiment, the loss-based approach is more sample-efficient then the method-of-moments estimator. 
\begin{figure}[!ht]
\centering
\begin{minipage}[c]{.45\linewidth}
\includegraphics[width=\linewidth]{Plots/angle,d=100,r=5,T=20,test_n=50.pdf}
\end{minipage}
\begin{minipage}[c]{.45\linewidth}
\includegraphics[width=\linewidth]{Plots/synthetic,d=100,r=5,T=20,test_n=50.pdf}
\end{minipage}
\caption{Left: LF-FO vs. LF-MoM estimator with error measured in the subspace angle distance $\sin \theta(\Bone, \B)$. Right: meta-LR-FO and meta-LR-MoM vs. LR on new task with error measured on new task parameter. Here $d=100$, $r=5$, $t=20$, and $n_2=50$ while the number of training points per task ($n_t$) is varied.
}
\label{fig:easy_task_n_train_change}
\vspace{-0.3cm}
\end{figure}
\vspace{-0.4cm}

==> icml/test.tex <==
%!TEX root = main.tex

\section{Transferring Features to New Tasks}
\label{sec:new_task}
\vspace*{-0.2cm}
\begin{algorithm}[!t]
\caption{Linear Regression for Learning a New Task with a Feature Estimate}\label{algo:LF_newtask}
\begin{algorithmic}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\REQUIRE $\Bone, \{ (\x_i, y_i) \}_{i=1}^{n_2}$.
\STATE $\halpha \leftarrow (\sum_{i=1}^{n_2} \Bone \x_i \x_i^\top \Bone^\top)^{\dagger} \Bone^\top \sum_{i=1}^{n_2} \x_i y_i$
\STATE \textbf{return} $\halpha$
\end{algorithmic}
\end{algorithm}
Having estimated a linear feature representation $\Bone$ shared across related tasks, our second goal is to use this representation to improve learning in a new, unseen task (the $t+1$st task). In the context of the model in \cref{eq:model_main}, the approach taken in \cref{algo:LF_newtask} uses $\Bone$ as a plug-in surrogate to the unknown $\B$, and attempts to estimate $\balpha_{t+1} \in \mR^{r}$.  Formally we define our estimator $\balpha$ as,
\begin{align}
	\halpha = \arg \min_{\balpha} \norm{\y - \X \Bone \balpha}^2	 \label{eq:lr_red}
\end{align}
where $n_2$ samples $(\X, \y)$ are generated from the model in \cref{eq:model_main} from the $t+1$st task. Effectively, the feature representation $\Bone$ performs dimension-reduction on the input covariates $\X$, allowing us to learn in a lower-dimensional space. Since the optimization problem in \eqref{eq:lr_red} is simply an ordinary least-squares objective, not only can it be analytically solved as in \cref{algo:LF_newtask}, but is also amenable to fast, high-precision optimization by gradient-based methods\footnote{Under the conditions in \cref{assump:design}, in the regime $n \gtrsim r$, $\sigma_{\min}(\X \Bone) \geq \Omega(1)$ w.h.p. and hence the objective can be optimized with first-order methods to precision $\epsilon$ in $O(\log(\frac{1}{\epsilon}))$ iterations \citep{bubeck2015convex}.}. 

Hence, our focus is on understanding the generalization properties of the estimator in \cref{algo:LF_newtask}. Assuming we have produced an estimate $\Bone$ of the true feature matrix $\B$ we can present our main result on the sample complexity of meta-learned linear regression. 
\begin{theorem}
	Suppose $n_2$ data samples $\{ (\x_i, y_i) \}_{i=1}^{n_2}$, are generated from the model in \eqref{eq:model_main} where \cref{assump:design} holds, from a single task satisfying $\norm{\balpha_{t+1}}^2 \leq O(1)$. Then, if $\sin(\Bone, \B) \leq \delta$ and $n_2 \gtrsim  r \log n$, the output $\halpha$ from \cref{algo:LF_newtask} satisfies
	\begin{align}
		\norm{\Bone \halpha-\B \balpha_{t+1}}^2 \leq \tlO \left( \frac{r}{n_2} + \delta^2 \right), \label{eq:transfer_guarantee}
	\end{align}
	with probability at least $1-O(n_2^{-100})$.
	\label{thm:lr_transfer}
\end{theorem}
Note that $\B \balpha_{t+1}$ is simply the underlying parameter in the regression model in \cref{eq:model_main}. We make several remarks about this result,
\begin{itemize}[leftmargin=.5cm]
	\vspace{-0.3cm}
	\item \cref{thm:lr_transfer} decomposes the error of transfer learning into two components. The first term $\tlO(\frac{r}{n_2})$ in \cref{eq:transfer_guarantee} arises from the variance of learning in a space of reduced dimensionality. The second term $\tlO(\delta^2)$ arises from the bias of using an imperfect feature estimate $\Bone$ to transfer knowledge across tasks. 
	\item Standard generalization guarantees for random design linear regression ensure the parameter recovery error is bounded by $O(\frac{d}{n_2})$ w.h.p. under the same assumptions \citep{hsu2012random}. Meta-learning the linear representation $\Bone$ can provide a significant reduction in the sample complexity of learning when $\delta^2 \ll \frac{d}{n_2}$ and $r \ll d$. 
	\item Conversely, if $\delta^2 \gg \frac{d}{n_2}$ the bounds in \cref{eq:transfer_guarantee} imply the overhead of learning the feature representation may overwhelm the potential benefits of transfer learning (with respect to baseline of learning the $t+1$st task in isolation). This accords with the well-documented empirical phenomena of ``negative" transfer observed in large-scale deep learning problems where meta/transfer-learning techniques actually result in a degradation in performance on new tasks \citep{wang2019characterizing}. Using \cref{algo:LF_learn} to estimate $\Bone$ suggests that ensuring $\delta^2 \ll \frac{d}{n_2}$ where $\delta^2 = \tlO(\frac{dr}{n_1})$ requires $\frac{n_1}{n_2} \gg r$. That is, the ratio of the number of samples used for feature learning to the number of samples used for learning the new task should exceed the complexity of the feature representation to achieve ``positive" transfer.
	\vspace{-0.3cm}
\end{itemize}
In order to obtain the rate in \cref{thm:lr_transfer} we use a direct analysis of the estimator error $\Bone \halpha-\B \balpha_{t+1}$ (and do not appeal to uniform convergence arguments). Using the definition of the $\y$ we can write the error as,
\begin{align*}
	& \Bone\halpha-\B \balpha_0 = \Bone (\Bone^\top \X^\top \X \Bone)^{-1} \Bone \X^\top \X \B \balpha_0 - \B \balpha_0 + \\
	& \Bone(\Bone^\top \X^\top \X \Bone)^{-1} \Bone^\top \X^\top \bepsilon
\end{align*}
The first term contributes the bias term to \cref{eq:transfer_guarantee} while the second contributes the variance term. 
Analyzing the fluctuations of the (mean-zero) variance term can be done controlling the norm of its square -- $\bepsilon^\top \A \bepsilon$ where $\A = \X \Bone (\Bone^\top \X^\top \X \Bone)^{-2} \Bone^\top \X^\top$. We can bound this (random) quadratic form by first appealing to the Hanson-Wright inequality to show w.h.p. that $\bepsilon^\top \A \bepsilon \lesssim \tr(\A) + \tlO(\fnorm{\A} + \norm{\A})$. The remaining randomness in $\A$ can be controlled using matrix concentration/perturbation arguments (see \cref{lem:test_bias}).

With access to the true feature matrix $\Bone$ (i.e. setting $\Bone=\B$) the term $\Bone (\B^\top \X^\top \X \B)^{-1} \B \X^\top \X \B \balpha_0 - \B \balpha_0 = 0$, due to the cancellation in the empirical covariance matrices -- $(\B^\top \X^\top \X \B)^{-1} \B \X^\top \X \B = \I_r$. This cancellation of the empirical covariance is essential to obtaining a tight analysis of the least-squares estimator. We cannot rely on this effect in full since $\Bone \neq \B$. However, a naive analysis which splits these terms, $(\Bone^\top \X^\top \X \Bone)^{-1}$ and $\Bone \X^\top \X \B $ can lead to a large increase in the variance in the bound. To exploit the fact $\Bone \approx \B$, we project the matrix $\B$ in the leading $\X \B$ term onto the column space of $\Bone$ and its complement -- which allows a partial cancellation of the empirical covariances in the subspace spanned by $\Bone$. The remaining variance can be controlled as in the previous term (see \cref{lem:test_var}).
\vspace{-0.3cm}

==> icml/train_gd.tex <==
%!TEX root = main.tex
\section{The Landscape of Feature Learning}
\label{sec:lf_gd}
The remarkable, practical success of first-order methods for training non-convex optimization problems (including meta/multi-task learning objectives) motivates us to study the optimization landscape of the empirical risk induced by the model in \eqref{eq:model_main}. While a comprehensive analysis of the global landscape of solutions is beyond the scope of this paper, we present evidence that first-order methods can find \textit{local minima that generalize well}. 

Jointly learning the population parameters $\B$ and $(\balpha_1, \hdots, \balpha_t)^\top$ defined by \cref{eq:model_main} is remniscent of a matrix sensing/completion problem and we leverage this connection for our analysis \citep{ge2017no}. Throughout this section assume that we are in a uniform task sampling model -- at each iteration the task $t(i)$ for the $i$th datapoint is uniformly sampled from the $t$ underlying tasks. We first recast our problem in the language of matrices, by defining the matrix we hope to recover as $\M_{\star} = (\balpha_1, \hdots, \balpha_t)^\top \B^\top  \underbrace{=}_{\text{SVD}} \X^{\star} \D^{\star} (\Y^{\star})^\top \in \mR^{t \times d}$,  $\U^{\star}=\X^{\star} (\D^{\star})^{1/2}$, $\V^{\star} = (\D^{\star})^{1/2} \Y^{\star}$ and letting $\sigstarl$ and $\sigstarr$ denote the $1$st and $r$th singular values of $\M^{\star}$ and $\kappa^{\star}=\sigstarl/\sigstarr$ its condition number. In this notation, we see the observations\footnote{We rescaled the model and introduce a noise scale $\sigma$ here for convenience.},
\begin{align}
	y_i = \langle \sqrt{t} \e_{t(i)} \x_i^\top, \M_{\star} \rangle + \sqrt{t} \sigma \cdot \epsilon_i
\end{align}
To frame recovery as an optimization problem we consider the Burer-Monteiro factorization of the parameter $\M = \U \V^\top$, which motivates the objective, 
\begin{align}
	& \min_{\U \in \mR^{t \times r}, \V \in \mR^{d \times r}} f(\U, \V) \quad \text{where} \ f(\U, \V) = \label{eq:objective_main} \\
	& \frac{2}{n} \sum_{i=1}^{n} (y_i-\sqrt{t} \langle \e_{t(i)} \x_i^\top , \U \V^\top \rangle)^2 +  \frac{1}{2}\fnorm{\U^\top \U-\V^\top \V}^2 \nonumber.
\end{align}
The second term in \cref{eq:objective_main} functions as a regularization to prevent solutions which send $\fnorm{\U} \to 0$ while $\fnorm{\V} \to \infty$. If the value of this objective \cref{eq:objective_main} is small we might hope that an estimate of $\B$ can be extracted from the column space of the parameter $\V$, since the column space of $\V^{\star}$ spans the same subspace as $\B$. Informally, our main result states that all local minima of the regularized \textit{empirical} risk in the neighborhood of the optimal $\V^{\star}$ have subspaces that approximate $\B$ well. Before stating our result we define the local ``incoherence" set as,
\begin{align*}
& \cW = \{~ (\U, \V) ~|~ \max_{i\in[t]} \norm{\e_i\trans \U}^2 \le \frac{C_0 \bkappa r \sigstarl}{t}, \\
& \quad \norm{\U}^2 \le C_0 \sigstarl, \quad \norm{\V}^2 \le C_0 \sigstarl ~\}
\label{eq:constraint_main}
\end{align*}
for some large constant $C_0$. This set contains the optimal parameters\footnote{Note $\U^{\star}$ and $\V^{\star}$ satisfy the final two constraints by definition and \cref{lem:diverse_to_incoh} can be used to show that that \cref{assump:task} actually implies $\U^{\star}$ satisfies the first incoherence-like constraint.} under \cref{assump:task}. Our main result then becomes, 
\begin{theorem}\label{thm:main_landscape_convert}
Let \cref{assump:design,,assump:task} hold in the uniform task sampling model. If the number of samples $n_1$ satisfies $n_1 \gtrsim \polylog(n_1,d,t) \bkappa^2 r^4 \max\{t, d\}  (\cn^\star)^4$, then with probability at least $1-1/\poly(d)$, we have that given any local minimum $(\U, \V) \in \text{int}(\cW)$ of the objective \cref{eq:objective_main}, the column space of $\V$, spanned by the orthonormal feature matrix $\Bone$, satisfies:
\begin{equation*}
\sin \theta(\Bone, \B) \leq O \left( \frac{\sigma}{\sqrt{\nu}} \sqrt{\frac{\max\{t, d\} r\log n_1}{n_1}} \right).
\end{equation*}
\end{theorem}
We make several comments on this result,
\vspace{-0.3cm}
\begin{itemize}[leftmargin=.5cm]
	\item In short, the guarantee in \cref{thm:main_landscape_convert} suggests the local optimization landscape near $\M^{\star}$ will not inhibit generalization. \cref{thm:feature_lb} guarantees any estimator (including the empirical risk minimizer) must incur error $\gtrsim \sqrt{\frac{d r}{n}}$. In the regime $t \leq O(d)$, \cref{thm:main_landscape_convert}, ensures with enough samples $n_1 \gtrsim \poly(r) d$, all local minima are at most $\tlO(\sqrt{\frac{dr}{n_1}})$ away from the true solution. Thus, the error from finding a local minima of the empirical risk -- contained in the set $\text{int}(\cW)$ -- is of roughly the same order as the statistical generalization error.
	\item Recent work in \citet{jin2017escape} shows that (noisy) gradient descent can efficiently escape strict saddle points to find local minima. While \cref{thm:main_landscape_convert} does not fully characterize the global geometry of the objective, we believe in conjunction with the previous result provides preliminary evidence that first-order methods can efficiently meta-learn linear features. 
	\vspace{-0.2cm}
\end{itemize}
The proof of \cref{thm:main_landscape_convert} is technical so we only sketch the high-level ideas. The overall strategy is to analyze the Hessian of the objective \cref{eq:objective_main} at a stationary point $(\U, \V)$ in $\text{int}(\cW)$ to exhibit a direction $\Delta$ of negative curvature which can serve as a direction of local improvement pointing towards $\M^{\star}$ (and hence show $(\U, \V)$ is not a local minimum). Implementing this idea requires surmounting several technical hurdles including 1. establishing various concentration of measure results (e.g., RIP-like conditions) for the sensing matrices $\sqrt{t} \e_{t(i)} \x_i^\top$ unique to our setting and 2. handling the interaction of the optimization analysis with the regularizer and noise terms. Performing this analysis establishes that under the aforementioned conditions all local minima in $\text{int}(\cW)$ satisfy, $
	\norm{\U\V^\top - \M^\star}_F\leq O(\sigma\sqrt{t\frac{\max\{t, d\} r\log n}{n}})
$
(see \cref{thm:main_landscape}).
Guaranteeing this loss is small is not sufficient to ensure recovery of the underlying features. Transferring this guarantee in the Frobenius norm to a result on the subspace angle critically uses the task diversity assumption (see \cref{lem:frob_to_angle}) to give the final result.
\vspace{-0.3cm}

==> icml/train_lb.tex <==
%!TEX root = main.tex
\section{Lower Bounds for Feature Learning}
\label{sec:lf_lb}
To complement the upper bounds provided by the aforementioned estimators, here we demonstrate the information-theoretic limits of feature learning in the model \cref{eq:model_main}. To our knowledge, this is the first sample-complexity lower bound for feature learning in the multi-task setting.  
While, there is existing literature on (minimax)-optimal estimation of low-rank matrices (see for example \citet{rohde2011estimation}), this work focuses on the (high-dimensional) estimation of matrices, whose only constraint is to be low-rank. Moreover, error is measured in the additive prediction norm. In our setting, we must handle the additional difficulties that arising from the fact that we are interesting in 1. learning a column space (i.e. an element in the $\Gr$) and 2. that error between such representatives is measured in the subspace angle distance. We begin by presenting our (asymptotic) lower bound for feature recovery.

\begin{theorem}
	Suppose a total of $n$ data samples are generated from the model in \eqref{eq:model_main} satisfying \cref{assump:design} with $\epsilon_i \sim \cN(0, 1)$, with an equal number from each task, and that \cref{assump:task} holds with $\balpha_j$ for each task normalized to $\norm{\balpha_i}=1$ and $\nu \geq \Omega(1)$. Fix $r \geq 2$, a constant integer $k > 2$, and set $n = k \cdot r d$. Then for sufficiently large $d$ (which may depend on $r, k$) we have that,
	\begin{align*}
		\inf_{\Bone} \sup_{\B \in \Gr} \sin \theta(\Bone, \B) \geq \Omega \left(\sqrt{\frac{dr}{n}} \right)
	\end{align*} 
 with probability at least $\frac{1}{100}$, where the infimum is taken over the class of estimators that are functions of the $n$ data samples.
 \label{thm:feature_lb}
\end{theorem}
Before diving into the technical analysis we make several comments on the result.
\begin{itemize}[leftmargin=.5cm]
	\vspace{-0.3cm}
	\item The result of \cref{thm:feature_lb} shows that the estimator in \cref{algo:LF_learn} provides a minimax-optimal estimator of the feature representation parametrized by $\B$ (up to logarithmic factors) when $\nu \geq \Omega(1)$. 
	\item The dimension of the $\Gr$ (i.e. the number of free parameters needed to specify a feature set) is $r(d-r) \geq \Omega(dr)$ as $d \to \infty$; hence in the high-dimensional limit \cref{thm:feature_lb} matches the rate we intuit from parameter counting.
	\item \cref{thm:feature_lb} requires fixing $r$ and the ratio $\frac{n}{dr}$, and then taking $d$ to be sufficiently large. The particular order of the quantifiers here arises from the difficulty of obtaining an tight estimate of the (local) packing number of $\Gr$ used in (local) Fano method. Our proof exploits the simplifications to the complex geometry of the Grassmann manifold that occur in the high-dimensional limit to approximately compute this packing number.
	\vspace{-0.3cm}
\end{itemize}
We now present an overview of the proof strategy which relies on the (local) Fano method we restate for convenience.
In the following, we let $\rho$ denote a semi-metric on the underlying space $\Theta$, $\hat{\theta}$ an estimator of $\theta$, and $\Phi$ an increasing function.
\begin{proposition}[Fano method]
	Let $\{ \theta^{1}, \hdots, \theta^{M} \}$ be a $2\delta$-separated set in the $\rho$ semi-metric on $\Theta$, and suppose $J$ is uniformly distributed over the index set $\{1, \hdots, M \}$ and $(Z | J=j) \sim \Pr_{\theta^{j}}$. Then for any increasing function $\Phi : [0, \infty) \to [0, \infty)$, the minimax risk is lower bounded as,
\begin{align}
\inf_{\hat{\theta}} \sup_{\theta \in \Theta} \Pr_{\theta}[\Phi(\rho(\hat{\theta}, \theta)) \geq \Phi(\delta)] \geq 1-\frac{I(Z;J)+\log 2}{\log M}, \nonumber
\end{align}
where $I(Z;J)$ denotes the mutual information between $Z$ and $J$.
\label{prop:fano}
\end{proposition}
 There are two key ingredients to obtaining a tight lower bound. First, we must to exhibit a large family of distinct, well-separated feature matrices $\{ \B_i \}_{i=1}^M$  (i.e. a packing) -- to show $\log M$ is large. Second, we must argue this set of feature matrices induces a family of distributions over data $\{ (\x_i, y_i) \}_{B_i}$ which are statistically ``close" and fundamentally difficult to distinguish between -- as captured by the fact $I(Z;J)$ is small.
 
The first and most technical step in our argument is to demonstrate the existence of suitably large, (local) packing in $\Gr$. This hinges on the ability to estimate the volume of a ball of radius $\delta$ (in the subspace angle distance), we denote $\vol(B(\delta))$\footnote{Given exact expression for $\vol(B(\delta_1))$ and $\vol(B(\delta_2))$ the standard Hamming and Gilbert-Varshamov arguments can be used to compute bounds on the packing/covering numbers of a $\delta_1$ ball by $\delta_2$ balls.}. Our argument builds on techniques from the coding theory literature in \citet{barg2002bounds} which (in the $d \to \infty$ limit) estimate the volume of balls in the $\Gr$ in the chordal distance. The argument begins by explicitly writing down a (reduced) expression for the volume form isolated to the density on the principal angles $\theta_1, \hdots, \theta_k$: $
		\int_{\Omega} f(\x) e^{d \cdot S(\x)} d \x$
	where $x_i = \sin \theta_i$, $S(\x) = \sum_{i=1}^r \ln(x_i)$,	$f(\x) = \left( \Pi_{i=1}^r x_i^{-2r} (1-x_i^2)^{-1/2} \right) \Pi_{i < j} (x_i^2-x_j^2)$, and $\Omega = \{ \x : \norm{\x}_{\infty} \leq \delta, 0 < x_1 < x_2 \hdots < x_r < 1 \}$. The expression is complicated. However, intuitively as $d \to \infty$ the $e^{d S(\x)}$ will decay quickly away from the point $\xstar = \arg \max_{x} S(\x)$ and we might expect the integral can be approximated by restricting to the region around $\xstar$  using $S(\x) \approx S(\xstar) + \frac{1}{2}((\x-\xstar)^\top H(\xstar)(\x-\xstar)^\top$ where $H$ is the Hessian of $S$. The Laplace method renders this intuition rigorous (see \cref{thm:ball_vol} for the full statement). 
	
	The second step is to upper bound the mutual information $I(Z; J)$. To begin we use a standard, convexity-based upper bound on the mutual information $I(Z; J) \leq \sum_{i \neq j}^{M} \KL(\Pr_{\B_i},\Pr_{\B_j})$. This bound is convenient in our linear model setting since the KL-divergence between the Gaussian distributed conditionals of $\y | \X, \B_i$ can be analytically computed; this expression can in turn be written as a function of the angular distance between $\B_i$ and $\B_j$ and bounded by the diameter of the local packing. Combining these two results and tuning the size of the (local) packing, paying mind to the error arising from approximating the packing number, gives the result.
\vspace{-0.3cm}





==> icml/train_mom.tex <==
%!TEX root = main.tex

\section{Learning Linear Features}
\label{sec:lf_mom}
\begin{algorithm}[!t]
\caption{MoM Estimator for Learning Linear Features}\label{algo:LF_learn}
\begin{algorithmic}
\renewcommand{\algorithmicrequire}{\textbf{Input: }}
\renewcommand{\algorithmicensure}{\textbf{Output: }}
\REQUIRE $\{ (\x_i, y_i) \}_{i=1}^{n_1}$.
\STATE $\Bone \D_1 \Bone \trans \leftarrow$ top-$r$ SVD of $\frac{1}{n_1} \cdot \sum_{i=1}^{n_1} y_i^2 \x_i\x_i\trans$
\STATE \textbf{return} $\Bone$
\end{algorithmic}
\end{algorithm}
Here we address both the algorithmic and statistical challenges of provably learning the feature representation $\B$. We begin by presenting a method-of-moments algorithm to recover the feature matrix $\B$ as an alternative to optimization-based approach such as maximum likelihood estimation. The method of moments is amongst the oldest statistical techniques dating back to Pearson's solution for parameter identification in a two-mixture Gaussian model \citep{pearson1894contributions}. It has also seen a recent revival in a series of works where it has been used to estimate parameters in latent variable models (see \citep{anandkumar2012method} for example).

As we will see, the technique is particularly well-suited to the problem of multi-task feature learning we consider (and its use in this setting is novel). Before presenting our first result we define the averaged empirical task matrix as $\barLambda = \sumton \balpha_{t(i)} \balpha_{t(i)}^\top$ where $\tnu = \sigma_{r}(\barLambda)$, and $\tkappa = \frac{\tr(\barLambda)}{r \tnu}$ in analogy with \cref{assump:task}.
\begin{theorem}
Suppose the $n_1$ data samples $\{ (\x_i, y_i) \}_{i=1}^{n_1}$ are generated from the model in \eqref{eq:model_main} and that \cref{assump:design} holds. Then if $n_1 \gtrsim \polylog(d, n_1) rd   \tkappa /\tnu$ the output $\Bone$ of \cref{algo:LF_learn} satisfies,
\begin{align*}
	\sin \theta(\Bone, \B) \leq \tlO \left(\sqrt{\frac{\tkappa}{\tnu} \frac{d  r}{n_1}} \right)
\end{align*}
with probability at least $1-O(n_1^{-100})$. Moreover, under \cref{assump:task} if the number of samples generated from each task are equal (i.e. $\barLambda = \frac{1}{t} \A^\top \A$), then the aforementioned guarantee holds with $\tkappa=\bkappa$ and $\tnu=\nu$.
\label{thm:B_recovery}
\end{theorem}
We first make several remarks regarding this result before sketching the proof of the theorem.
\begin{itemize}[leftmargin=.5cm]
	\vspace{-0.3cm}
	\item \cref{thm:B_recovery} is flexible -- the only dependence of the estimator on the distribution of samples across the various tasks is factored into the \textit{empirical} task diversity parameters $\tnu$ and $\tkappa$. Under a uniform observation model the guarantee also immediately translates into an analogous statement which holds with the population task diversity parameters $\nu$ and $\bkappa$.
	\item \cref{thm:B_recovery} provides a non-trivial guarantee even in the setting where we only have $\Theta(1)$ samples from each task but $t=\tlTheta(dr)$. In this setting, recovering the parameters of any given task is information-theoretically impossible. However, the method-of-moment estimator can efficiently aggregate information \textit{across} the tasks to learn $\B$. 
	\item The estimator does rely on the moment structure implicit in the Gaussian design to extract $\B$. However, \cref{thm:B_recovery}, to our knowledge, establishes the first information-theoretically optimal recovery guarantee for linear feature learning\footnote{up to logarithmic/conditioning parameter factors.} (see \cref{thm:feature_lb} for our lower bound).
\end{itemize}

We now briefly sketch the proof of the theorem. Under oracle access to the population mean $\mE[\frac{1}{n} \sum_i y_i^2 \x_i \x_i^\top] = (2\barGamma + (1+\tr(\barGamma)) \I_d)$, where $\barGamma = \sumton \B \balpha_{t(i)} \balpha_{t(i)}^\top \B^\top$ (see \cref{lem:estimator_mean}), we can extract the features $\B$ by directly applying PCA to this matrix under the condition that $\tkappa > 0$ to extract its column space. In practice, we only have access to the samples $\{(\x_i, y_i) \}_{i=1}^{n}$.  \cref{algo:LF_learn} uses the empirical moments $\frac{1}{n} \sum_i y_i^2 \x_i \x_i^\top$ in lieu of the population mean. To show the result, we argue that $\sumton y_i^2 \x_i\x_i\trans = \mE[\sumton y_i^2 \x_i\x_i\trans] + \E$ where $\norm{\E}$ is small, stochastic error (see \cref{thm:estimator_conc}). If this holds, the Davis-Kahan $\sin \theta$ theorem \citep{bhatia2013matrix} shows PCA applied to the empirical moments provides an accurate estimate of $\B$ under perturbation by a sufficiently small $\E$.

 The key technical step to show this estimator works is to show sharp concentration (in spectral norm) of several, matrix-valued noise terms $\E_1$, $\E_2$, and $\E_3$,
\begin{align*}
	& \sumton y_i^2 \x_i\x_i\trans - (2\barGamma + (1+\tr(\barGamma)) \I_d = \E_1+\E_2+\E_3.
\end{align*}
which separate the empirical moment from its population mean (see \cref{lem:first_noise,,lem:second_noise,,lem:third_noise}). The exact forms are deferred to the \cref{app:mom}, but as an example we have that $\E_2 = \sumton 2 \epsilon_i \x_i^\top \B \balpha_{t(i)} \x_i \x_i^\top$. The noise terms $\E_1, \E_2, \E_3$ are neither bounded (in spectral norm) nor sub-gaussian/sub-exponential-like since they contain 4th-order terms in the $\x_i$ and $\epsilon_i$. The important tool we use to show concentration of measure for these objects is a truncation argument along with the matrix Bernstein inequality (see \cref{lem:trunc_mb}). 
\vspace{-0.3cm}

==> train_gd.tex <==
%!TEX root = main.tex
\section{The Landscape of Feature Learning}
\label{sec:lf_gd}
The remarkable, practical success of first-order methods for training non-convex optimization problems (including meta/multi-task learning objectives) motivates us to study the optimization landscape of the empirical risk induced by the model in \eqref{eq:model_main}. While a comprehensive analysis of the global landscape of solutions is beyond the scope of this paper, we present evidence that first-order methods can find \textit{local minima that generalize well}. 

Jointly learning the population parameters $\B$ and $(\balpha_1, \hdots, \balpha_t)^\top$ defined by \cref{eq:model_main} is remniscent of a matrix sensing/completion problem and we leverage this connection for our analysis \citep{ge2017no}. Throughout this section assume that we are in a uniform task sampling model -- at each iteration the task $t(i)$ for the $i$th datapoint is uniformly sampled from the $t$ underlying tasks. We first recast our problem in the language of matrices, by defining the matrix we hope to recover as $\M_{\star} = (\balpha_1, \hdots, \balpha_t)^\top \B^\top  \underbrace{=}_{\text{SVD}} \X^{\star} \D^{\star} (\Y^{\star})^\top \in \mR^{t \times d}$,  $\U^{\star}=\X^{\star} (\D^{\star})^{1/2}$, $\V^{\star} = (\D^{\star})^{1/2} \Y^{\star}$ and letting $\sigstarl$ and $\sigstarr$ denote the $1$st and $r$th singular values of $\M^{\star}$ and $\kappa^{\star}=\sigstarl/\sigstarr$ its condition number. In this notation, we see the observations\footnote{We rescaled the model and introduce a noise scale $\sigma$ here for convenience.},
\begin{align}
	y_i = \langle \sqrt{t} \e_{t(i)} \x_i^\top, \M_{\star} \rangle + \sqrt{t} \sigma \cdot \epsilon_i
\end{align}
To frame recovery as an optimization problem we consider the Burer-Monteiro factorization of the parameter $\M = \U \V^\top$, which motivates the objective, 
\begin{align}
	& \min_{\U \in \mR^{t \times r}, \V \in \mR^{d \times r}} f(\U, \V) \quad \text{where} \ f(\U, \V) = \label{eq:objective_main} \\
	& \frac{2}{n} \sum_{i=1}^{n} (y_i-\sqrt{t} \langle \e_{t(i)} \x_i^\top , \U \V^\top \rangle)^2 +  \frac{1}{2}\fnorm{\U^\top \U-\V^\top \V}^2 \nonumber.
\end{align}
The second term in \cref{eq:objective_main} functions as a regularization to prevent solutions which send $\fnorm{\U} \to 0$ while $\fnorm{\V} \to \infty$. If the value of this objective \cref{eq:objective_main} is small we might hope that an estimate of $\B$ can be extracted from the column space of the parameter $\V$, since the column space of $\V^{\star}$ spans the same subspace as $\B$. Informally, our main result states that all local minima of the regularized \textit{empirical} risk in the neighborhood of the optimal $\V^{\star}$ have subspaces that approximate $\B$ well. Before stating our result we define the local ``incoherence" set as,
\begin{align*}
& \cW = \{~ (\U, \V) ~|~ \max_{i\in[t]} \norm{\e_i\trans \U}^2 \le \frac{C_0 \bkappa r \sigstarl}{t}, \\
& \quad \norm{\U}^2 \le C_0 \sigstarl, \quad \norm{\V}^2 \le C_0 \sigstarl ~\}
\label{eq:constraint_main}
\end{align*}
for some large constant $C_0$. This set contains the optimal parameters\footnote{Note $\U^{\star}$ and $\V^{\star}$ satisfy the final two constraints by definition and \cref{lem:diverse_to_incoh} can be used to show that that \cref{assump:task} actually implies $\U^{\star}$ satisfies the first incoherence-like constraint.} under \cref{assump:task}. Our main result then becomes, 
\begin{theorem}\label{thm:main_landscape_convert}
Let \cref{assump:design,,assump:task} hold in the uniform task sampling model. If the number of samples $n_1$ satisfies $n_1 \gtrsim \polylog(n_1,d,t) \bkappa^2 r^4 \max\{t, d\}  (\cn^\star)^4$, then with probability at least $1-1/\poly(d)$, we have that given any local minimum $(\U, \V) \in \text{int}(\cW)$ of the objective \cref{eq:objective_main}, the column space of $\V$, spanned by the orthonormal feature matrix $\Bone$, satisfies:
\begin{equation*}
\sin \theta(\Bone, \B) \leq O \left( \frac{\sigma}{\sqrt{\nu}} \sqrt{\frac{\max\{t, d\} r\log n_1}{n_1}} \right).
\end{equation*}
\end{theorem}
We make several comments on this result,
\vspace{-0.3cm}
\begin{itemize}[leftmargin=.5cm]
	\item In short, the guarantee in \cref{thm:main_landscape_convert} suggests the local optimization landscape near $\M^{\star}$ will not inhibit generalization. \cref{thm:feature_lb} guarantees any estimator (including the empirical risk minimizer) must incur error $\gtrsim \sqrt{\frac{d r}{n}}$. In the regime $t \leq O(d)$, \cref{thm:main_landscape_convert}, ensures with enough samples $n_1 \gtrsim \poly(r) d$, all local minima are at most $\tlO(\sqrt{\frac{dr}{n_1}})$ away from the true solution. Thus, the error from finding a local minima of the empirical risk -- contained in the set $\text{int}(\cW)$ -- is of roughly the same order as the statistical generalization error.
	\item Recent work in \citet{jin2017escape} shows that (noisy) gradient descent can efficiently escape strict saddle points to find local minima. While \cref{thm:main_landscape_convert} does not fully characterize the global geometry of the objective, we believe in conjunction with the previous result provides preliminary evidence that first-order methods can efficiently meta-learn linear features. 
	\vspace{-0.2cm}
\end{itemize}
The proof of \cref{thm:main_landscape_convert} is technical so we only sketch the high-level ideas. The overall strategy is to analyze the Hessian of the objective \cref{eq:objective_main} at a stationary point $(\U, \V)$ in $\text{int}(\cW)$ to exhibit a direction $\Delta$ of negative curvature which can serve as a direction of local improvement pointing towards $\M^{\star}$ (and hence show $(\U, \V)$ is not a local minimum). Implementing this idea requires surmounting several technical hurdles including 1. establishing various concentration of measure results (e.g., RIP-like conditions) for the sensing matrices $\sqrt{t} \e_{t(i)} \x_i^\top$ unique to our setting and 2. handling the interaction of the optimization analysis with the regularizer and noise terms. Performing this analysis establishes that under the aforementioned conditions all local minima in $\text{int}(\cW)$ satisfy, $
	\norm{\U\V^\top - \M^\star}_F\leq O(\sigma\sqrt{t\frac{\max\{t, d\} r\log n}{n}})
$
(see \cref{thm:main_landscape}).
Guaranteeing this loss is small is not sufficient to ensure recovery of the underlying features. Transferring this guarantee in the Frobenius norm to a result on the subspace angle critically uses the task diversity assumption (see \cref{lem:frob_to_angle}) to give the final result.
\vspace{-0.3cm}
